There Once Was a Really Bad Poet, It Was Automated but You Didn't Know It

Limerick generation exemplifies some of the most difficult challenges faced in poetry generation, as the poems must tell a story in only five lines, with constraints on rhyme, stress, and meter. To address these challenges, we introduce LimGen, a novel and fully automated system for limerick generation that outperforms state-of-the-art neural network-based poetry models, as well as prior rule-based poetry models. LimGen consists of three important pieces: the Adaptive Multi-Templated Constraint algorithm that constrains our search to the space of realistic poems, the Multi-Templated Beam Search algorithm which searches efficiently through the space, and the probabilistic Storyline algorithm that provides coherent storylines related to a user-provided prompt word. The resulting limericks satisfy poetic constraints and have thematically coherent storylines, which are sometimes even funny (when we are lucky).

==> LimGen_poem.tex <==
1: \textit{Surprise:-2.943}, Method: LimGen\\
There was a silly man named Dwight,
Who did all his writing in a night. 
His stories were so sweet, 
They were the perfect treat, 
But he knew he was doing it right. \\ \vspace{0.1pt}

2: \textit{Shaken:-3.222}, Method: LimGen\\
There was a loud waiter named Les,
Who poured a cold beer on our mess. 
When we returned to stand, 
We were met by our band, 
And that is the end of this process. \\ \vspace{0.1pt}

3: \textit{Born:-2.970}, Method: LimGen\\
There was a brave boy named Stan,
Who lived all his life within a man. 
He was a physician, 
He was on a mission, 
He was ready to die and to plan. \\ \vspace{0.1pt}

4: \textit{Humiliation:-3.080}, Method: LimGen\\
There was a cruel boy named Pierre,
Who faced all his life in a nightmare. 
When he returned to hell, 
He was saved by a spell, 
But he does not trust in his prayer. \\ \vspace{0.1pt}

5: \textit{Kindness:-3.436}, Method: LimGen\\
There was a selfish man named Cole,
Who loved a young lady on his soul. 
But his heart was cruel, 
And he was to the fool, 
And that is the reason of this hole. \\ \vspace{0.1pt}

6: \textit{Laugh:-3.293}, Method: LimGen\\
There once was a grandpa named Dewitt,
Who loved a good story on his spit. 
His stories were so cool, 
He had so much fuel, 
It was hard to keep a straight outfit. \\ \vspace{0.1pt}

7: \textit{Restore:-2.958}, Method: LimGen\\
There was a vain man named Stan,
Who lost all his money in a plan. 
When he returned to work, 
He was told by a clerk, 
And that is the reason of this ban. \\ \vspace{0.1pt}

8: \textit{Tears:-3.394}, Method: LimGen\\
There was a vain boy named Dwight,
Who cried a great deal on our sight. 
He was a nobody, 
And he was to the sea, 
So we went up and put on the light. \\ \vspace{0.1pt}

9: \textit{Victory:-3.081}, Method: LimGen\\
There once was a captain named Theodore,
Who lost all his money in a war. 
When he returned to court, 
He was forced by his tort, 
And that is the reason of this score. \\ \vspace{0.1pt}

10: \textit{Christmas:-2.830}, Method: LimGen\\
There was a lucky boy named Dwight,
Who got all his money in a night. 
It was for his birthday, 
And he went to the play, 
So he had to go down on the right. \\ \vspace{0.1pt}

11: \textit{Wedding:-2.775}, Method: LimGen\\
There was a tailor named Jess,
Who cut out my nipples for a dress. 
It was for my birthday, 
Which I was in the way, 
So I had to go down on the mess. \\ \vspace{0.1pt}

12: \textit{Thanksgiving:-2.907}, Method: LimGen\\
There was a humble chef named Dwight,
Who cooked a great meal on our night. 
It was for his birthday, 
Which we were in the way, 
So we never got on the invite. \\ \vspace{0.1pt}

13: \textit{Holiday:-2.789}, Method: LimGen\\
There was a silly chef named Kip,
Who spent all his money in a trip. 
When he returned to town, 
He was met by a clown, 
And that is the story of this strip. \\ \vspace{0.1pt}

14: \textit{Alien:-3.215}, Method: LimGen\\
There was a cunning man named Kip,
Who trapped a young woman on his ship. 
When he returned to land, 
He was met by his band, 
And they took down and captured his whip. \\ \vspace{0.1pt}

15: \textit{Birthday:-2.912}, Method: LimGen\\
There was a jealous boy named Dwight,
Who got all his money in a night. 
When he went to midnight, 
He was met by a light, 
So he had to go down on the right. \\ \vspace{0.1pt}

16: \textit{Pillow:-2.862}, Method: LimGen\\
There was a skinny boy named Ted,
Who slept a good deal on our bed. 
And in our bedroom, 
Which we shared in the room, 
We had plenty to eat and to read. \\ \vspace{0.1pt}

17: \textit{Fiance:-2.889}, Method: LimGen\\
There was a shy grandpa named Jake,
Who loved a good story on his cake. 
The day of his birthday, 
He was ready to play, 
So he went to work down on the lake. \\ \vspace{0.1pt}

18: \textit{Dawn:-3.078}, Method: LimGen\\
There once was a soldier named Pierre,
Who slept all his life in a nightmare. 
He came back from the war, 
Broke the chains that he wore, 
And that is the story of this bear. \\ \vspace{0.1pt}

19: \textit{Traffic:-2.972}, Method: LimGen\\
There once was a man named Pete,
Who drove a white van on our street. 
It was on the highway, 
He was stopped by a stray, 
So he had to get down on the seat. \\ \vspace{0.1pt}

20: \textit{Wine:-3.411}, Method: LimGen\\
There was a waiter named Chase,
Who served a great meal on our place. 
Our servers were so sweet, 
And our server and meat, 
We thoroughly enjoyed our space. \\ \vspace{0.1pt}

21: \textit{Heartbreak:-2.684}, Method: LimGen\\
There once was a boy named Pierre,
Who cried all his life in a nightmare. 
He came back from the grave, 
And he went to the cave, 
And he sat down and wrote his prayer. \\ \vspace{0.1pt}

22: \textit{Beer:-2.819}, Method: LimGen\\
There was a lucky chef named Dwight,
Who ate all his chicken in a night. 
When he returned to town, 
He was met by a clown, 
And that is the story of this site. \\ \vspace{0.1pt}

23: \textit{River:-2.872}, Method: LimGen\\
There was a brave man named Nathanael,
Who crossed a great river on his sail. 
He came back from the sea, 
With a sword on his knee, 
And set fire to his ship in detail. \\ \vspace{0.1pt}

24: \textit{Musuem:-3.260}, Method: LimGen\\
There once was a blacksmith named Pete,
Who housed a small shop on our street. 
When we moved to greenwood, 
Our house was so good, 
We were able to rent and to eat. \\ \vspace{0.1pt}

25: \textit{Mountain:-3.176}, Method: LimGen\\
There was a quiet man named Jermaine,
Who traveled together in a train. 
He was on the railroad, 
So he went down the road, 
Then turned into a tunnel of pain. \\ \vspace{0.1pt}

26: \textit{Injury:-2.971}, Method: LimGen\\
There was a firefighter named Marquis,
Who caused a small fire on his knee. 
When he returned to fight, 
He was struck by a light, 
So he had to go down on the tree. \\ \vspace{0.1pt}

27: \textit{Mud:-2.967}, Method: LimGen\\
There was a lazy man named Cole,
Who stuck all his money in a hole. 
He got back from the cave, 
And he went to the grave, 
And that is the story of this soul. \\ \vspace{0.1pt}

28: \textit{Spider:-3.221}, Method: LimGen\\
There was a nasty boy named Jerrell,
Who trapped a young lady on his tail. 
It was like a nightmare, 
He was scared by his hair, 
He was afraid to move and to fail. \\ \vspace{0.1pt}

29: \textit{Rain:-2.843}, Method: LimGen\\
There was a quiet boy named Jerrell,
Who kept a close eye on our trail. 
When we arrived to ride, 
We were met by our guide, 
And that is the story of this tale. \\ \vspace{0.1pt}

30: \textit{Memory:-2.707}, Method: LimGen\\
There was a wise grandpa named Chase,
Who lost all his money in a case. 
He came back from the grave, 
He was able to save, 
And now he has a family place. \\ \vspace{0.1pt}

31: \textit{Season:-2.988}, Method: LimGen\\
There was a actor named Beau,
Who played a big role on our show. 
He came back from the past, 
And he was to the cast, 
But he does not work in our shadow. \\ \vspace{0.1pt}

32: \textit{Winter:-2.850}, Method: LimGen\\
There was a harsh boy named Dwight,
Who spent all his money in a night. 
When he got to midnight, 
He was ready to fight, 
So he went up and put on the light. \\ \vspace{0.1pt}

33: \textit{Throne:-3.225}, Method: LimGen\\
There was a fierce man named Javier,
Who stood all his life in a prayer. 
He was like a shadow, 
And he was to the show, 
So he had to go down on the chair. \\ \vspace{0.1pt}

34: \textit{Bank:-2.820}, Method: LimGen\\
There was a smart farmer named Pete,
Who owned a small farm on our street. 
The owner of our town, 
His wife had a breakdown, 
She was afraid to live and to eat. \\ \vspace{0.1pt}

35: \textit{Politics:-2.925}, Method: LimGen\\
There was a general named Theodore,
Who learned a great deal on our war. 
When he returned to fight, 
He was struck by a light, 
So he had to go down on the floor. \\ \vspace{0.1pt}

36: \textit{Promise:-3.130}, Method: LimGen\\
There was a lucky man named Bill,
Who did a great job on our will. 
He came back from the break, 
He was ready to take, 
So we had to go down on the hill. \\ \vspace{0.1pt}

37: \textit{Money:-2.969}, Method: LimGen\\
There was a honest man named Rashad,
Who lost all his money in a fraud. 
When he returned to work, 
He was told by his clerk, 
That the amount he had paid a god. \\ \vspace{0.1pt}

38: \textit{Limerick:-3.759}, Method: LimGen\\
There was a plumber named Jerrell,
Who wright all his money in a tale. 
It was a satire, 
But it also had fire, 
So it had to go down on the scale. \\ \vspace{0.1pt}

39: \textit{Love:-2.812}, Method: LimGen\\
There was a lucky man named Scot,
Who got all his money in a lot. 
It was for his birthday, 
And he went to the play, 
So he had to go down on the spot. \\ \vspace{0.1pt}

40: \textit{Cunning:-3.165}, Method: LimGen\\
There was a magician named Rick,
Who fooled all his family in a trick. 
But his father was cruel, 
His mother was a fool, 
So he had to go down on the stick. \\ \vspace{0.1pt}

41: \textit{Dog:-2.970}, Method: LimGen\\
There was a lucky boy named Wayne,
Who got a free ride on our train. 
He asked for his girlfriend, 
He was told by his friend, 
So he went up and slept on the plane. \\ \vspace{0.1pt}

42: \textit{Blood:-2.995}, Method: LimGen\\
There was a nasty man named Dwight,
Who drank all his money in a fight. 
When he returned to hell, 
He was killed by a spell, 
So he had to go down on the light. \\ \vspace{0.1pt}

43: \textit{Death:-2.690}, Method: LimGen\\
There once was a soldier named Javier,
Who lived all his life in a nightmare. 
He came back from the war, 
And he went to the store, 
And he looked down and said his prayer. \\ \vspace{0.1pt}

44: \textit{War:-2.901}, Method: LimGen\\
There was a fierce man named Dwight,
Who killed all his family in a fight. 
When he returned to hell, 
He was saved by a spell, 
And now he is a hero outright. \\ \vspace{0.1pt}

45: \textit{Disease:-3.257}, Method: LimGen\\
There was a doctor named Zane,
Who caused a big problem on my brain. 
When I got to trial, 
I was shocked by his style, 
And that is the reason of this pain. \\ \vspace{0.1pt}

46: \textit{World:-2.787}, Method: LimGen\\
There was a general named Chase,
Who lived a long time on our place. 
He was back from the war, 
And he came to the door, 
So we had to go down on the base. \\ \vspace{0.1pt}

47: \textit{Planet:-3.012}, Method: LimGen\\
There was a cruel man named Cole,
Who lived all his life within a hole. 
He was like a shadow, 
And he came to the snow, 
And that is the story of this soul. \\ \vspace{0.1pt}

48: \textit{Fire:-3.185}, Method: LimGen\\
There was a brave man named Saul,
Who put all his money in a wall. 
When he went to someone, 
He was told by his son, 
He said that his father was football. \\ \vspace{0.1pt}

49: \textit{Beach:-2.982}, Method: LimGen\\
There was a lazy man named Kip,
Who went a long distance on his trip. 
When he returned to town, 
He was met by a clown, 
So he gave up and quit on the ship. \\ \vspace{0.1pt}

50: \textit{Water:-2.986}, Method: LimGen\\
There was a harsh man named Scot,
Who put all his money in a pot. 
When he went to spring, 
He was met by a ring, 
And that is the reason of this knot. \\ \vspace{0.1pt}

51: \textit{Love:-2.850}, Method: LimGen\\
There was a lucky boy named Scot,
Who did a great job on our lot. 
When we arrived to work, 
We were met by our clerk, 
So we had to sit down on the spot. \\ \vspace{0.1pt}

52: \textit{Sports:-2.828}, Method: LimGen\\
There was a smart boxer named Claudio,
Who played a big role on our show. 
He was on the program, 
He was on a programme, 
And he came down and had his photo. \\ \vspace{0.1pt}

53: \textit{Car:-3.092}, Method: LimGen\\
There was a loud cleaner named Pete,
Who ran a small shop on our street. 
He would come to a place, 
We were on a staircase, 
And say hi to my daughter in heat. \\ \vspace{0.1pt}

54: \textit{Animal:-3.063}, Method: LimGen\\
There was a nasty boy named Nathanael,
Who made a big mess on our tail. 
He was back from the sea, 
He was ready to flee, 
He was sure to find a nice female. \\ \vspace{0.1pt}

55: \textit{Violent:-2.867}, Method: LimGen\\
There was a cruel man named Salvador,
Who killed all his family in a war. 
When he returned to hell, 
He was met by a bell, 
And that is the story of this door. \\ \vspace{0.1pt}

56: \textit{Opera:-2.756}, Method: LimGen\\
There was a actor named Claudio,
Who played a big role on our show. 
When we started to work, 
We were on a network, 
We were ready to go and to grow. \\ \vspace{0.1pt}

57: \textit{Monster:-3.040}, Method: LimGen\\
There was a stupid man named Cole,
Who got all his money in a hole. 
It was like a nightmare, 
He was trapped by his hair, 
So he had to go down on the pole. \\ \vspace{0.1pt}

58: \textit{Doctor:-2.637}, Method: LimGen\\
There was a surgeon named Dane,
Who did a great job on our brain. 
He was a physician, 
He was on a mission, 
He totally understood our pain. \\ \vspace{0.1pt}

59: \textit{Library:-3.124}, Method: LimGen\\
There was a general named Dwight,
Who found a great treasure on his site. 
When he returned to work, 
He was met by a clerk, 
So he went up and put on the light. \\ \vspace{0.1pt}

60: \textit{Noble:-3.173}, Method: LimGen\\
There was a vain soldier named Theodore,
Who wished all his money in a war. 
But his father was cruel, 
His mother was a fool, 
So he went to live down on the shore. \\ \vspace{0.1pt}

61: \textit{Ball:-2.868}, Method: LimGen\\
There was a stupid boy named Cole,
Who threw all his money in a hole. 
When he returned to play, 
He was ready to pay, 
And that is the story of this role. \\ \vspace{0.1pt}

62: \textit{Funeral:-3.033}, Method: LimGen\\
There once was a soldier named Salvador,
Who killed all his family in a war. 
He came back from the grave, 
He was the perfect slave, 
He was not the enemy he bore. \\ \vspace{0.1pt}

63: \textit{Body:-2.888}, Method: LimGen\\
There was a skinny man named Chase,
Who put a big smile on our face. 
His eyes were so intense, 
He made every sense, 
And that is the beauty of this place. \\ \vspace{0.1pt}

64: \textit{Smart:-3.067}, Method: LimGen\\
There was a wise boy named Dick,
Who put all his money in a trick. 
He was a nobody, 
He got caught by a tree, 
So he had to go down on the stick. \\ \vspace{0.1pt}

65: \textit{Exercise:-3.358}, Method: LimGen\\
There was a wise doctor named Rex,
Who practiced on one of my subjects. 
He had a condition, 
And with his permission, 
I went through the test and found defects. \\ \vspace{0.1pt}

66: \textit{Art:-3.100}, Method: LimGen\\
There was a teacher named Cole,
Who made a big impact on my soul. 
When I came to childhood, 
My mother was so good, 
She was really the reason I stole. \\ \vspace{0.1pt}

67: \textit{Gun:-2.903}, Method: LimGen\\
There was a loud soldier named Chase,
Who put a big smile on our face. 
He was a nobody, 
He was killed by a tree, 
But he is still live in our place. \\ \vspace{0.1pt}

68: \textit{Forest:-2.997}, Method: LimGen\\
There was a fierce farmer named Nathanael,
Who hunted as he went on a trail. 
When he got to willow, 
He was met by a crow, 
So he had to go down on the tail. \\ \vspace{0.1pt}

69: \textit{Music:-2.828}, Method: LimGen\\
There was a loud artist named Gaylord,
Who played a big role on our record. 
When we started to play, 
It was easy to say, 
So we had to go down on the board. \\ \vspace{0.1pt}

70: \textit{Boxing:-2.472}, Method: LimGen\\
There was a fierce boxer named Dwight,
Who lost all his money in a fight. 
When he tried to retire, 
He was killed by a fire, 
Then turned into a spirit of light. \\ \vspace{0.1pt}

71: \textit{Philosophy:-3.202}, Method: LimGen\\
There was a wise teacher named Rex,
Who taught on a number of subjects. 
When he returned to school, 
He was struck by his cool, 
And now he has a degree complex. \\ \vspace{0.1pt}

72: \textit{Night:-3.040}, Method: LimGen\\
There once was a boy named Chase,
Who had all his money in a place. 
He would go to a show, 
He would get a photo, 
And that is the picture of this case. \\ \vspace{0.1pt}

73: \textit{Market:-2.987}, Method: LimGen\\
There once was a farmer named Jerrell,
Who sold all his produce in a sale. 
When he returned to store, 
He was met by a door, 
Which was sealed with the greatest detail. \\ \vspace{0.1pt}

74: \textit{Scary:-3.115}, Method: LimGen\\
There was a boring boy named Joaquin,
Who seemed a good fit on our scene. 
When we started to talk, 
He was ready to walk, 
He was willing to learn and to lean. \\ \vspace{0.1pt}

75: \textit{Creativity:-3.384}, Method: LimGen\\
There was a writer named Les,
Who learned a great deal on his process. 
When he started to work, 
He would have a framework, 
And it was much like writing of chess. \\ \vspace{0.1pt}

76: \textit{Angry:-3.205}, Method: LimGen\\
There was a loud boy named Dwight,
Who shouted as he went on a fight. 
When he came to protest, 
He was met by his guest, 
And that is the story of this night. \\ \vspace{0.1pt}

77: \textit{Evil:-3.207}, Method: LimGen\\
There was a cruel man named Javier,
Who thought as he did on a nightmare. 
He was like a shadow, 
And he looked to the snow, 
Then he saw it glowing in the air. \\ \vspace{0.1pt}

78: \textit{Law:-3.208}, Method: LimGen\\
There was a wise judge named Lyle,
Who brought a young man on his trial. 
He was back from the war, 
But had a new mentor, 
And that is the story of this file. \\ \vspace{0.1pt}

79: \textit{Pride:-3.479}, Method: LimGen\\
There was a honest man named Cole,
Who loved a good story on his soul. 
It was a tradition, 
I would say a mission, 
But it does not happen in my role. \\ \vspace{0.1pt}

80: \textit{School:-2.872}, Method: LimGen\\
There was a lucky boy named Saul,
Who got all his money in a fall. 
When he returned to town, 
He was met by a clown, 
So he had to go down on the ball. \\ \vspace{0.1pt}

81: \textit{Light:-3.100}, Method: LimGen\\
There was a cleaner named Ervin,
Who made a huge difference on my skin. 
When I started to fall, 
I was able to crawl, 
But I felt I was wearing it thin. \\ \vspace{0.1pt}

82: \textit{Rich:-3.141}, Method: LimGen\\
There was a smart man named Ervin,
Who made a big difference on my skin. 
When I started to shine, 
I had so much sunshine, 
So I had to go down on the chin. \\ \vspace{0.1pt}

83: \textit{Color:-3.152}, Method: LimGen\\
There was a cleaner named Chase,
Who used a big hammer on my face. 
When I tried to object, 
He said something perfect, 
So I had to go down on the place. \\ \vspace{0.1pt}

84: \textit{Loss:-2.907}, Method: LimGen\\
There was a nervous man named Jamal,
Who lost all his money in a fall. 
When he returned to fight, 
He was stunned by his plight, 
And that is the story of this brawl. \\ \vspace{0.1pt}

85: \textit{Park:-3.226}, Method: LimGen\\
There was a lucky boy named Kip,
Who went a long way on our trip. 
When we returned to town, 
We saw the old playground, 
But it does not hold in our grip. \\ \vspace{0.1pt}

86: \textit{Airplane:-3.025}, Method: LimGen\\
There once was a captain named Chase,
Who blew all his money in a chase. 
When he returned to ship, 
He was ordered to strip, 
And he stripped down and started his race. \\ \vspace{0.1pt}

87: \textit{Useful:-3.189}, Method: LimGen\\
There was a smart tailor named Scot,
Who put all his money in a lot. 
When he started to work, 
He got laid by a clerk, 
And that is the reason of this plot. \\ \vspace{0.1pt}

88: \textit{Weight:-2.938}, Method: LimGen\\
There once was a boxer named Scot,
Who lost all his money in a squat. 
When he returned to work, 
He was told by a clerk, 
That the building he had worked a lot. \\ \vspace{0.1pt}

89: \textit{Applaud:-3.233}, Method: LimGen\\
There was a humble judge named Javier,
Who praised a young woman on her dare. 
When she refused to stand, 
She was struck by his hand, 
And she fell down and broke her prayer. \\ \vspace{0.1pt}

90: \textit{Union:-3.176}, Method: LimGen\\
There was a fierce teacher named Dwight,
Who sought out his students for a fight. 
When they arrived to school, 
They were met by a pool, 
And it was then like lightning of light. \\ \vspace{0.1pt}

91: \textit{Home:-2.722}, Method: LimGen\\
There once was a man named Scot,
Who had all his money in a lot. 
He got back from the store, 
And he went to the door, 
So he had to get down on the spot. \\ \vspace{0.1pt}

92: \textit{Child:-3.144}, Method: LimGen\\
There was a teacher named Chase,
Who taught a small class on our place. 
When we arrived to school, 
We were met by a pool, 
So we got up and put on the race. \\ \vspace{0.1pt}

93: \textit{Cheat:-2.862}, Method: LimGen\\
There was a greedy man named Nick,
Who put all his money in a stick. 
He got back from the war, 
And he came to the door, 
And he looked down and saw my lipstick. \\ \vspace{0.1pt}

94: \textit{Hope:-3.052}, Method: LimGen\\
There was a honest boy named Wes,
Who did a great job on my progress. 
When I started to cry, 
I was told by a guy, 
That the reason I cried was a mess. \\ \vspace{0.1pt}

95: \textit{Working:-2.855}, Method: LimGen\\
There was a technician named Wes,
Who did a great job on our process. 
When we started to talk, 
It was easy to walk, 
And that is the beauty of this press. \\ \vspace{0.1pt}

96: \textit{Fall:-2.638}, Method: LimGen\\
There was a lucky boy named Chase,
Who did a great job on our place. 
We got back from the show, 
We were ready to go, 
And he came down and took our space. \\ \vspace{0.1pt}

97: \textit{Time:-3.118}, Method: LimGen\\
There was a honest man named Chase,
Who did a great job on our place. 
He was a nobody, 
He was born by a tree, 
And that is the beauty of this race. \\ \vspace{0.1pt}

98: \textit{Flower:-2.901}, Method: LimGen\\
There was a bright boy named Bert,
Who cut a nice figure on his shirt. 
It was for his birthday, 
He was happy to say, 
So he got up and put on the skirt. \\ \vspace{0.1pt}

99: \textit{Leader:-3.023}, Method: LimGen\\
There was a fierce soldier named Dwight,
Who led all my army in a fight. 
He was back from the war, 
And he was to the door, 
So I went up and put on the light. \\ \vspace{0.1pt}

100: \textit{Random:-3.087}, Method: LimGen\\
There was a boring man named Lyle,
Who stuck all his money in a pile. 
When he went to someone, 
He was told by his son, 
He has a good chance of a trial. \\ \vspace{0.1pt}

101: \textit{Impressive:-3.412}, Method: LimGen\\
There was a bright man named Hugh,
Who helped a young girl on her debut. 
His eyes were so intense, 
I was struck by his sense, 
That the way he looked was a statue. \\ \vspace{0.1pt}

102: \textit{Born:-2.574}, Method: LimGen\\
There once was a woman named Renee,
Who lived a good life on her birthday. 
She was a musician, 
She was on a mission, 
She was blessed to have a perfect day. \\ \vspace{0.1pt}

103: \textit{Tears:-2.821}, Method: LimGen\\
There once was a woman named Grace,
Who felt a deep longing on her face. 
It was like a prayer, 
And she prayed to the air, 
And that is the meaning of this place. \\ \vspace{0.1pt}

104: \textit{Restore:-2.981}, Method: LimGen\\
There was a wise cleaner named Jacque,
Who helped out her parents for a break. 
When they returned to work, 
They were told by a clerk, 
That the woman they saw was a fake. \\ \vspace{0.1pt}

105: \textit{Shaken:-3.314}, Method: LimGen\\
There was a loud waitress named Jacque,
Who poured all her coffee in a shake. 
But the moment she stirred, 
She was struck by a bird, 
Then she saw it fly towards the lake. \\ \vspace{0.1pt}

106: \textit{Surprise:-2.999}, Method: LimGen\\
There was a shy woman named Kay,
Who did a great job on my birthday. 
She was a nobody, 
She was pretty to see, 
She was pretty to hear and to say. \\ \vspace{0.1pt}

107: \textit{Kindness:-3.006}, Method: LimGen\\
There once was a grandma named Kay,
Who loved all her family in a way. 
It was like a prayer, 
And she prayed to the air, 
And that is the spirit of this day. \\ \vspace{0.1pt}

108: \textit{Victory:-2.992}, Method: LimGen\\
There was a fierce judge named Kay,
Who fought a great battle on her way. 
When she arrived to fight, 
She was met by a knight, 
She was glad to have a good birthday. \\ \vspace{0.1pt}

109: \textit{Humiliation:-2.851}, Method: LimGen\\
There once was a girl named Grace,
Who faced a big problem on her face. 
When she started to cry, 
She was saved by a guy, 
So she got up and put on the case. \\ \vspace{0.1pt}

110: \textit{Wedding:-3.001}, Method: LimGen\\
There once was a lady named Renee,
Who wore a red dress on her birthday. 
She was like a fairy, 
Though a little scary, 
She has a big heart out in the way. \\ \vspace{0.1pt}

111: \textit{Laugh:-3.185}, Method: LimGen\\
There once was a girl named Lorelei,
Who cried out her feelings for a guy. 
But the moment she did, 
She was caught by a kid, 
And that is the story of this lie. \\ \vspace{0.1pt}

112: \textit{Alien:-3.062}, Method: LimGen\\
There was a cruel witch named Ardelle,
Who trapped all my family in a hell. 
It was like a nightmare, 
I was scared by her stare, 
But I knew she was watching me spell. \\ \vspace{0.1pt}

113: \textit{Holiday:-2.990}, Method: LimGen\\
There was a silly chef named Kay,
Who spent all her money in a day. 
When she returned to town, 
She was met by a frown, 
Because she was wearing her resume. \\ \vspace{0.1pt}

114: \textit{Christmas:-2.920}, Method: LimGen\\
There was a grandma named Renee,
Who got a new car on her birthday. 
I was back from the store, 
And she was to the door, 
So I walked up and hit on the way. \\ \vspace{0.1pt}

115: \textit{Birthday:-3.129}, Method: LimGen\\
There was a lucky girl named Kay,
Who got all her money in a day. 
It was like a rainbow, 
And it was to the show, 
I thought that my character was gay. \\ \vspace{0.1pt}

116: \textit{Thanksgiving:-2.847}, Method: LimGen\\
There was a silly chef named Renee,
Who cooked a great meal on my birthday. 
It was a tradition, 
She was on a mission, 
And that is the reason of this day. \\ \vspace{0.1pt}

117: \textit{Pillow:-3.264}, Method: LimGen\\
There was a bright grandma named Freda,
Who slept all her life outside a bed. 
She was like a fairy, 
She lived on a ferry, 
But she does not sleep outside her head. \\ \vspace{0.1pt}

118: \textit{Fiance:-2.976}, Method: LimGen\\
There was a nervous girl named Renee,
Who talked a big game on her birthday. 
But the moment they met, 
She was ready to get, 
So she got up and put on the play. \\ \vspace{0.1pt}

119: \textit{Dawn:-2.903}, Method: LimGen\\
There was a harsh girl named Maire,
Who slept all her life in a nightmare. 
When she awoke to light, 
She was shocked by a sight, 
Then fell into a state of prayer. \\ \vspace{0.1pt}

120: \textit{Traffic:-3.134}, Method: LimGen\\
There was a quiet judge named Charmaine,
Who noticed as she was on a train. 
She asked for her address, 
Which she found in the dress, 
So she went up and put on the chain. \\ \vspace{0.1pt}

121: \textit{Heartbreak:-3.211}, Method: LimGen\\
There was a fierce woman named Nicolle,
Who cried a long time on our soul. 
Her tears were so intense, 
But they never left sense, 
And that is the beauty of this role. \\ \vspace{0.1pt}

122: \textit{Injury:-3.156}, Method: LimGen\\
There was a firefighter named Grace,
Who caused a small fire on her face. 
When she returned to fight, 
She was met by a light, 
And she fell down and broke her staircase. \\ \vspace{0.1pt}

123: \textit{Wine:-3.114}, Method: LimGen\\
There was a neat waitress named Renee,
Who cooked a great meal on our day. 
When we arrived to shop, 
We were met by a top, 
So we had to stop down on the way. \\ \vspace{0.1pt}

124: \textit{Beer:-3.262}, Method: LimGen\\
There was a silly chef named Kay,
Who cooked a great meal on our day. 
When we arrived to town, 
We were met by a brown, 
So we went up and drank on the way. \\ \vspace{0.1pt}

125: \textit{Musuem:-3.139}, Method: LimGen\\
There was a artist named Grace,
Who housed all her art in a staircase. 
It was like a statue, 
It was the perfect view, 
And that is the beauty of this place. \\ \vspace{0.1pt}

126: \textit{River:-2.806}, Method: LimGen\\
There was a farmer named Kay,
Who crossed a dead body on her way. 
When she returned to town, 
She was met by a clown, 
And that is the story of this play. \\ \vspace{0.1pt}

127: \textit{Mountain:-3.473}, Method: LimGen\\
There was a harsh woman named Maryann,
Who carved out her feelings for a man. 
She was like a fire, 
And with her desire, 
So it burned up and burst on the fan. \\ \vspace{0.1pt}

128: \textit{Mud:-3.016}, Method: LimGen\\
There was a lazy witch named Grace,
Who stuck a hot iron on her face. 
When she started to sweat, 
She was pushed by her pet, 
So she had to go down on the base. \\ \vspace{0.1pt}

129: \textit{Spider:-3.118}, Method: LimGen\\
There was a warrior named Marcell,
Who crawled a long distance on her tail. 
She was like a shadow, 
Which I saw in the snow, 
So I tried to climb down on the trail. \\ \vspace{0.1pt}

130: \textit{Rain:-3.015}, Method: LimGen\\
There was a harsh woman named Kay,
Who kept a close eye on our day. 
But the moment she came, 
She was shocked by her name, 
And she looked down and saw our way. \\ \vspace{0.1pt}

131: \textit{Memory:-2.776}, Method: LimGen\\
There was a wise grandma named Grace,
Who lost all her money in a case. 
She came back from the grave, 
She was able to save, 
And now she has a family face. \\ \vspace{0.1pt}

132: \textit{Season:-2.862}, Method: LimGen\\
There was a shy captain named Amal,
Who kept a close eye on her football. 
When it came to baseball, 
Which she played in the fall, 
She was happy to play and to call. \\ \vspace{0.1pt}

133: \textit{Winter:-2.939}, Method: LimGen\\
There was a quiet girl named Renee,
Who spent all her money in a day. 
When she went to midnight, 
Which she did in the night, 
She had enough to eat and to pay. \\ \vspace{0.1pt}

134: \textit{Throne:-3.088}, Method: LimGen\\
There was a fierce lady named Brande,
Who stood a great distance on her land. 
She was like a shadow, 
With the face of a crow, 
And her eyes were smaller and inland. \\ \vspace{0.1pt}

135: \textit{Politics:-3.006}, Method: LimGen\\
There was a professor named Renee,
Who learned a new language on her way. 
When she returned to mind, 
She was surprised to find, 
She was able to write and to play. \\ \vspace{0.1pt}

136: \textit{Promise:-3.019}, Method: LimGen\\
There was a lady named Kay,
Who did a great job on our way. 
Her parents were so kind, 
She was able to find, 
And that is the beauty of this day. \\ \vspace{0.1pt}

137: \textit{Bank:-2.949}, Method: LimGen\\
There was a smart farmer named Marquerite,
Who owned a small farm on our street. 
She would go to a store, 
And she said to the floor, 
You never can tell unless you eat. \\ \vspace{0.1pt}

138: \textit{Money:-3.144}, Method: LimGen\\
There was a lady named Maud,
Who lost all her money in a fraud. 
But her mother was right, 
She was saved by her light, 
So she went up and put on the rod. \\ \vspace{0.1pt}

139: \textit{Limerick:-4.039}, Method: LimGen\\
There was a writer named Celeste,
Who wright all his life in a contest. 
It was a satire, 
It would be a liar, 
It is a true story of a quest. \\ \vspace{0.1pt}

140: \textit{Beach:-3.049}, Method: LimGen\\
There was a bright girl named Bridgette,
Who stayed a long time on our street. 
She was like a girlfriend, 
We had the same boyfriend, 
But our lives were down to our feet. \\ \vspace{0.1pt}

141: \textit{Love:-2.967}, Method: LimGen\\
There was a funny girl named Renee,
Who did all her singing in a way. 
When she started to cry, 
She was afraid to die, 
So she tried to get down on the tray. \\ \vspace{0.1pt}

142: \textit{Cunning:-3.387}, Method: LimGen\\
There was a cunning witch named Lorelei,
Who fooled all her family in a lie. 
But her mother was blind, 
Her father was a mind, 
And that is the story of this guy. \\ \vspace{0.1pt}

143: \textit{Dog:-2.900}, Method: LimGen\\
There was a silly girl named Kai,
Who got a big crush on our guy. 
She wanted a boyfriend, 
He would have a girlfriend, 
And that is the beauty of this lie. \\ \vspace{0.1pt}

144: \textit{Blood:-3.042}, Method: LimGen\\
There was a cruel nurse named Nanette,
Who drank all her water in a sweat. 
When she returned to hell, 
She was able to tell, 
She saw that her husband was upset. \\ \vspace{0.1pt}

145: \textit{Death:-2.976}, Method: LimGen\\
There was a woman named Clare,
Who lived all her life in a nightmare. 
She came back from the grave, 
Which she found in the cave, 
And told her grandmother a prayer. \\ \vspace{0.1pt}

146: \textit{Disease:-3.290}, Method: LimGen\\
There was a nasty nurse named Tess,
Who caused a big mess on my progress. 
When I got to trial, 
I was shocked by her style, 
But I knew she was doing it less. \\ \vspace{0.1pt}

147: \textit{World:-2.939}, Method: LimGen\\
There was a lucky girl named Kay,
Who lost all her money in a day. 
She came back from the sea, 
And she said to the tree, 
I was afraid to come and to stay. \\ \vspace{0.1pt}

148: \textit{Planet:-3.028}, Method: LimGen\\
There was a wise lady named Nicole,
Who lived all her life within a hole. 
She was like a shadow, 
But she also was snow, 
And that is the beauty of this soul. \\ \vspace{0.1pt}

149: \textit{Fire:-3.153}, Method: LimGen\\
There was a loud woman named Kay,
Who put a big smile on our way. 
When we arrived to town, 
We were stopped by a clown, 
It was funny to see and to play. \\ \vspace{0.1pt}

150: \textit{Water:-2.982}, Method: LimGen\\
There was a bright cleaner named Dot,
Who put all her money in a pot. 
When she started to smoke, 
She was struck by a stroke, 
She has a severe case of a clot. \\ \vspace{0.1pt}

151: \textit{Love:-2.972}, Method: LimGen\\
There was a funny girl named Kay,
Who did all her singing in a way. 
When she started to cry, 
She was afraid to die, 
So she went up and put on the play. \\ \vspace{0.1pt}

152: \textit{Sports:-3.022}, Method: LimGen\\
There was a writer named Renee,
Who played a big role on our play. 
When we started to talk, 
She was ready to walk, 
She was eager to go and to stay. \\ \vspace{0.1pt}

153: \textit{Animal:-3.254}, Method: LimGen\\
There was a nasty girl named Kay,
Who made a big mess on our way. 
When we arrived to land, 
We were met by a band, 
We were able to talk and to play. \\ \vspace{0.1pt}

154: \textit{War:-2.673}, Method: LimGen\\
There was a warrior named Brande,
Who fought a great battle on her land. 
When she returned to fight, 
She was killed by a knight, 
And that is the story of this band. \\ \vspace{0.1pt}

155: \textit{Car:-3.200}, Method: LimGen\\
There was a smart girl named Lorelei,
Who took out her feelings for a guy. 
But her boyfriend was cool, 
So she went down the pool, 
So she got up and put on the tie. \\ \vspace{0.1pt}

156: \textit{Violent:-2.883}, Method: LimGen\\
There was a fierce woman named Lore,
Who killed all her family in a war. 
When she returned to hell, 
She was saved by a spell, 
And that is the basis of this lore. \\ \vspace{0.1pt}

157: \textit{Opera:-2.887}, Method: LimGen\\
There once was a dancer named Brande,
Who played a big part on our band. 
When we started to play, 
It was every day, 
And now it is a week beforehand. \\ \vspace{0.1pt}

158: \textit{Monster:-3.188}, Method: LimGen\\
There once was a witch named Claribel,
Who got all her power in a spell. 
She was like a shadow, 
She was able to grow, 
She was also the reason she fell. \\ \vspace{0.1pt}

159: \textit{Library:-2.734}, Method: LimGen\\
There was a neat teacher named Renee,
Who shared all her knowledge in a way. 
It was like a playground, 
It was the perfect sound, 
It was easy to learn and to play. \\ \vspace{0.1pt}

160: \textit{Market:-2.840}, Method: LimGen\\
There once was a farmer named Maile,
Who sold all her produce in a sale. 
When she returned to store, 
She was met by a door, 
And that is the story of this tale. \\ \vspace{0.1pt}

161: \textit{Doctor:-2.921}, Method: LimGen\\
There was a nervous nurse named Renee,
Who did a great job on our day. 
When we arrived to work, 
We were met by our clerk, 
So we got up and drove on the way. \\ \vspace{0.1pt}

162: \textit{Funeral:-2.879}, Method: LimGen\\
There was a brave nurse named Renee,
Who told a young girl on her birthday. 
When she returned to town, 
She was met by a clown, 
And that is the story of this play. \\ \vspace{0.1pt}

163: \textit{Smart:-2.959}, Method: LimGen\\
There was a wise lady named Kay,
Who put a big smile on our way. 
When we arrived to work, 
We were told by a clerk, 
We were welcome to come and to stay. \\ \vspace{0.1pt}

164: \textit{Ball:-2.899}, Method: LimGen\\
There was a lady named Nicolle,
Who threw all her money in a hole. 
It was like a baseball, 
And she hit to the wall, 
So she had to go down on the pole. \\ \vspace{0.1pt}

165: \textit{Body:-2.948}, Method: LimGen\\
There was a lady named Grace,
Who put a big smile on our face. 
When we arrived to work, 
We were met by a clerk, 
He instantly recognized our place. \\ \vspace{0.1pt}

166: \textit{Exercise:-3.055}, Method: LimGen\\
There once was a woman named Renee,
Who learned all her knowledge in a day. 
When she returned to work, 
She was told by a clerk, 
She was lucky to have and to stay. \\ \vspace{0.1pt}

167: \textit{Gun:-2.947}, Method: LimGen\\
There was a silly girl named Grace,
Who put a big smile on our face. 
She was a nobody, 
She was pretty to see, 
And she looked down and saw our place. \\ \vspace{0.1pt}

168: \textit{Art:-3.039}, Method: LimGen\\
There was a artist named Amal,
Who made a great painting on my wall. 
It was like a photo, 
It was the perfect flow, 
It was easy to read and to call. \\ \vspace{0.1pt}

169: \textit{Noble:-3.368}, Method: LimGen\\
There was a vain woman named Roseanne,
Who wished all her beauty in a man. 
But her husband was cruel, 
And she had to the school, 
So she had to live down on the plan. \\ \vspace{0.1pt}

170: \textit{Music:-2.784}, Method: LimGen\\
There was a loud dancer named Brande,
Who played a big part on our band. 
When we started to play, 
It was every day, 
And now it is a week beforehand. \\ \vspace{0.1pt}

171: \textit{Boxing:-2.888}, Method: LimGen\\
There was a fierce dancer named Celeste,
Who lost all her hair in a contest. 
When she returned to play, 
She was able to say, 
She was proud to be a female guest. \\ \vspace{0.1pt}

172: \textit{Philosophy:-2.987}, Method: LimGen\\
There was a wise teacher named Renee,
Who taught a great sermon on her way. 
When she returned to work, 
She was told by her clerk, 
She was ordered to leave and to stay. \\ \vspace{0.1pt}

173: \textit{Forest:-2.832}, Method: LimGen\\
There was a fierce farmer named Dayle,
Who hunted as she went on a trail. 
When she returned to town, 
She was met by a clown, 
And that is the story of this tale. \\ \vspace{0.1pt}

174: \textit{Night:-2.858}, Method: LimGen\\
There was a loud girl named Flor,
Who had a big smile on her before. 
But the moment they met, 
She was ready to get, 
So she had to go down on the floor. \\ \vspace{0.1pt}

175: \textit{Scary:-3.149}, Method: LimGen\\
There was a boring girl named Sabine,
Who seemed a good fit on our scene. 
When we started to talk, 
She was ready to walk, 
So we gave up and put on the screen. \\ \vspace{0.1pt}

176: \textit{Evil:-3.202}, Method: LimGen\\
There was a selfish witch named Roxanne,
Who thought out her feelings for a man. 
It was like a nightmare, 
It was painful to bear, 
It was frightening to think and to can. \\ \vspace{0.1pt}

177: \textit{Pride:-3.364}, Method: LimGen\\
There was a vain lady named Nicole,
Who felt a great longing on her soul. 
She wanted to enjoy, 
It was the perfect joy, 
But she knew she was losing him whole. \\ \vspace{0.1pt}

178: \textit{Angry:-3.292}, Method: LimGen\\
There was a fierce lady named Lorelei,
Who shouted as she went on a cry. 
When she came to someone, 
She was told by her son, 
He said that his mother was nearby. \\ \vspace{0.1pt}

179: \textit{Law:-3.199}, Method: LimGen\\
There was a harsh teacher named Grace,
Who sought out her students for a case. 
When she arrived to school, 
She was met by a pool, 
So she went to get down on the base. \\ \vspace{0.1pt}

180: \textit{Light:-3.306}, Method: LimGen\\
There was a harsh girl named Amal,
Who made a big mess on our wall. 
It was like a rainbow, 
And in our photo, 
In seconds we were all in the hall. \\ \vspace{0.1pt}

181: \textit{School:-2.513}, Method: LimGen\\
There was a shy girl named Lenore,
Who had a big smile on her before. 
When she started to talk, 
She was able to walk, 
So she had to sit down on the floor. \\ \vspace{0.1pt}

182: \textit{Rich:-2.992}, Method: LimGen\\
There was a smart farmer named Aline,
Who made a small fortune on her wine. 
When she returned to sea, 
She was able to flee, 
And that is the story of this line. \\ \vspace{0.1pt}

183: \textit{Creativity:-3.188}, Method: LimGen\\
There was a designer named Renee,
Who shared all her knowledge in a way. 
When she started to share, 
It was easy to care, 
Because she was sharing her birthday. \\ \vspace{0.1pt}

184: \textit{Leader:-2.842}, Method: LimGen\\
There was a lieutenant named Kay,
Who met a young woman on her way. 
She was a musician, 
She was on a mission, 
And that is the beauty of this day. \\ \vspace{0.1pt}

185: \textit{Color:-2.977}, Method: LimGen\\
There was a chunky girl named Grace,
Who used a red lipstick on her face. 
It looked like a rainbow, 
But was a black shadow, 
And that is the color of this place. \\ \vspace{0.1pt}

186: \textit{Park:-2.993}, Method: LimGen\\
There was a lively girl named Renee,
Who drove a white van on our way. 
When we arrived to town, 
We were met by a clown, 
Then we found him hiding in the hay. \\ \vspace{0.1pt}

187: \textit{Loss:-3.052}, Method: LimGen\\
There was a wise woman named Renee,
Who helped a poor widow on her way. 
When she returned to fight, 
She was killed by a knight, 
But she survived his arrows and lay. \\ \vspace{0.1pt}

188: \textit{Airplane:-3.280}, Method: LimGen\\
There was a captain named Grace,
Who blew all her money in a chase. 
When she returned to shore, 
She was met by a door, 
So she quickly left on the staircase. \\ \vspace{0.1pt}

189: \textit{Weight:-3.161}, Method: LimGen\\
There was a nervous girl named Chin,
Who put a big smile on our skin. 
She was back from the break, 
She was ready to take, 
And that is the beauty of this spin. \\ \vspace{0.1pt}

190: \textit{Useful:-3.242}, Method: LimGen\\
There was a neat cleaner named Dot,
Who put a big smile on our lot. 
When we arrived to work, 
We were met by our clerk, 
And greeted with a polite onslaught. \\ \vspace{0.1pt}

191: \textit{Union:-3.047}, Method: LimGen\\
There was a fierce lawyer named Sharon,
Who sought out her parents for a loan. 
When they refused to sign, 
She was on a deadline, 
So she had to go down on the bone. \\ \vspace{0.1pt}

192: \textit{Child:-2.898}, Method: LimGen\\
There was a selfish girl named Susanne,
Who put all her money in a man. 
It was for her birthday, 
It was the perfect day, 
Then she heard him crying in the van. \\ \vspace{0.1pt}

193: \textit{Home:-2.992}, Method: LimGen\\
There was a neat grandma named Dot,
Who had all her money in a lot. 
She was back from the store, 
And she was to the door, 
And she looked down and saw our spot. \\ \vspace{0.1pt}

194: \textit{Working:-2.928}, Method: LimGen\\
There was a lucky nurse named Dot,
Who did a great job on our lot. 
Our neighbors were so kind, 
We were able to find, 
And that is the beauty of this spot. \\ \vspace{0.1pt}

195: \textit{Cheat:-3.151}, Method: LimGen\\
There once was a liar named Renee,
Who put all her money in a play. 
It was for her boyfriend, 
And she got to the end, 
And now she has a family day. \\ \vspace{0.1pt}

196: \textit{Fall:-3.172}, Method: LimGen\\
There was a wise girl named Kay,
Who did all her sewing in a day. 
She would go to a place, 
She would make a staircase, 
She was sure to have a good birthday. \\ \vspace{0.1pt}

197: \textit{Time:-2.865}, Method: LimGen\\
There was a woman named Renee,
Who did all her sewing in a day. 
When she returned to work, 
She was told by a clerk, 
She was ordered to sew and to pay. \\ \vspace{0.1pt}

198: \textit{Applaud:-3.590}, Method: LimGen\\
There was a polite judge named Dede,
Who wished a good day on her indeed. 
But the moment she heard, 
She was struck by his word, 
And she fell down and began her deed. \\ \vspace{0.1pt}

199: \textit{Hope:-3.103}, Method: LimGen\\
There was a lucky girl named Renee,
Who got all her money in a way. 
She was a nobody, 
She was raised by a tree, 
And she went down and had her birthday. \\ \vspace{0.1pt}

200: \textit{Flower:-3.019}, Method: LimGen\\
There was a neat lady named Kay,
Who cut a sweet smile on my birthday. 
She was like a fairy, 
Though a little scary, 
So I tried to be down on the day. \\ \vspace{0.1pt}

201: \textit{Random:-3.595}, Method: LimGen\\
There was a lady named Lise,
Who happened on one of our guys. 
She was a nobody, 
And she was to the tree, 
And she was down and got our prize. \\ \vspace{0.1pt}

202: \textit{Impressive:-3.354}, Method: LimGen\\
There was a neat artist named Dot,
Who helped out her parents for a lot. 
Her parents were so kind, 
She was able to find, 
As her brother and sister cannot. \\ \vspace{0.1pt}

203: \textit{River:-2.844}, Method: LimGen\\
There was a brave farmer named Jerrell,
Who crossed a dead body on his trail. 
When he returned to town, 
He was chased by a clown, 
And drove home to his mother in jail. \\ \vspace{0.1pt}

204: \textit{Christmas:-3.066}, Method: LimGen\\
There was a silly boy named Claudio,
Who got a good deal on his photo. 
It was for his birthday, 
He was able to pay, 
But I am not sure for tomorrow. \\ \vspace{0.1pt}

205: \textit{Alien:-2.977}, Method: LimGen\\
There was a warrior named Theodore,
Who captured an enemy of war. 
When he returned to fight, 
He was struck by a light, 
And he fell down and killed his mentor. \\ \vspace{0.1pt}

206: \textit{Fiance:-3.085}, Method: LimGen\\
There was a shy grandpa named Jake,
Who loved a good story on his cake. 
It was for his birthday, 
It was the perfect day, 
And he went down and ordered his steak. \\ \vspace{0.1pt}

207: \textit{Injury:-2.965}, Method: LimGen\\
There was a doctor named Marquis,
Who healed a young lady on her knee. 
He was a physician, 
He was on a mission, 
And that is the story of this tree. \\ \vspace{0.1pt}

208: \textit{Dawn:-3.207}, Method: LimGen\\
There was a fierce man named Salvador,
Who lit a small fire on his shore. 
When he returned to sea, 
He was ordered to flee, 
And he did not like hearing of war. \\ \vspace{0.1pt}

209: \textit{Thanksgiving:-2.941}, Method: LimGen\\
There was a lucky chef named Dwight,
Who cooked a great meal on our night. 
It was for my birthday, 
It was the perfect day, 
And that is the reason of this site. \\ \vspace{0.1pt}

210: \textit{Holiday:-3.038}, Method: LimGen\\
There was a lively chef named Kip,
Who spent a long time on our trip. 
When we returned to town, 
We saw the old playground, 
And that is the center of this strip. \\ \vspace{0.1pt}

211: \textit{Wedding:-2.925}, Method: LimGen\\
There was a tailor named Kurt,
Who wore a red jacket on his shirt. 
When he returned to town, 
He was chased by a clown, 
And he fell down and broke his turret. \\ \vspace{0.1pt}

212: \textit{Traffic:-3.005}, Method: LimGen\\
There was a general named Blaine,
Who drove all his family in a train. 
He worked on the railroad, 
And he went to the road, 
And he came down and started his plane. \\ \vspace{0.1pt}

213: \textit{Musuem:-3.149}, Method: LimGen\\
There was a blacksmith named Pete,
Who housed a small shop on our street. 
He worked on the railroad, 
And he kept to the road, 
And he went down and bought our wheat. \\ \vspace{0.1pt}

214: \textit{Kindness:-3.316}, Method: LimGen\\
There was a selfish man named Cole,
Who loved a young woman on his soul. 
When he came to someone, 
He would take a shotgun, 
And that is the story of this role. \\ \vspace{0.1pt}

215: \textit{Birthday:-2.912}, Method: LimGen\\
There was a lucky boy named Kip,
Who got a free ride on our trip. 
He asked for his photo, 
He was happy to go, 
And he came down and took our tip. \\ \vspace{0.1pt}

216: \textit{Heartbreak:-2.830}, Method: LimGen\\
There once was a soldier named Mel,
Who overcame an onslaught of hell. 
He came back from the grave, 
And he went to the cave, 
And he sat down and opened his cell. \\ \vspace{0.1pt}

217: \textit{Wine:-2.932}, Method: LimGen\\
There once was a waiter named Cole,
Who drank all his money in a bowl. 
When he returned to light, 
He was shocked by his sight, 
And he fell down and broke his console. \\ \vspace{0.1pt}

218: \textit{Memory:-3.110}, Method: LimGen\\
There was a wise grandpa named Chase,
Who lost all his money in a case. 
He came back from the grave, 
Bought the family cave, 
And started with a different face. \\ \vspace{0.1pt}

219: \textit{Mountain:-3.155}, Method: LimGen\\
There once was a man named Brock,
Who climbed a great mountain on his rock. 
He came back from the sea, 
And he said to the tree, 
I went through the water and got stock. \\ \vspace{0.1pt}

220: \textit{Pillow:-3.030}, Method: LimGen\\
There was a bright boy named Chase,
Who felt a strange feeling on his face. 
It was like a rainbow, 
It was the perfect glow, 
And he looked down and saw his birthplace. \\ \vspace{0.1pt}

221: \textit{Beer:-2.674}, Method: LimGen\\
There was a funky chef named Dwight,
Who cooked a great meal on our night. 
We got back from the bar, 
And we walked to the car, 
And we sat down and had our bite. \\ \vspace{0.1pt}

222: \textit{Tears:-2.728}, Method: LimGen\\
There was a nervous boy named Chase,
Who felt a strange feeling on his face. 
When he started to cry, 
He was chased by a guy, 
And he fell down and covered his place. \\ \vspace{0.1pt}

223: \textit{Surprise:-2.756}, Method: LimGen\\
There was a lucky boy named Dwight,
Who did a great job on our night. 
We got back from the show, 
We were ready to go, 
We knew that our schedule was tight. \\ \vspace{0.1pt}

224: \textit{Shaken:-3.223}, Method: LimGen\\
There was a fierce waiter named Jess,
Who poured a cold beer on our mess. 
When he returned to knock, 
He was met by a rock, 
And that is the end of this process. \\ \vspace{0.1pt}

225: \textit{Humiliation:-3.086}, Method: LimGen\\
There was a harsh bully named Chase,
Who forced a young woman on her face. 
When she refused to scream, 
She was struck by a beam, 
And died on the medical staircase. \\ \vspace{0.1pt}

226: \textit{Laugh:-3.699}, Method: LimGen\\
There was a silly man named Chase,
Who knew a good story on his face. 
He was a nobody, 
And he looked to the sea, 
He saw it and had visions and space. \\ \vspace{0.1pt}

227: \textit{Victory:-2.861}, Method: LimGen\\
There was a fierce man named Chase,
Who fought a great battle on our place. 
He was back from the war, 
And he came to the door, 
He looked through the window and saw ace. \\ \vspace{0.1pt}

228: \textit{Mud:-3.141}, Method: LimGen\\
There once was a man named Cole,
Who spilled all his money in a hole. 
When he returned to land, 
He was met by a band, 
But they were his enemies and stole. \\ \vspace{0.1pt}

229: \textit{Restore:-2.950}, Method: LimGen\\
There was a general named Stan,
Who lost all his money in a plan. 
He decided to run, 
And he ran to the sun, 
He was proud to be a chinese man. \\ \vspace{0.1pt}

230: \textit{Spider:-3.354}, Method: LimGen\\
There was a clever boy named Jed,
Who crawled a long distance on his head. 
He was like a shadow, 
But had a long torso, 
And he looked down and saw our bed. \\ \vspace{0.1pt}

231: \textit{Money:-3.097}, Method: LimGen\\
There was a greedy man named Todd,
Who lost all his money in a fraud. 
When he returned to work, 
He was robbed by his clerk, 
And never could buy a cod. \\ \vspace{0.1pt}

232: \textit{Season:-2.573}, Method: LimGen\\
There was a shy actor named Dario,
Who played a big role on our show. 
He came back from the break, 
And we went to the lake, 
And he sat down and took his photo. \\ \vspace{0.1pt}

233: \textit{Beach:-2.972}, Method: LimGen\\
There was a lively man named Theodore,
Who stayed a long time on our shore. 
He was on the lookout, 
And he came to the scout, 
And he went down and saw our store. \\ \vspace{0.1pt}

234: \textit{Rain:-3.129}, Method: LimGen\\
There was a quiet boy named Nathanael,
Who kept a close eye on our trail. 
He was back from the sea, 
And he was to the tree, 
And he came down and took our tail. \\ \vspace{0.1pt}

235: \textit{Winter:-3.030}, Method: LimGen\\
There was a bright boy named Les,
Who wore a red jacket on his dress. 
He was back from the sea, 
He was happy to see, 
He was glad to have a new address. \\ \vspace{0.1pt}

236: \textit{Blood:-3.082}, Method: LimGen\\
There was a cruel man named Cole,
Who caused a great evil on my soul. 
He was a physician, 
He was on a mission, 
He went through the temple and found coal. \\ \vspace{0.1pt}

237: \textit{Politics:-2.912}, Method: LimGen\\
There was a general named Chase,
Who learned a great deal on our race. 
He was back from the war, 
And he came to the store, 
And he went down and saw our place. \\ \vspace{0.1pt}

238: \textit{Promise:-3.373}, Method: LimGen\\
There was a humble boy named Scot,
Who did all his work within a thought. 
He was a nobody, 
He was born by a tree, 
And now he has a family plot. \\ \vspace{0.1pt}

239: \textit{Bank:-2.677}, Method: LimGen\\
There was a greedy man named Pete,
Who owned a small shop on our street. 
He worked on the railroad, 
And he came to the road, 
And he went down and bought our wheat. \\ \vspace{0.1pt}

240: \textit{War:-2.895}, Method: LimGen\\
There was a brave soldier named Saul,
Who fought a great battle on his fall. 
When he returned to fight, 
He was killed by a knight, 
And that is the reason of this wall. \\ \vspace{0.1pt}

241: \textit{Disease:-3.223}, Method: LimGen\\
There was a doctor named Duane,
Who caused a big problem on my brain. 
When I got to trial, 
I was shocked by his style, 
But I knew he was doing it plain. \\ \vspace{0.1pt}

242: \textit{Throne:-2.869}, Method: LimGen\\
There was a vain man named Javier,
Who stood all his life in a prayer. 
He came back from the war, 
And he went to the store, 
And he sat down and opened his share. \\ \vspace{0.1pt}

243: \textit{Dog:-2.804}, Method: LimGen\\
There was a bully named Dane,
Who got a free ride on our train. 
When he started to walk, 
He was stopped by a rock, 
And he fell down and shattered his brain. \\ \vspace{0.1pt}

244: \textit{Cunning:-3.317}, Method: LimGen\\
There was a magician named Nick,
Who fooled all his family in a trick. 
When he returned to hide, 
He was found by his bride, 
And killed with a magical lipstick. \\ \vspace{0.1pt}

245: \textit{Planet:-3.412}, Method: LimGen\\
There was a cruel man named Hugh,
Who lived a long time on my into. 
He was back from the war, 
He had been by my door, 
He said that his family was new. \\ \vspace{0.1pt}

246: \textit{World:-2.747}, Method: LimGen\\
There once was a man named Theodore,
Who lost all his money in a war. 
When he returned to fight, 
He was killed by a knight, 
And that is the reason of this lore. \\ \vspace{0.1pt}

247: \textit{Love:-3.032}, Method: LimGen\\
There was a honest man named Scot,
Who did a good job on our lot. 
He would go to a place, 
He would find a staircase, 
And that is the secret of this spot. \\ \vspace{0.1pt}

248: \textit{Death:-3.145}, Method: LimGen\\
There was a cruel judge named Lyle,
Who killed a young girl on his trial. 
It was like a nightmare, 
I was scared by his stare, 
But I knew his intentions and smile. \\ \vspace{0.1pt}

249: \textit{Water:-3.272}, Method: LimGen\\
There was a harsh cleaner named Burt,
Who covered an area of dirt. 
When he started to spray, 
He was struck by a ray, 
But I think that it probably hurt. \\ \vspace{0.1pt}

250: \textit{Sports:-3.003}, Method: LimGen\\
There was a smart boxer named Saul,
Who put all his money in a ball. 
It was like a football, 
And it was to the wall, 
And he got down and threw his baseball. \\ \vspace{0.1pt}

251: \textit{Limerick:-3.929}, Method: LimGen\\
There was a grandpa named Jerrell,
Who hearted as he passed on a tale. 
He went back from the inn, 
Took two bottles of gin, 
And started with a little detail. \\ \vspace{0.1pt}

252: \textit{Fire:-2.946}, Method: LimGen\\
There was a loud soldier named Salvador,
Who blew a big whistle on my door. 
He was back from the war, 
And he came to the store, 
He went through the window and said more. \\ \vspace{0.1pt}

253: \textit{Love:-3.112}, Method: LimGen\\
There was a jealous man named Scot,
Who put all his money in a lot. 
When he wanted to share, 
He would say a prayer, 
It was easy to do and to got. \\ \vspace{0.1pt}

254: \textit{Car:-3.082}, Method: LimGen\\
There was a funny boy named Pete,
Who ran a fish market on my street. 
He was on the railroad, 
So he was down the road, 
He saw me and said thanks and upbeat. \\ \vspace{0.1pt}

255: \textit{Animal:-2.859}, Method: LimGen\\
There was a farmer named Pete,
Who made a huge profit on his meat. 
When he returned to mind, 
He was surprised to find, 
He was able to walk and to eat. \\ \vspace{0.1pt}

256: \textit{Doctor:-2.605}, Method: LimGen\\
There was a dentist named Dane,
Who did a great job on our brain. 
He was a physician, 
He was on a mission, 
And he came down and saw our pain. \\ \vspace{0.1pt}

257: \textit{Opera:-2.775}, Method: LimGen\\
There was a lame artist named Romeo,
Who played a big role on our show. 
He was a musician, 
He was on a mission, 
He was willing to work and to grow. \\ \vspace{0.1pt}

258: \textit{Monster:-3.288}, Method: LimGen\\
There was a stupid boy named Javier,
Who got a high score on his nightmare. 
He went back from the dream, 
And it was to the team, 
And he came down and gave his prayer. \\ \vspace{0.1pt}

259: \textit{Noble:-3.385}, Method: LimGen\\
There was a wise man named Cole,
Who wished a good morning on his soul. 
He was back from the war, 
And he knew to the core, 
He was ready to fight and to roll. \\ \vspace{0.1pt}

260: \textit{Body:-2.643}, Method: LimGen\\
There was a nervous man named Chase,
Who put a big smile on our face. 
We got back from the break, 
And we went to the lake, 
And we sat down and took our place. \\ \vspace{0.1pt}

261: \textit{Market:-3.118}, Method: LimGen\\
There was a wise farmer named Chase,
Who bought a small farm on our place. 
When he started to shop, 
He was able to stop, 
And he came down and saw our space. \\ \vspace{0.1pt}

262: \textit{Smart:-3.231}, Method: LimGen\\
There was a clever boy named Jess,
Who put a great deal on his impress. 
He started like a kid, 
Did the things that he did, 
And that is the end of this process. \\ \vspace{0.1pt}

263: \textit{Ball:-3.037}, Method: LimGen\\
There was a lucky boy named Cole,
Who threw all his money in a hole. 
It was like a baseball, 
And he hit to the wall, 
And now he has a broken console. \\ \vspace{0.1pt}

264: \textit{Library:-3.432}, Method: LimGen\\
There was a smart teacher named Brock,
Who used a black board on our block. 
He would talk to a class, 
I was able to pass, 
And it was still pretty intense shock. \\ \vspace{0.1pt}

265: \textit{Funeral:-2.925}, Method: LimGen\\
There once was a soldier named Theodore,
Whose father died a hero in war. 
When he returned to town, 
He was met by a clown, 
Then he heard him singing in the store. \\ \vspace{0.1pt}

266: \textit{Exercise:-3.173}, Method: LimGen\\
There was a lazy judge named Brock,
Who learned a hard lesson on his walk. 
He was on the program, 
He was on a programme, 
He was ready to go and to talk. \\ \vspace{0.1pt}

267: \textit{Art:-2.714}, Method: LimGen\\
There was a artist named Cole,
Who made a huge impact on my soul. 
He was a musician, 
He was on a mission, 
And that is the beauty of this role. \\ \vspace{0.1pt}

268: \textit{Music:-3.003}, Method: LimGen\\
There was a funky boy named Beau,
Who played a big role on our show. 
He was on the program, 
He was on a programme, 
He basically was our shadow. \\ \vspace{0.1pt}

269: \textit{Philosophy:-3.097}, Method: LimGen\\
There was a teacher named Jess,
Who taught a short course on my progress. 
When I returned to school, 
I was struck by his cool, 
And I went down and got his address. \\ \vspace{0.1pt}

270: \textit{Gun:-2.616}, Method: LimGen\\
There was a loud boy named Chase,
Who put a big smile on our face. 
He came back from the war, 
And he went to the store, 
And he looked down and saw our place. \\ \vspace{0.1pt}

271: \textit{Boxing:-2.523}, Method: LimGen\\
There was a boxer named Dwight,
Who lost all his money in a fight. 
When he tried to retire, 
He was killed by a fire, 
And that is the story of this knight. \\ \vspace{0.1pt}

272: \textit{Scary:-3.309}, Method: LimGen\\
There was a funny boy named Joaquin,
Who seemed a good fit on our scene. 
He was like a nightmare, 
He had the perfect hair, 
He was through the roof and was fifteen. \\ \vspace{0.1pt}

273: \textit{Creativity:-3.216}, Method: LimGen\\
There once was a teacher named Jess,
Who learned a great deal on his process. 
When he returned to work, 
He took the same framework, 
But he changed his methods and address. \\ \vspace{0.1pt}

274: \textit{Forest:-3.036}, Method: LimGen\\
There was a wise farmer named Nathanael,
Who hunted as he went on a trail. 
When he returned to town, 
He was chased by a clown, 
And lost her because she was female. \\ \vspace{0.1pt}

275: \textit{Violent:-2.801}, Method: LimGen\\
There was a cruel boy named Theodore,
Whose father killed a woman in war. 
He came back from the grave, 
And he went to the cave, 
And he sat down and opened his door. \\ \vspace{0.1pt}

276: \textit{Night:-2.819}, Method: LimGen\\
There was a loud man named Claudio,
Who did a great job on our show. 
He came back from the break, 
And we got to the lake, 
So we had to get down on the snow. \\ \vspace{0.1pt}

277: \textit{Pride:-3.142}, Method: LimGen\\
There was a humble boy named Cole,
Who loved a good story on his soul. 
It was a tradition, 
He was on a mission, 
He was ready to learn and to roll. \\ \vspace{0.1pt}

278: \textit{Evil:-3.114}, Method: LimGen\\
There was a warrior named Javier,
Who thought as he did on a nightmare. 
He came back from the grave, 
And he went to the cave, 
And he fell asleep again elsewhere. \\ \vspace{0.1pt}

279: \textit{Law:-3.413}, Method: LimGen\\
There was a wise lawyer named Lyle,
Who brought out his lawyers for a trial. 
He was back from the war, 
And he was to the fore, 
But he is now set in his exile. \\ \vspace{0.1pt}

280: \textit{Angry:-3.207}, Method: LimGen\\
There was a rude boy named Dwight,
Who shouted as he took on a fight. 
When he tried to protest, 
He was told by his guest, 
He was welcome to stay and to write. \\ \vspace{0.1pt}

281: \textit{Light:-2.905}, Method: LimGen\\
There was a harsh cleaner named Erwin,
Who made a big difference on my skin. 
When I started to shine, 
My face became so fine, 
I noticed that my makeup looked thin. \\ \vspace{0.1pt}

282: \textit{School:-2.957}, Method: LimGen\\
There was a shy teacher named Abram,
Who did a great job on our program. 
He was like a mentor, 
And he was to the core, 
He totally knew our programme. \\ \vspace{0.1pt}

283: \textit{Rich:-3.245}, Method: LimGen\\
There was a bright farmer named Erwin,
Who made a huge profit on his skin. 
He was back from the sea, 
He was ready to flee, 
But he knew he was losing it thin. \\ \vspace{0.1pt}

284: \textit{Leader:-3.020}, Method: LimGen\\
There was a lieutenant named Ted,
Who led a small army on his head. 
When he returned to fight, 
He was killed by a knight, 
But he survived his battles and fled. \\ \vspace{0.1pt}

285: \textit{Loss:-3.168}, Method: LimGen\\
There once was a doctor named Jamal,
Who helped a young woman on her fall. 
When she returned to fight, 
She was met by a light, 
And she fell down and broke her baseball. \\ \vspace{0.1pt}

286: \textit{Color:-2.996}, Method: LimGen\\
There was a bright cleaner named Chase,
Who used a hot iron on my face. 
When I tried to object, 
He said the same effect, 
But it does not happen in my case. \\ \vspace{0.1pt}

287: \textit{Weight:-2.739}, Method: LimGen\\
There was a wise boxer named Dewitt,
Who lost all his money in a fit. 
When he returned to work, 
He was told by a clerk, 
He was ordered to leave and to quit. \\ \vspace{0.1pt}

288: \textit{Park:-2.890}, Method: LimGen\\
There was a funny boy named Pete,
Who drove a white van on our street. 
He came back from the store, 
And I went to the door, 
And that is the story of this beat. \\ \vspace{0.1pt}

289: \textit{Home:-2.821}, Method: LimGen\\
There was a lucky man named Dwight,
Who lost all his money in a night. 
When he returned to work, 
He was told by a clerk, 
That no payment was due but midnight. \\ \vspace{0.1pt}

290: \textit{Useful:-2.994}, Method: LimGen\\
There was a smart doctor named Scot,
Who found a dead body on his lot. 
When he returned to work, 
He was told by a clerk, 
He looked through the window and saw shot. \\ \vspace{0.1pt}

291: \textit{Applaud:-3.197}, Method: LimGen\\
There was a wise bully named Dwight,
Who wished a good time on his invite. 
He wanted to impress, 
So he turned down the dress, 
But he thought he was doing it right. \\ \vspace{0.1pt}

292: \textit{Union:-3.007}, Method: LimGen\\
There was a fierce teacher named Dwight,
Who sought out his students for a fight. 
When they arrived to school, 
They were met by a pool, 
And that is the story of this night. \\ \vspace{0.1pt}

293: \textit{Airplane:-2.991}, Method: LimGen\\
There was a loud captain named Kip,
Who blew a big whistle on his ship. 
When he returned to shore, 
He was met by a door, 
And he went down and opened its lip. \\ \vspace{0.1pt}

294: \textit{Child:-3.133}, Method: LimGen\\
There was a doctor named Pierre,
Who cared a great deal on my welfare. 
When I returned to school, 
I was struck by his cool, 
He was able to talk and to care. \\ \vspace{0.1pt}

295: \textit{Working:-2.960}, Method: LimGen\\
There was a smart teacher named Wes,
Who did a great job on my progress. 
I learned on the way, 
I was able to play, 
I got myself down in the process. \\ \vspace{0.1pt}

296: \textit{Fall:-2.784}, Method: LimGen\\
There was a lucky man named Chase,
Who did a great job on our place. 
We got back from the show, 
We were ready to go, 
And that is the story of this case. \\ \vspace{0.1pt}

297: \textit{Cheat:-3.006}, Method: LimGen\\
There was a bully named Rick,
Who put a hot iron on his stick. 
When he started to cry, 
He was struck by a fly, 
But he said he was taking it quick. \\ \vspace{0.1pt}

298: \textit{Time:-2.829}, Method: LimGen\\
There was a wise doctor named Chase,
Who kept a close eye on our place. 
When we arrived to work, 
We were met by our clerk, 
And we sat down and made our case. \\ \vspace{0.1pt}

299: \textit{Hope:-2.907}, Method: LimGen\\
There was a stupid boy named Wes,
Who did a great job on my progress. 
I got back from the break, 
And I went to the lake, 
And I sat down and wrote my address. \\ \vspace{0.1pt}

300: \textit{Flower:-2.988}, Method: LimGen\\
There was a funky boy named Saul,
Who cut a nice figure on my wall. 
It was for his birthday, 
It was the perfect day, 
And he came down and played his football. \\ \vspace{0.1pt}

301: \textit{Random:-3.162}, Method: LimGen\\
There was a general named Scot,
Who filled a small office on our lot. 
When we arrived to talk, 
We were met by a knock, 
But he said he was taking it hot. \\ \vspace{0.1pt}

302: \textit{Impressive:-3.412}, Method: LimGen\\
There was a bright man named Hugh,
Who showed a great deal on his debut. 
He got on the record, 
And it was to the board, 
And it was not good coaching review. \\ \vspace{0.1pt}

303: \textit{Musuem:-3.573}, Method: LimGen\\
There was a blacksmith named Bridgette,
Who housed a small cottage on her street. 
She was like a statue, 
She was the perfect view, 
She was up in heaven and concrete. \\ \vspace{0.1pt}

304: \textit{Dawn:-2.862}, Method: LimGen\\
There was a warrior named Rose,
Who slept on a mountain of shadows. 
When she awoke to light, 
She was shocked by a sight, 
And she fell down and covered her nose. \\ \vspace{0.1pt}

305: \textit{Memory:-3.209}, Method: LimGen\\
There was a wise grandma named Lorraine,
Who used a hot iron on her brain. 
It was like a process, 
It was so much progress, 
She thought that her mother was insane. \\ \vspace{0.1pt}

306: \textit{Alien:-2.758}, Method: LimGen\\
There was a warrior named Brande,
Who captured an area of land. 
When she began to fight, 
She was struck by a light, 
And she fell down and wounded her hand. \\ \vspace{0.1pt}

307: \textit{Heartbreak:-3.019}, Method: LimGen\\
There once was a girl named Cher,
Who cried all her life in a nightmare. 
When she started to cry, 
Her mother told a lie, 
She said that her daughter was elsewhere. \\ \vspace{0.1pt}

308: \textit{Traffic:-3.256}, Method: LimGen\\
There was a smart judge named Marguerite,
Who stopped a drunk driver on my street. 
She asked for my address, 
I gave the right access, 
And she got down and started her beat. \\ \vspace{0.1pt}

309: \textit{Pillow:-3.319}, Method: LimGen\\
There was a chunky girl named Grace,
Who felt a strange presence on her face. 
She looked like a fairy, 
She was on a ferry, 
She was up in paradise and space. \\ \vspace{0.1pt}

310: \textit{Injury:-3.033}, Method: LimGen\\
There was a surgeon named Geri,
Who healed a gunshot wound on her knee. 
When she returned to fight, 
She was shocked by her sight, 
And she fell down and broke her sunday. \\ \vspace{0.1pt}

311: \textit{Wine:-3.225}, Method: LimGen\\
There was a waitress named Kay,
Who served a great meal on our day. 
It was a tradition, 
We were on a mission, 
And it was not easy work sunday. \\ \vspace{0.1pt}

312: \textit{Christmas:-3.134}, Method: LimGen\\
There was a silly girl named Renee,
Who got a black eye on her birthday. 
It was like a rainbow, 
And she went to the show, 
She walked through the crowd and cried okay. \\ \vspace{0.1pt}

313: \textit{Thanksgiving:-3.147}, Method: LimGen\\
There once was a lady named Kay,
Who ate a hot dog on her birthday. 
When she started to cry, 
It was the perfect guy, 
And she fell asleep quickly sunday. \\ \vspace{0.1pt}

314: \textit{Fiance:-2.969}, Method: LimGen\\
There was a shy waitress named Kai,
Who talked as she waited on a guy. 
When she started to flirt, 
It was enough to hurt, 
But she thought she was getting him high. \\ \vspace{0.1pt}

315: \textit{Shaken:-3.225}, Method: LimGen\\
There was a loud waitress named Tess,
Who poured a cold beer on our mess. 
When we arrived to stand, 
We were met by her hand, 
And she sat down and opened her dress. \\ \vspace{0.1pt}

316: \textit{Holiday:-3.311}, Method: LimGen\\
There was a lucky girl named Renee,
Who stayed as she was on a birthday. 
It was like a spring, 
It was the perfect thing, 
It was nice to have a big buffet. \\ \vspace{0.1pt}

317: \textit{Kindness:-3.031}, Method: LimGen\\
There once was a teacher named Kay,
Who learned a new language on her way. 
When she returned to mind, 
She was surprised to find, 
She was able to talk and to play. \\ \vspace{0.1pt}

318: \textit{River:-3.370}, Method: LimGen\\
There once was a woman named Louise,
Who wandered on a mountain of seas. 
She came back from the sea, 
Took shelter of that tree, 
And she sat down and opened her trees. \\ \vspace{0.1pt}

319: \textit{Birthday:-2.971}, Method: LimGen\\
There once was a lady named Renee,
Who gave all her money in a day. 
It was like a contest, 
And it was to the west, 
So we had to go down on the way. \\ \vspace{0.1pt}

320: \textit{Tears:-2.827}, Method: LimGen\\
There was a vain lady named Grace,
Who felt a strange feeling on her face. 
When she started to cry, 
She was afraid to die, 
But she does not suffer in her place. \\ \vspace{0.1pt}

321: \textit{Surprise:-3.031}, Method: LimGen\\
There was a shy lady named Kay,
Who did a great job on my birthday. 
She came back from the break, 
And we went to the lake, 
Was totally a different day. \\ \vspace{0.1pt}

322: \textit{Humiliation:-3.146}, Method: LimGen\\
There was a lady named Grace,
Who faced a big problem on her face. 
She decided to cry, 
And she cried to the sky, 
It was easy to see and to trace. \\ \vspace{0.1pt}

323: \textit{Beer:-3.197}, Method: LimGen\\
There was a silly chef named Kay,
Who ate all her dinner in a day. 
She was a potato, 
But had a nice torso, 
So she got up and slept on the tray. \\ \vspace{0.1pt}

324: \textit{Mud:-3.405}, Method: LimGen\\
There was a chunky witch named Bok,
Who stuck out her fingers for a rock. 
It was like a playground, 
And it was to the ground, 
And that is the beauty of this walk. \\ \vspace{0.1pt}

325: \textit{Restore:-3.043}, Method: LimGen\\
There was a wise cleaner named In,
Who tried a new method on her skin. 
When she returned to work, 
She was told by her clerk, 
She was ordered to strip and to spin. \\ \vspace{0.1pt}

326: \textit{Wedding:-2.883}, Method: LimGen\\
There was a tailor named Rose,
Who decided on one of my clothes. 
I got back from the shop, 
And I went to the top, 
And I looked down and noticed my nose. \\ \vspace{0.1pt}

327: \textit{Victory:-2.781}, Method: LimGen\\
There was a lieutenant named Grace,
Who fought a great battle on my place. 
She was back from the war, 
And she came to the door, 
And she sat down and opened her face. \\ \vspace{0.1pt}

328: \textit{Laugh:-3.118}, Method: LimGen\\
There was a loud girl named Grace,
Who smiled a big smile on our face. 
I noticed on the way, 
She was stopped by a tray, 
And she looked down and saw our place. \\ \vspace{0.1pt}

329: \textit{Promise:-3.525}, Method: LimGen\\
There was a vain liar named Dot,
Who wanted an audience of thought. 
She was a nobody, 
She was ashamed to be, 
She was proud to be a complete shot. \\ \vspace{0.1pt}

330: \textit{Season:-2.856}, Method: LimGen\\
There was a shy captain named Kay,
Who put a big smile on our day. 
It was like a spring, 
It was the perfect thing, 
It was nice to have a warm birthday. \\ \vspace{0.1pt}

331: \textit{Rain:-3.169}, Method: LimGen\\
There was a quiet girl named Marcell,
Who kept a close eye on our trail. 
When we got to twilight, 
We were met by a light, 
Which was filled with the finest detail. \\ \vspace{0.1pt}

332: \textit{Throne:-3.360}, Method: LimGen\\
There once was a lady named Bethel,
Whose husband fled a battle in hell. 
When she returned to land, 
She was met by a hand, 
And asked her because she was rebel. \\ \vspace{0.1pt}

333: \textit{Politics:-3.150}, Method: LimGen\\
There was a professor named Kay,
Who learned a new language on her way. 
She came back from the war, 
And she went to the store, 
And now she has a job resume. \\ \vspace{0.1pt}

334: \textit{Winter:-3.260}, Method: LimGen\\
There was a bright lady named Rose,
Who decided on one of her clothes. 
It was on the daytime, 
It was the perfect time, 
It was also the moment she chose. \\ \vspace{0.1pt}

335: \textit{Beach:-3.382}, Method: LimGen\\
There was a lazy girl named Rose,
Who went on a holiday of clothes. 
She came back from the trip, 
Found the dress on her slip, 
And decided on the perfect pose. \\ \vspace{0.1pt}

336: \textit{Spider:-3.407}, Method: LimGen\\
There was a funny witch named Nicole,
Who trapped all my money in a hole. 
I got back from the cave, 
And I went to the grave, 
And killed her because she was charcoal. \\ \vspace{0.1pt}

337: \textit{Cunning:-3.258}, Method: LimGen\\
There once was a liar named Kai,
Who fooled a grand jury on her lie. 
I had a suspicion, 
I was on a mission, 
I was ready to fight and to die. \\ \vspace{0.1pt}

338: \textit{Limerick:-4.092}, Method: LimGen\\
There was a writer named Rose,
Who wright a short story on his prose. 
It was a satire, 
But it also had fire, 
And it came down and hit our nose. \\ \vspace{0.1pt}

339: \textit{Money:-2.841}, Method: LimGen\\
There was a woman named Kay,
Who got a flat tire on her way. 
When she returned to work, 
She was told by a clerk, 
She did not have money left this day. \\ \vspace{0.1pt}

340: \textit{Love:-2.959}, Method: LimGen\\
There was a jealous girl named Kay,
Who got a flat tire on her way. 
It was for her birthday, 
It was the perfect day, 
She walked through the door and saw sunday. \\ \vspace{0.1pt}

341: \textit{Bank:-2.867}, Method: LimGen\\
There once was a farmer named Margarete,
Who owned a small farm on our street. 
She worked on the railroad, 
And she took to the road, 
And now she has a family seat. \\ \vspace{0.1pt}

342: \textit{Born:-2.707}, Method: LimGen\\
There was a brave farmer named Kay,
Who died a young girl on her birthday. 
She came back from the grave, 
And she went to the cave, 
And she sat down and began her day. \\ \vspace{0.1pt}

343: \textit{War:-2.792}, Method: LimGen\\
There was a warrior named Brande,
Who fought a great battle on her land. 
When she arrived to fight, 
She was struck by a light, 
And fell on the treacherous wasteland. \\ \vspace{0.1pt}

344: \textit{World:-2.919}, Method: LimGen\\
There was a brave girl named Kay,
Who made a huge impact on my day. 
She was a nobody, 
She was raised by a tree, 
And she came down and saved my birthday. \\ \vspace{0.1pt}

345: \textit{Death:-3.051}, Method: LimGen\\
There was a cruel judge named Clare,
Who lived all her life in a nightmare. 
When she returned to hell, 
She was able to tell, 
She saw all her friends lying nowhere. \\ \vspace{0.1pt}

346: \textit{Water:-3.157}, Method: LimGen\\
There once was a cleaner named Dot,
Who washed out her windows for a pot. 
When she returned to land, 
She was able to stand, 
So she went up and slept on the spot. \\ \vspace{0.1pt}

347: \textit{Blood:-2.931}, Method: LimGen\\
There was a vain doctor named Collette,
Who drank all her water in a sweat. 
She was a physician, 
She was on a mission, 
She was trained to be a great asset. \\ \vspace{0.1pt}

348: \textit{Sports:-3.004}, Method: LimGen\\
There was a smart writer named Grace,
Who put a great spin on our race. 
She started on the show, 
She was ready to go, 
She was prepared to fight and to ace. \\ \vspace{0.1pt}

349: \textit{Fire:-3.236}, Method: LimGen\\
There was a fierce woman named Maryann,
Who brought out my feelings for a man. 
We met on the roadside, 
It was raining outside, 
She said that her husband was afghan. \\ \vspace{0.1pt}

350: \textit{Planet:-2.851}, Method: LimGen\\
There was a warrior named Brande,
Who lived a long time on our land. 
She came back from the war, 
And she went to the door, 
And stood on the threshold beforehand. \\ \vspace{0.1pt}

351: \textit{Disease:-3.237}, Method: LimGen\\
There was a stubborn nurse named Joycelyn,
Who suffered an injury of skin. 
When she returned to fight, 
She was shocked by her sight, 
And now she has a permanent grin. \\ \vspace{0.1pt}

352: \textit{Dog:-2.696}, Method: LimGen\\
There was a lucky girl named Loraine,
Who got a free ride on our train. 
When she started to walk, 
She was afraid to talk, 
So she had to sit down on the plane. \\ \vspace{0.1pt}

353: \textit{Love:-3.310}, Method: LimGen\\
There was a jealous girl named Renee,
Who got a new boyfriend on her way. 
It was for her birthday, 
And she went to the play, 
And saw her because she was halfway. \\ \vspace{0.1pt}

354: \textit{Opera:-3.121}, Method: LimGen\\
There was a lame dancer named Amal,
Who danced as she sat on a football. 
It was like a nightmare, 
It was painful to stare, 
But I knew she was watching me crawl. \\ \vspace{0.1pt}

355: \textit{Animal:-3.150}, Method: LimGen\\
There was a woman named Renee,
Who found a dead body on her way. 
When she returned to land, 
She was met by her band, 
And they took down and burned her cache. \\ \vspace{0.1pt}

356: \textit{Car:-3.054}, Method: LimGen\\
There was a smart woman named Jone,
Who put all her money in a loan. 
It was like a fire, 
And it burned to the wire, 
And she went down and broke her backbone. \\ \vspace{0.1pt}

357: \textit{Monster:-3.032}, Method: LimGen\\
There was a sexy girl named Freda,
Who got a flat tire on her head. 
When she started to scream, 
She was stopped by her team, 
But they said she was doing it dead. \\ \vspace{0.1pt}

358: \textit{Library:-3.228}, Method: LimGen\\
There once was a teacher named Dot,
Who found a dead body on her lot. 
She came back from the store, 
Saw the clothes that she wore, 
And knew her because she heard gunshot. \\ \vspace{0.1pt}

359: \textit{Noble:-3.437}, Method: LimGen\\
There once was a lady named Ariane,
Who wished a good morning on her man. 
It was a tradition, 
She was on a mission, 
She was ready to go and to van. \\ \vspace{0.1pt}

360: \textit{Exercise:-3.333}, Method: LimGen\\
There was a wise woman named Renee,
Who learned a great fortune on her way. 
When she returned to work, 
She was married to turk, 
But she knew she was getting him gay. \\ \vspace{0.1pt}

361: \textit{Market:-3.097}, Method: LimGen\\
There was a wise farmer named Grace,
Who bought a small farm on our place. 
She started on the lot, 
And we moved to the plot, 
And now she has a permanent space. \\ \vspace{0.1pt}

362: \textit{Funeral:-3.188}, Method: LimGen\\
There once was a grandma named Kay,
Who died a sad death on her birthday. 
She was like a statue, 
She had the perfect view, 
She was tall to be a female day. \\ \vspace{0.1pt}

363: \textit{Body:-2.966}, Method: LimGen\\
There was a skinny girl named Grace,
Who put a big smile on our face. 
We got back from the break, 
And we went to the lake, 
Was totally a different place. \\ \vspace{0.1pt}

364: \textit{Doctor:-2.738}, Method: LimGen\\
There was a nervous nurse named Loraine,
Who had a new baby on her brain. 
When she learned to talk, 
She was able to walk, 
She finally understood her pain. \\ \vspace{0.1pt}

365: \textit{Smart:-3.245}, Method: LimGen\\
There was a smart lady named Lorelei,
Who put a blind fold on our guy. 
She asked for our key, 
And we went to the tree, 
And we had keys everywhere nearby. \\ \vspace{0.1pt}

366: \textit{Art:-2.691}, Method: LimGen\\
There was a neat teacher named Kay,
Who made a big impact on my way. 
She was a musician, 
She was on a mission, 
She was ready to go and to play. \\ \vspace{0.1pt}

367: \textit{Gun:-2.939}, Method: LimGen\\
There was a loud woman named Grace,
Who put a big smile on our face. 
It was like a flashlight, 
It was the perfect light, 
It came through the window and hit space. \\ \vspace{0.1pt}

368: \textit{Ball:-2.847}, Method: LimGen\\
There was a lucky girl named Freda,
Who made a huge impact on my head. 
She was like a spring, 
She was the perfect thing, 
She was easy to write and to read. \\ \vspace{0.1pt}

369: \textit{Creativity:-3.503}, Method: LimGen\\
There was a artist named Ines,
Who learned a great deal on her process. 
She started on the art, 
But she also worked smart, 
And she wrote down and showed her progress. \\ \vspace{0.1pt}

370: \textit{Boxing:-3.072}, Method: LimGen\\
There was a warrior named Brande,
Who fought a great battle on her hand. 
She came back from the fight, 
Healed the wound on her knight, 
And entered the battlefield with brand. \\ \vspace{0.1pt}

371: \textit{Forest:-3.240}, Method: LimGen\\
There was a bright lady named Bok,
Who covered as she went on a walk. 
She looked like a rainbow, 
She had so much shadow, 
It was hard to focus and to talk. \\ \vspace{0.1pt}

372: \textit{Philosophy:-3.159}, Method: LimGen\\
There was a wise teacher named Bess,
Who taught a short course on my progress. 
She was like a mentor, 
And I felt to the core, 
She really admired my process. \\ \vspace{0.1pt}

373: \textit{Scary:-3.280}, Method: LimGen\\
There was a boring girl named Sharleen,
Who seemed a good fit on our scene. 
She was like a nightmare, 
She was perfect to wear, 
She was easy to read and to mean. \\ \vspace{0.1pt}

374: \textit{Violent:-3.075}, Method: LimGen\\
There was a harsh woman named Lore,
Whose husband killed a baby in war. 
When she returned to hell, 
She was saved by a spell, 
And now she is a holy mentor. \\ \vspace{0.1pt}

375: \textit{Night:-2.936}, Method: LimGen\\
There was a quiet girl named Laure,
Who had a big smile on her before. 
It was for her birthday, 
It was the perfect day, 
It was also the party she wore. \\ \vspace{0.1pt}

376: \textit{Evil:-3.703}, Method: LimGen\\
There was a selfish witch named Adell,
Whose soul possessed a demon in hell. 
She decided to flee, 
But it soon became he, 
And now she is a demon rebel. \\ \vspace{0.1pt}

377: \textit{Angry:-3.156}, Method: LimGen\\
There was a fierce woman named Michele,
Whose death provoked a riot in hell. 
When she arrived to fight, 
She was killed by a knight, 
But she does not die within her cell. \\ \vspace{0.1pt}

378: \textit{Music:-2.949}, Method: LimGen\\
There was a teacher named Brande,
Who played a big role on our band. 
She was on the record, 
And she came to the board, 
And now she has a permanent hand. \\ \vspace{0.1pt}

379: \textit{Color:-3.289}, Method: LimGen\\
There once was a artist named Grace,
Who used a red lipstick on her face. 
When she started to fade, 
She was the perfect shade, 
But I am not ashamed for race. \\ \vspace{0.1pt}

380: \textit{Pride:-2.812}, Method: LimGen\\
There was a fierce woman named Nicolle,
Who felt a deep longing on her soul. 
When she started to cry, 
She was afraid to die, 
So she chose to go down on the hole. \\ \vspace{0.1pt}

381: \textit{Rich:-3.060}, Method: LimGen\\
There once was a farmer named Arline,
Who made a huge profit on her wine. 
It was a tradition, 
She was on a mission, 
And she did not like something of mine. \\ \vspace{0.1pt}

382: \textit{Law:-3.081}, Method: LimGen\\
There was a honest judge named Grace,
Who passed a fair judgment on my case. 
She said on the trial, 
She was shocked by my file, 
It was strange to see a female face. \\ \vspace{0.1pt}

383: \textit{Light:-3.229}, Method: LimGen\\
There was a woman named Renee,
Who made all her money in a way. 
It was like a rainbow, 
It was the perfect show, 
I loved that her character was gay. \\ \vspace{0.1pt}

384: \textit{Weight:-3.099}, Method: LimGen\\
There was a wise girl named Shin,
Who felt a strange presence on her skin. 
When she started to sweat, 
Her body was so wet, 
She thought that her husband had akin. \\ \vspace{0.1pt}

385: \textit{Loss:-2.975}, Method: LimGen\\
There was a wise woman named Kay,
Who helped a poor widow on her way. 
When she returned to fight, 
She was struck by a light, 
And she fell down and became her prey. \\ \vspace{0.1pt}

386: \textit{Leader:-2.932}, Method: LimGen\\
There was a lieutenant named Kay,
Who led a small army on their way. 
When they arrived to fight, 
She was killed by a knight, 
But she does not die in our play. \\ \vspace{0.1pt}

387: \textit{Useful:-2.741}, Method: LimGen\\
There was a smart cleaner named Dot,
Who found a dead body on her lot. 
When she returned to work, 
She was told by a clerk, 
She was not the manager she thought. \\ \vspace{0.1pt}

388: \textit{School:-3.049}, Method: LimGen\\
There was a shy teacher named Pam,
Who did a great job on our program. 
She was like a mentor, 
And she taught to the core, 
And she got down and wrote our programme. \\ \vspace{0.1pt}

389: \textit{Applaud:-3.729}, Method: LimGen\\
There was a wise writer named Dede,
Who wished a great deal on her indeed. 
She wanted to impress, 
She was eager to press, 
And she looked down and noticed her speed. \\ \vspace{0.1pt}

390: \textit{Union:-3.710}, Method: LimGen\\
There was a fierce teacher named Willette,
Whose family paid a fortune in debt. 
When she returned to school, 
She was shocked by her cool, 
Young teachers are older and upset. \\ \vspace{0.1pt}

391: \textit{Airplane:-3.188}, Method: LimGen\\
There was a captain named Germaine,
Who flew a big flag on our plane. 
We were on the highway, 
And we got to the bay, 
And we went right past something insane. \\ \vspace{0.1pt}

392: \textit{Child:-2.640}, Method: LimGen\\
There was a nervous girl named Grace,
Who put a big smile on our face. 
When she started to cry, 
I was ready to die, 
But I knew she was giving me grace. \\ \vspace{0.1pt}

393: \textit{Park:-2.871}, Method: LimGen\\
There once was a lady named Bridgette,
Who drove a white van on our street. 
We were on the highway, 
And we saw to the way, 
And we went down and took our seat. \\ \vspace{0.1pt}

394: \textit{Home:-2.758}, Method: LimGen\\
There was a neat grandma named Kay,
Who had a new baby on her way. 
When she returned to town, 
Her son had a breakdown, 
And that is the story of this day. \\ \vspace{0.1pt}

395: \textit{Hope:-2.883}, Method: LimGen\\
There was a lucky girl named Renee,
Who got a flat tire on her way. 
She decided to stay, 
It was the perfect day, 
It was easy to walk and to play. \\ \vspace{0.1pt}

396: \textit{Flower:-3.158}, Method: LimGen\\
There was a bright woman named Ines,
Who cut a perfect line on her dress. 
It was on the rainbow, 
It was on a photo, 
It was easy to find and to press. \\ \vspace{0.1pt}

397: \textit{Cheat:-3.001}, Method: LimGen\\
There was a hustler named Renee,
Who put all her money in a play. 
She was like a girlfriend, 
She would have a boyfriend, 
She was ready to go and to stay. \\ \vspace{0.1pt}

398: \textit{Working:-2.870}, Method: LimGen\\
There was a smart nurse named Ines,
Who kept a close eye on my progress. 
When I needed to talk, 
She was ready to walk, 
But she does not travel in her dress. \\ \vspace{0.1pt}

399: \textit{Time:-2.993}, Method: LimGen\\
There was a lady named Kay,
Who spent all her money in a day. 
She was a nobody, 
She was raised by a tree, 
She did not know life happened this way. \\ \vspace{0.1pt}






==> candidate_rank_poem.tex <==
1: \textit{Born:-2.913}, Method: Candidate-Rank\\
There was a brave boy named Lyle,
Who lived all his life in a exile. 
He came back from the war, 
And he went to the door, 
He looked through the window and saw trial. \\ \vspace{0.1pt}

2: \textit{Shaken:-2.990}, Method: Candidate-Rank\\
There was a nervous man named Jake,
Who shook all his money in a shake. 
It was like a earthquake, 
And we went to the lake, 
And we sat down and took our break. \\ \vspace{0.1pt}

3: \textit{Kindness:-3.077}, Method: Candidate-Rank\\
There was a humble man named Javier,
Who loved a good story and prayer. 
He would say to a friend, 
It was easy to end, 
It was hard to start a new nightmare. \\ \vspace{0.1pt}

4: \textit{Surprise:-2.821}, Method: Candidate-Rank\\
There was a clever boy named Dwight,
Who did all his writing in a night. 
He would go to a show, 
He would take a photo, 
And that is the basis of this site. \\ \vspace{0.1pt}

5: \textit{Tears:-2.819}, Method: Candidate-Rank\\
There was a vain boy named Chase,
Who smiled a cruel smile on his face. 
He was a nobody, 
His father was a tree, 
So he had to look down on the place. \\ \vspace{0.1pt}

6: \textit{Restore:-2.882}, Method: Candidate-Rank\\
There was a wise man named Stan,
Who lost all his money in a plan. 
He decided to run, 
And he ran to the sun, 
And he came down and started his van. \\ \vspace{0.1pt}

7: \textit{Laugh:-3.086}, Method: Candidate-Rank\\
There was a stupid boy named Chase,
Who watched a bad movie on his face. 
When he turned to someone, 
He was met by a gun, 
So he had to go down on the base. \\ \vspace{0.1pt}

8: \textit{Alien:-3.086}, Method: Candidate-Rank\\
There was a warrior named Kip,
Who trapped a young woman on his ship. 
When she refused to fight, 
She was killed by a knight, 
And now she is a prisoner hip. \\ \vspace{0.1pt}

9: \textit{Holiday:-2.710}, Method: Candidate-Rank\\
There was a bright chef named Kip,
Who spent a small fortune on his trip. 
When he returned to town, 
His wife had a breakdown, 
So he gave up and quit on the ship. \\ \vspace{0.1pt}

10: \textit{Thanksgiving:-2.774}, Method: Candidate-Rank\\
There was a funny chef named Dwight,
Who ate all his dinner in a night. 
When he got to midnight, 
He was ready to fight, 
And that is the story of this site. \\ \vspace{0.1pt}

11: \textit{Injury:-2.893}, Method: Candidate-Rank\\
There once was a surgeon named Tyree,
Who healed a gunshot wound on his knee. 
When he returned to fight, 
He was shocked by his sight, 
So he went to look down on the sea. \\ \vspace{0.1pt}

12: \textit{Birthday:-2.670}, Method: Candidate-Rank\\
There was a jealous boy named Dwight,
Who got all his money in a night. 
When he returned to school, 
He was shocked by his cool, 
But he knew he was doing it right. \\ \vspace{0.1pt}

13: \textit{Pillow:-3.058}, Method: Candidate-Rank\\
There was a skinny boy named Ted,
Who felt a strange feeling on his head. 
He looked like a fairy, 
His hair was so hairy, 
But it seemed he was growing it red. \\ \vspace{0.1pt}

14: \textit{Wine:-2.916}, Method: Candidate-Rank\\
There was a neat chef named Chase,
Who served a great menu on his place. 
We decided to eat, 
So we walked down the street, 
Then they put us right outside the space. \\ \vspace{0.1pt}

15: \textit{Traffic:-2.845}, Method: Candidate-Rank\\
There was a quiet man named Pete,
Who drove a small car on our street. 
He was on the railroad, 
And he came to the road, 
So he had to get down on the seat. \\ \vspace{0.1pt}

16: \textit{Beer:-2.965}, Method: Candidate-Rank\\
There was a lucky chef named Dwight,
Who ate all his dinner in a night. 
When he returned to town, 
His wife had a breakdown, 
And he took down and buried his site. \\ \vspace{0.1pt}

17: \textit{Mountain:-3.087}, Method: Candidate-Rank\\
There was a harsh boy named Jerrell,
Who rode a white horse on our trail. 
When we arrived to ride, 
We were told by our guide, 
He was dead to find a black female. \\ \vspace{0.1pt}

18: \textit{Fiance:-2.945}, Method: Candidate-Rank\\
There once was a grandpa named Jake,
Who told all his story in a cake. 
It was for my birthday, 
And we went to the play, 
So we had to go down on the lake. \\ \vspace{0.1pt}

19: \textit{Memory:-2.565}, Method: Candidate-Rank\\
There was a wise man named Chase,
Who lost all his money in a case. 
He came back from the grave, 
And he went to the cave, 
And that is the story of this place. \\ \vspace{0.1pt}

20: \textit{Mud:-2.874}, Method: Candidate-Rank\\
There was a harsh cleaner named Chase,
Who stuck a hot iron on her face. 
When she started to sweat, 
She was afraid to get, 
So she tried to go down on the place. \\ \vspace{0.1pt}

21: \textit{Rain:-2.723}, Method: Candidate-Rank\\
There was a quiet boy named Jerrell,
Who kept a close eye on our trail. 
When we arrived to ride, 
We were told by our guide, 
That the horse we rode was a female. \\ \vspace{0.1pt}

22: \textit{Season:-2.524}, Method: Candidate-Rank\\
There was a bright actor named Dario,
Who played a big role on our show. 
He came back from the break, 
And he went to the lake, 
And he sat down and took his photo. \\ \vspace{0.1pt}

23: \textit{Throne:-2.858}, Method: Candidate-Rank\\
There was a fierce man named Pierre,
Who stood all his life in a prayer. 
When he began to cry, 
He was told by a lie, 
That the woman he loved was a bear. \\ \vspace{0.1pt}

24: \textit{Politics:-2.730}, Method: Candidate-Rank\\
There was a general named Theodore,
Whose son became a soldier in war. 
When he learned to talk, 
He was able to walk, 
So he used to sit down on the floor. \\ \vspace{0.1pt}

25: \textit{Beach:-2.725}, Method: Candidate-Rank\\
There was a lively man named Theodore,
Who stayed a long time on our shore. 
He came back from the sea, 
And he went to the tree, 
And he sat down and read our lore. \\ \vspace{0.1pt}

26: \textit{Love:-2.872}, Method: Candidate-Rank\\
There was a lucky boy named Scot,
Who put all his money in a lot. 
When he started to fall, 
He got caught by a wall, 
And now he has a permanent spot. \\ \vspace{0.1pt}

27: \textit{Promise:-3.130}, Method: Candidate-Rank\\
There was a honest man named Scot,
Who gave a long lecture on his thought. 
When he started to cry, 
I was ready to die, 
And that is the reason of this plot. \\ \vspace{0.1pt}

28: \textit{Cunning:-3.112}, Method: Candidate-Rank\\
There was a magician named Nick,
Who fooled all his family in a trick. 
But his father was cruel, 
And he went to the school, 
But he knew he was getting him sick. \\ \vspace{0.1pt}

29: \textit{Dog:-2.716}, Method: Candidate-Rank\\
There was a lucky boy named Dewayne,
Who got a free ride on our train. 
He came back from the car, 
And we went to the bar, 
So we had to sit down on the plane. \\ \vspace{0.1pt}

30: \textit{Bank:-2.608}, Method: Candidate-Rank\\
There was a greedy man named Wade,
Who lost all his money in a trade. 
When he returned to town, 
His wife had a breakdown, 
So he had to go down on the raid. \\ \vspace{0.1pt}

31: \textit{Death:-2.618}, Method: Candidate-Rank\\
There was a brave soldier named Javier,
Who lived all his life in a nightmare. 
He came back from the grave, 
And he went to the cave, 
And he sat down and said his prayer. \\ \vspace{0.1pt}

32: \textit{Blood:-2.929}, Method: Candidate-Rank\\
There was a cruel man named Dwight,
Who drank all his money in a fight. 
When he returned to hell, 
He was able to tell, 
He found that his family was right. \\ \vspace{0.1pt}

33: \textit{World:-2.860}, Method: Candidate-Rank\\
There was a wise man named Theodore,
Who lost all his money in a war. 
When he returned to fight, 
He was killed by a knight, 
And now he has a family mentor. \\ \vspace{0.1pt}

34: \textit{Planet:-2.726}, Method: Candidate-Rank\\
There was a bright man named Kip,
Who lived a long time on our ship. 
He came back from the war, 
And he went to the shore, 
And that is the story of this trip. \\ \vspace{0.1pt}

35: \textit{Sports:-2.864}, Method: Candidate-Rank\\
There was a smart boy named Claudio,
Who played a big role on our show. 
He would go to a game, 
He would get a nickname, 
But you knew he was playing it pro. \\ \vspace{0.1pt}

36: \textit{Water:-2.533}, Method: Candidate-Rank\\
There was a bright cleaner named Scot,
Who put all his money in a pot. 
When he started to smoke, 
His father had a stroke, 
So he got up and quit on the spot. \\ \vspace{0.1pt}

37: \textit{Violent:-2.679}, Method: Candidate-Rank\\
There was a harsh soldier named Dwight,
Who killed all his family in a fight. 
When he returned to hell, 
He was saved by a spell, 
And now he is a warrior knight. \\ \vspace{0.1pt}

38: \textit{Opera:-2.633}, Method: Candidate-Rank\\
There was a actor named Dario,
Who played a big role on our show. 
He was a musician, 
He was on a mission, 
He made sure to get a good photo. \\ \vspace{0.1pt}

39: \textit{Fire:-2.758}, Method: Candidate-Rank\\
There was a fierce man named Dwight,
Who killed all his family in a fight. 
He came back from the war, 
And he went to the store, 
But he said he was doing it right. \\ \vspace{0.1pt}

40: \textit{Monster:-2.865}, Method: Candidate-Rank\\
There was a fierce boy named Chase,
Who caught a stray bullet on his face. 
When he returned to fight, 
He was struck by a light, 
So he had to go down on the base. \\ \vspace{0.1pt}

41: \textit{Library:-2.906}, Method: Candidate-Rank\\
There was a smart teacher named Ward,
Who found a strange object on his board. 
When he returned to school, 
He was caught by a rule, 
So he had to sit down on the sword. \\ \vspace{0.1pt}

42: \textit{Noble:-3.180}, Method: Candidate-Rank\\
There was a cruel man named Cole,
Who wished a great deal on our soul. 
He asked for our grace, 
Our love and our space, 
But we refused his demands and stole. \\ \vspace{0.1pt}

43: \textit{Doctor:-2.472}, Method: Candidate-Rank\\
There was a doctor named Zane,
Who did a great treatment on my brain. 
He was a physician, 
He was on a mission, 
And he came down and treated my pain. \\ \vspace{0.1pt}

44: \textit{Ball:-2.896}, Method: Candidate-Rank\\
There was a lucky boy named Chase,
Who put a big smile on our face. 
When we started to play, 
It was easy to say, 
But we knew we were doing it place. \\ \vspace{0.1pt}

45: \textit{Body:-2.551}, Method: Candidate-Rank\\
There was a skinny man named Chase,
Who put a big smile on our face. 
When we arrived to work, 
We were met by a clerk, 
And we sat down and took our place. \\ \vspace{0.1pt}

46: \textit{Smart:-2.959}, Method: Candidate-Rank\\
There was a clever boy named Rick,
Who put all his money in a trick. 
When he learned to talk, 
He was able to walk, 
And that is the story of this stick. \\ \vspace{0.1pt}

47: \textit{Music:-2.714}, Method: Candidate-Rank\\
There was a funny boy named Romeo,
Who played a big role on our show. 
He was a musician, 
He was on a mission, 
And now he has a job tomorrow. \\ \vspace{0.1pt}

48: \textit{Art:-2.579}, Method: Candidate-Rank\\
There was a neat artist named Lyle,
Who made a huge impact on my style. 
I would go to a show, 
He would take a photo, 
It was great to have a big profile. \\ \vspace{0.1pt}

49: \textit{Gun:-2.578}, Method: Candidate-Rank\\
There was a loud boy named Chase,
Who put a big smile on our face. 
He was back from the war, 
And he came to the door, 
And we went down and took our place. \\ \vspace{0.1pt}

50: \textit{Forest:-2.941}, Method: Candidate-Rank\\
There was a brave farmer named Burt,
Who harvested an acre of dirt. 
When he returned to town, 
His wife had a breakdown, 
And he ran down and buried his shirt. \\ \vspace{0.1pt}

51: \textit{Philosophy:-2.770}, Method: Candidate-Rank\\
There was a teacher named Rex,
Who taught on a couple of subjects. 
He was like a mentor, 
And he came to the door, 
And we sat down and had our sex. \\ \vspace{0.1pt}

52: \textit{Night:-2.608}, Method: Candidate-Rank\\
There was a loud man named Dario,
Who did a great job on our show. 
He came back from the break, 
And he went to the lake, 
And he sat down and took his photo. \\ \vspace{0.1pt}

53: \textit{Exercise:-3.018}, Method: Candidate-Rank\\
There was a wise judge named Brock,
Who learned a great lesson on his walk. 
When he returned to work, 
He was told by a clerk, 
That the man he replaced was a cock. \\ \vspace{0.1pt}

54: \textit{Scary:-3.388}, Method: Candidate-Rank\\
There was a boring boy named Valentin,
Who seemed a good fit on our scene. 
When we started to talk, 
He was ready to walk, 
But we needed his hands and protein. \\ \vspace{0.1pt}

55: \textit{Angry:-3.085}, Method: Candidate-Rank\\
There was a fierce boy named Stan,
Who shouted as he jumped on a man. 
When he turned to someone, 
He was met by a gun, 
So he got up and put on the van. \\ \vspace{0.1pt}

56: \textit{Pride:-2.843}, Method: Candidate-Rank\\
There was a warrior named Cole,
Who felt a deep sadness on his soul. 
When he returned to mind, 
He was surprised to find, 
That the person he loved was a hole. \\ \vspace{0.1pt}

57: \textit{Light:-2.753}, Method: Candidate-Rank\\
There was a loud cleaner named Jed,
Who used a big hammer on my head. 
When I started to fall, 
I was pushed by a wall, 
And I fell down and hit our bed. \\ \vspace{0.1pt}

58: \textit{School:-2.640}, Method: Candidate-Rank\\
There was a shy teacher named Graham,
Who did a great job on our program. 
He was like a mentor, 
And we went to the door, 
And we sat down and watched his programme. \\ \vspace{0.1pt}

59: \textit{Color:-2.858}, Method: Candidate-Rank\\
There was a bright artist named Chase,
Who used a red lipstick on his face. 
It looked like a rainbow, 
But was a black shadow, 
So it had to be down on the base. \\ \vspace{0.1pt}

60: \textit{Loss:-2.819}, Method: Candidate-Rank\\
There was a honest man named Saul,
Who lost all his money in a fall. 
When he returned to fight, 
He was met by a light, 
And he fell down and broke his football. \\ \vspace{0.1pt}

61: \textit{Park:-2.969}, Method: Candidate-Rank\\
There was a neat boy named Pete,
Who drove a white van on our street. 
He worked for our school, 
But he never saw pool, 
So he never played on the concrete. \\ \vspace{0.1pt}

62: \textit{Useful:-2.969}, Method: Candidate-Rank\\
There was a smart author named Dwight,
Who put a short story on his site. 
When he started to post, 
He was told by his host, 
He was welcome to read and to write. \\ \vspace{0.1pt}

63: \textit{Leader:-2.717}, Method: Candidate-Rank\\
There was a brave soldier named Scot,
Who joined a rebel army and fought. 
When he returned to fight, 
He was killed by a knight, 
So he had to go down on the spot. \\ \vspace{0.1pt}

64: \textit{Home:-2.696}, Method: Candidate-Rank\\
There once was a boy named Dwight,
Who lost all his money in a night. 
When he returned to work, 
He was told by a clerk, 
He had enough to eat and to write. \\ \vspace{0.1pt}

65: \textit{Applaud:-3.350}, Method: Candidate-Rank\\
There was a wise judge named Dwight,
Who wished a good time on his invite. 
When he arrived to stand, 
He was struck by a hand, 
So he ran up and put on the light. \\ \vspace{0.1pt}

66: \textit{Union:-2.772}, Method: Candidate-Rank\\
There was a general named Scot,
Who joined a rebel army and fought. 
When he returned to fight, 
He was killed by a knight, 
And that is the story of this plot. \\ \vspace{0.1pt}

67: \textit{Working:-2.581}, Method: Candidate-Rank\\
There was a smart teacher named Jess,
Who kept a close eye on my progress. 
When I started to talk, 
It was easy to walk, 
But I knew he was watching me dress. \\ \vspace{0.1pt}

68: \textit{Cheat:-3.018}, Method: Candidate-Rank\\
There was a greedy man named Theodore,
Who put all his money in a war. 
When he went to combat, 
He was killed by a cat, 
Because he was eating his mentor. \\ \vspace{0.1pt}

69: \textit{Fall:-2.780}, Method: Candidate-Rank\\
There was a wise boy named Bill,
Who lost all his money in a will. 
When he returned to school, 
His father was a fool, 
So he went to live down on the hill. \\ \vspace{0.1pt}

70: \textit{Flower:-2.804}, Method: Candidate-Rank\\
There was a lucky boy named Saul,
Who carved a big circle on his wall. 
It was for his birthday, 
So he wrote down the day, 
And then he gets a telephone call. \\ \vspace{0.1pt}

71: \textit{Random:-2.927}, Method: Candidate-Rank\\
There was a funny man named Lyle,
Who stuck all his money in a pile. 
He would go to a show, 
He would take a photo, 
And that is the basis of this file. \\ \vspace{0.1pt}

72: \textit{Born:-2.677}, Method: Candidate-Rank\\
There was a woman named Kay,
Who died a strange death on her birthday. 
She came back from the grave, 
And she went to the cave, 
And she sat down and began her day. \\ \vspace{0.1pt}

73: \textit{Shaken:-3.025}, Method: Candidate-Rank\\
There was a loud waitress named Brande,
Who poured all her coffee in a stand. 
When she returned to knock, 
She was met by a rock, 
So she went to sit down on the sand. \\ \vspace{0.1pt}

74: \textit{Hope:-2.855}, Method: Candidate-Rank\\
There was a brave man named Wes,
Who did a great work on our progress. 
He came back from the place, 
And he went to the base, 
And he got down and saw our mess. \\ \vspace{0.1pt}

75: \textit{Restore:-2.835}, Method: Candidate-Rank\\
There was a wise cleaner named Joycelyn,
Who tried a new method on her skin. 
She decided to try, 
With the help of a guy, 
And now she has a permanent grin. \\ \vspace{0.1pt}

76: \textit{Laugh:-2.813}, Method: Candidate-Rank\\
There was a loud girl named Grace,
Who smiled a big smile on our face. 
When we arrived to wait, 
We were met by our date, 
And we sat down and took our place. \\ \vspace{0.1pt}

77: \textit{Surprise:-2.756}, Method: Candidate-Rank\\
There once was a lady named Kay,
Who did a good deed on her birthday. 
When she went to someone, 
She was met by a gun, 
So she had to run down on the way. \\ \vspace{0.1pt}

78: \textit{Tears:-2.978}, Method: Candidate-Rank\\
There once was a girl named Nicolle,
Who felt a strange presence on her soul. 
It was like a prayer, 
And she prayed to the air, 
And her prayers grew stronger and whole. \\ \vspace{0.1pt}

79: \textit{Victory:-2.672}, Method: Candidate-Rank\\
There was a brave captain named Renee,
Who fought a great battle on her way. 
She came back from the war, 
And she went to the shore, 
And she sat down and wrote her birthday. \\ \vspace{0.1pt}

80: \textit{Wedding:-2.569}, Method: Candidate-Rank\\
There once was a lady named Renee,
Who wore a red dress on her birthday. 
It was like a costume, 
And she came to the room, 
And we sat down and had our day. \\ \vspace{0.1pt}

81: \textit{Holiday:-2.835}, Method: Candidate-Rank\\
There was a quiet chef named Emeline,
Who spent a small fortune on her wine. 
When she returned to town, 
She was met by a frown, 
But she said she was taking it fine. \\ \vspace{0.1pt}

82: \textit{Christmas:-2.584}, Method: Candidate-Rank\\
There was a lucky girl named Renee,
Who got a great deal on her birthday. 
She came back from the store, 
And she went to the door, 
And she looked down and saw her okay. \\ \vspace{0.1pt}

83: \textit{Thanksgiving:-2.682}, Method: Candidate-Rank\\
There was a funny chef named Kay,
Who cooked a great meal on my birthday. 
I asked for her invite, 
And she came to the site, 
And we sat down and shared our day. \\ \vspace{0.1pt}

84: \textit{Kindness:-3.050}, Method: Candidate-Rank\\
There was a grandma named Renee,
Who loved all her family in a way. 
She would say to a friend, 
She would have a boyfriend, 
But she knew she was doing it gay. \\ \vspace{0.1pt}

85: \textit{Birthday:-2.938}, Method: Candidate-Rank\\
There was a jealous girl named Kate,
Who got a new boyfriend on her date. 
When she arrived to school, 
She was met by a pool, 
So she had to sit down on the gate. \\ \vspace{0.1pt}

86: \textit{Alien:-2.770}, Method: Candidate-Rank\\
There was a cunning witch named Brande,
Who trapped a small village on their land. 
When they tried to rebel, 
They were crushed by her spell, 
So they had to stay down on the sand. \\ \vspace{0.1pt}

87: \textit{Fiance:-2.821}, Method: Candidate-Rank\\
There once was a girl named Renee,
Who loved a hot dog on her birthday. 
When she went to someone, 
She was told by her son, 
That the person she saw was a stray. \\ \vspace{0.1pt}

88: \textit{Dawn:-2.822}, Method: Candidate-Rank\\
There once was a girl named Maire,
Who slept all her life in a nightmare. 
When she awoke to light, 
She was shocked by a sight, 
And she looked down and noticed her hair. \\ \vspace{0.1pt}

89: \textit{Traffic:-2.941}, Method: Candidate-Rank\\
There was a loud lawyer named Kay,
Who stopped a young woman on her way. 
She asked for her address, 
Which she found in the press, 
So she knew to come down on the day. \\ \vspace{0.1pt}

90: \textit{Pillow:-3.128}, Method: Candidate-Rank\\
There was a bright lady named Grace,
Who felt a strange feeling on her face. 
She looked like a fairy, 
Her hair was a cherry, 
But her eyes were down to her birthplace. \\ \vspace{0.1pt}

91: \textit{Heartbreak:-2.752}, Method: Candidate-Rank\\
There was a cruel girl named Maire,
Who cried all her life in a nightmare. 
She came back from the grave, 
And she went to the cave, 
And she sat down and said her prayer. \\ \vspace{0.1pt}

92: \textit{Beer:-2.837}, Method: Candidate-Rank\\
There was a waitress named Renee,
Who ate all her money in a day. 
She would go to a bar, 
And she got to the car, 
And she sat down and had her birthday. \\ \vspace{0.1pt}

93: \textit{River:-2.859}, Method: Candidate-Rank\\
There was a brave farmer named Kay,
Who crossed a dead body on her way. 
When she returned to town, 
She was met by a clown, 
So she got up and put on the play. \\ \vspace{0.1pt}

94: \textit{Spider:-3.029}, Method: Candidate-Rank\\
There was a nasty witch named Nicole,
Who trapped all my family in a hole. 
It was like a nightmare, 
And I cried to the bear, 
And it came down and buried my soul. \\ \vspace{0.1pt}

95: \textit{Mud:-2.906}, Method: Candidate-Rank\\
There was a harsh witch named Grace,
Who stuck a hot iron on her face. 
When she started to sweat, 
Her friend was so upset, 
She threw herself down in the staircase. \\ \vspace{0.1pt}

96: \textit{Wine:-2.921}, Method: Candidate-Rank\\
There once was a chef named Dot,
Who cooked all her dinner in a pot. 
She would go to a bar, 
And she got to the car, 
And she sat down and started her shot. \\ \vspace{0.1pt}

97: \textit{Rain:-2.804}, Method: Candidate-Rank\\
There was a harsh lady named Dayle,
Who kept a close eye on our trail. 
When we arrived to ride, 
We were met by our guide, 
So we had to sit down on the rail. \\ \vspace{0.1pt}

98: \textit{Season:-2.702}, Method: Candidate-Rank\\
There was a shy captain named Amal,
Who kept a close eye on her football. 
When she started to play, 
It was easy to say, 
It was hard to get a good recall. \\ \vspace{0.1pt}

99: \textit{Mountain:-2.747}, Method: Candidate-Rank\\
There was a brave woman named Renee,
Who crossed a dead body on her way. 
When she returned to town, 
She was met by a clown, 
And that is the story of this play. \\ \vspace{0.1pt}

100: \textit{Politics:-3.004}, Method: Candidate-Rank\\
There was a writer named Renee,
Who learned a new language on her way. 
When she started to talk, 
She was able to walk, 
So she asked to sit down on the tray. \\ \vspace{0.1pt}

101: \textit{Promise:-2.814}, Method: Candidate-Rank\\
There was a vain lady named Renee,
Who did a good deed on our way. 
When we arrived to rest, 
We were met by our guest, 
And we sat down and enjoyed our day. \\ \vspace{0.1pt}

102: \textit{Beach:-2.862}, Method: Candidate-Rank\\
There was a bright lady named Bok,
Who went out her windows for a walk. 
She came back from the street, 
And she walked to the seat, 
And she sat down and began her talk. \\ \vspace{0.1pt}

103: \textit{Bank:-2.758}, Method: Candidate-Rank\\
There once was a lawyer named Natividad,
Who lost all her money in a fraud. 
She decided to go, 
And she came to the show, 
And we sat down and did our pod. \\ \vspace{0.1pt}

104: \textit{Cunning:-3.323}, Method: Candidate-Rank\\
There was a cunning witch named Lorelei,
Who fooled all her family in a lie. 
When she returned to hide, 
She was met by her side, 
But she knew she was doing it dry. \\ \vspace{0.1pt}

105: \textit{Love:-2.593}, Method: Candidate-Rank\\
There was a lucky girl named Renee,
Who got a free ticket on her way. 
We decided to go, 
And we went to the show, 
And we sat down and enjoyed our day. \\ \vspace{0.1pt}

106: \textit{Blood:-2.918}, Method: Candidate-Rank\\
There was a vain witch named Nicolle,
Who caused a great havoc on his soul. 
When he returned to hell, 
He was struck by a spell, 
And he fell down and broke his console. \\ \vspace{0.1pt}

107: \textit{Limerick:-3.649}, Method: Candidate-Rank\\
There was a writer named Celeste,
Who wright all her life in a contest. 
She came back from the inn, 
And she went to the gin, 
And she sat down and wrote her protest. \\ \vspace{0.1pt}

108: \textit{Death:-2.917}, Method: Candidate-Rank\\
There was a cruel judge named Grace,
Who brought a false verdict on my case. 
When I went to trial, 
I was shocked by her style, 
But I knew her intentions and face. \\ \vspace{0.1pt}

109: \textit{War:-2.595}, Method: Candidate-Rank\\
There was a warrior named Brande,
Who fought a great battle on our land. 
She came back from the fight, 
And she went to the light, 
And she sat down and took our hand. \\ \vspace{0.1pt}

110: \textit{Dog:-2.719}, Method: Candidate-Rank\\
There was a lady named Renee,
Who got a flat tire on her way. 
When she went to someone, 
She was told by her son, 
That the person she called was a stray. \\ \vspace{0.1pt}

111: \textit{Disease:-2.998}, Method: Candidate-Rank\\
There was a nervous nurse named Trinh,
Who spread a thin layer on my skin. 
Her fingers were so cold, 
It was painful to hold, 
But I knew she was doing me sin. \\ \vspace{0.1pt}

112: \textit{Money:-2.724}, Method: Candidate-Rank\\
There was a woman named Kay,
Who got a flat tire on her way. 
When she went to someone, 
She was told by her son, 
That the person she called was a stray. \\ \vspace{0.1pt}

113: \textit{World:-2.878}, Method: Candidate-Rank\\
There was a wise woman named Lenore,
Who lost all her money in a war. 
When she returned to hell, 
She was saved by a spell, 
And now she has a family therefore. \\ \vspace{0.1pt}

114: \textit{Planet:-2.900}, Method: Candidate-Rank\\
There once was a woman named Brande,
Who lived a perfect life on her land. 
She was a nobody, 
Her husband was a tree, 
And she did not own anything grand. \\ \vspace{0.1pt}

115: \textit{Fire:-2.826}, Method: Candidate-Rank\\
There once was a woman named Liane,
Who turned all her anger towards a man. 
When she came to someone, 
She was told by her son, 
That the person she saw was a fan. \\ \vspace{0.1pt}

116: \textit{Water:-2.522}, Method: Candidate-Rank\\
There once was a woman named Dot,
Who put all her money in a pot. 
When it started to smoke, 
Her husband had a stroke, 
So she got up and quit on the spot. \\ \vspace{0.1pt}

117: \textit{Love:-2.998}, Method: Candidate-Rank\\
There was a lady named Kay,
Who got a flat tire on her way. 
When she arrived to work, 
She was stopped by a clerk, 
But she said he was helping them pray. \\ \vspace{0.1pt}

118: \textit{Car:-2.884}, Method: Candidate-Rank\\
There was a smart cleaner named Margarete,
Who ran a pet store on our street. 
She would go to a shop, 
She would have a workshop, 
She was happy to talk and to eat. \\ \vspace{0.1pt}

119: \textit{Monster:-2.847}, Method: Candidate-Rank\\
There was a hairy witch named Grace,
Who got a strange feeling on her face. 
It was like a nightmare, 
And she went to the chair, 
And she sat down and opened my case. \\ \vspace{0.1pt}

120: \textit{Violent:-2.747}, Method: Candidate-Rank\\
There once was a woman named Lenore,
Who witnessed an incident of war. 
When she returned to fight, 
She was killed by a knight, 
So she had to go down on the floor. \\ \vspace{0.1pt}

121: \textit{Library:-2.799}, Method: Candidate-Rank\\
There was a teacher named Dot,
Who found a strange object on her lot. 
When she returned to work, 
She was told by a clerk, 
That the item she saw was a pot. \\ \vspace{0.1pt}

122: \textit{Doctor:-2.605}, Method: Candidate-Rank\\
There was a surgeon named Lorraine,
Who did a great job on our brain. 
She was a physician, 
She was on a mission, 
And she came down and saw our pain. \\ \vspace{0.1pt}

123: \textit{Funeral:-2.741}, Method: Candidate-Rank\\
There was a grandma named Kay,
Who died a quick death on her birthday. 
She was a physician, 
She was on a mission, 
She was up in heaven and okay. \\ \vspace{0.1pt}

124: \textit{Noble:-3.209}, Method: Candidate-Rank\\
There was a vain woman named Nicole,
Who wished a great favor on my soul. 
But my heart remained pure, 
And I went to the cure, 
Which was done with the strongest console. \\ \vspace{0.1pt}

125: \textit{Ball:-2.664}, Method: Candidate-Rank\\
There once was a captain named Grace,
Who put a big smile on our face. 
When we started to play, 
It was easy to say, 
It was nice to have a female ace. \\ \vspace{0.1pt}

126: \textit{Animal:-2.818}, Method: Candidate-Rank\\
There once was a farmer named Maile,
Who found a strange object on her tail. 
When she returned to land, 
She was struck by a hand, 
So she had to stay down on the trail. \\ \vspace{0.1pt}

127: \textit{Opera:-2.692}, Method: Candidate-Rank\\
There was a lame artist named Brande,
Who played a big role on our band. 
She would come to a show, 
She would take a photo, 
And that is the basis of this brand. \\ \vspace{0.1pt}

128: \textit{Body:-2.866}, Method: Candidate-Rank\\
There was a lady named Grace,
Who put a big smile on our face. 
When we arrived to work, 
We were told by a clerk, 
That the lady we met had a case. \\ \vspace{0.1pt}

129: \textit{Smart:-2.882}, Method: Candidate-Rank\\
There was a smart lady named Kai,
Who put a blind fold on our guy. 
When he started to talk, 
He was able to walk, 
But we thought we were getting him high. \\ \vspace{0.1pt}

130: \textit{Music:-2.589}, Method: Candidate-Rank\\
There was a loud artist named Brande,
Who played a big role on our band. 
She would come to a show, 
She would take a photo, 
And that is the basis of this brand. \\ \vspace{0.1pt}

131: \textit{Art:-2.904}, Method: Candidate-Rank\\
There was a teacher named Amal,
Who drew a big picture on her wall. 
It looked like a photo, 
But it really was though, 
And that is the story of this doll. \\ \vspace{0.1pt}

132: \textit{Gun:-2.677}, Method: Candidate-Rank\\
There was a loud girl named Grace,
Who put a big smile on our face. 
We decided to go, 
So we went down the row, 
So we had to sit down on the base. \\ \vspace{0.1pt}

133: \textit{Forest:-2.876}, Method: Candidate-Rank\\
There was a brave farmer named Brande,
Who harvested an acre of land. 
When she returned to town, 
She was met by a clown, 
And that is the story of this band. \\ \vspace{0.1pt}

134: \textit{Creativity:-3.111}, Method: Candidate-Rank\\
There was a writer named Renee,
Who learned a new language on her way. 
When she arrived to work, 
She was told by a clerk, 
That the woman she saw was a stray. \\ \vspace{0.1pt}

135: \textit{Philosophy:-3.208}, Method: Candidate-Rank\\
There was a wise teacher named Renee,
Who taught a great sermon on her way. 
When she returned to work, 
She was told by a clerk, 
She had not come home needed this day. \\ \vspace{0.1pt}

136: \textit{Evil:-2.965}, Method: Candidate-Rank\\
There was a cruel witch named Kay,
Who cursed a small village on her way. 
When she arrived to fight, 
She was met by a knight, 
And she fell down and became her prey. \\ \vspace{0.1pt}

137: \textit{Pride:-2.949}, Method: Candidate-Rank\\
There was a fierce woman named Nicolle,
Who felt a deep burning on her soul. 
When she came to yourself, 
You were shocked by your self, 
And that is the meaning of this scroll. \\ \vspace{0.1pt}

138: \textit{Angry:-3.176}, Method: Candidate-Rank\\
There was a loud lady named Kai,
Who panicked as I stepped on a guy. 
She screamed for her boyfriend, 
Her brother and her friend, 
And they came down and helped her nearby. \\ \vspace{0.1pt}

139: \textit{School:-2.733}, Method: Candidate-Rank\\
There was a lucky girl named Renee,
Who had a small baby on her way. 
When she arrived to work, 
She was stopped by a clerk, 
So she went to sit down on the tray. \\ \vspace{0.1pt}

140: \textit{Light:-2.900}, Method: Candidate-Rank\\
There was a harsh girl named Grace,
Who made a bad comment on my face. 
When she started to smile, 
I was shocked by her style, 
So I went to sit down on the base. \\ \vspace{0.1pt}

141: \textit{Scary:-2.940}, Method: Candidate-Rank\\
There was a funny witch named Lise,
Who happened on one of our guys. 
We decided to go, 
And we went to the show, 
And we came down and got our prize. \\ \vspace{0.1pt}

142: \textit{Color:-3.109}, Method: Candidate-Rank\\
There was a chunky girl named Grace,
Who used a red lipstick on her face. 
She looked like a rainbow, 
Her hair was a shadow, 
And she wore makeup everywhere place. \\ \vspace{0.1pt}

143: \textit{Park:-2.790}, Method: Candidate-Rank\\
There was a quiet girl named Bok,
Who walked a great distance on her walk. 
When she arrived to school, 
She was met by a pool, 
So she had to sit down on the rock. \\ \vspace{0.1pt}

144: \textit{Loss:-3.026}, Method: Candidate-Rank\\
There once was a doctor named Amal,
Who lost all her money in a fall. 
When she returned to fight, 
She was shocked by her height, 
But she knew she was fighting it tall. \\ \vspace{0.1pt}

145: \textit{Useful:-2.765}, Method: Candidate-Rank\\
There was a doctor named Dot,
Who found a dead body on her lot. 
When she went to someone, 
She was told by her son, 
They were not the family she thought. \\ \vspace{0.1pt}

146: \textit{Weight:-2.789}, Method: Candidate-Rank\\
There once was a girl named Gwyn,
Who felt a strange presence on her skin. 
It started out one day, 
She went outside to play, 
She walked through the forest and fell in. \\ \vspace{0.1pt}

147: \textit{Leader:-2.952}, Method: Candidate-Rank\\
There was a lieutenant named Kay,
Who led a small army on her way. 
When she arrived to fight, 
She was struck by a light, 
And she fell down and broke her okay. \\ \vspace{0.1pt}

148: \textit{Union:-3.085}, Method: Candidate-Rank\\
There was a fierce teacher named Jacque,
Who sought out her students for a break. 
When she returned to school, 
She was struck by her cool, 
But she knew she was doing it fake. \\ \vspace{0.1pt}

149: \textit{Home:-2.641}, Method: Candidate-Rank\\
There was a smart grandma named Dot,
Who had a small garden on her lot. 
She wanted a backyard, 
And we went to the yard, 
And we sat down and made our plot. \\ \vspace{0.1pt}

150: \textit{Child:-2.768}, Method: Candidate-Rank\\
There was a nervous girl named Grace,
Who put a big smile on our face. 
She was like a girlfriend, 
She was the perfect friend, 
It was great to have a female space. \\ \vspace{0.1pt}

151: \textit{Cheat:-2.800}, Method: Candidate-Rank\\
There was a hustler named Kay,
Who put all her money in a play. 
She wanted a boyfriend, 
Which she got in the end, 
And that is the story of this day. \\ \vspace{0.1pt}

152: \textit{Time:-2.733}, Method: Candidate-Rank\\
There was a wise doctor named Renee,
Who took a young woman on her way. 
When she came to someone, 
She was told by her son, 
That the person she saw was a stray. \\ \vspace{0.1pt}

153: \textit{Hope:-2.822}, Method: Candidate-Rank\\
There was a brave girl named Renee,
Who helped a young lady on her way. 
When she arrived to work, 
She was told by a clerk, 
That the woman she saw was a stray. \\ \vspace{0.1pt}

154: \textit{Impressive:-2.930}, Method: Candidate-Rank\\
There was a artist named Kay,
Who helped a young lady on her way. 
When she arrived to work, 
She was told by a clerk, 
That the woman she saw was a stray. \\ \vspace{0.1pt}

155: \textit{Flower:-2.815}, Method: Candidate-Rank\\
There was a lady named Brande,
Who cut a red ribbon on my hand. 
It was for her birthday, 
It was the perfect day, 
So I had to get down on the sand. \\ \vspace{0.1pt}

156: \textit{Random:-2.992}, Method: Candidate-Rank\\
There once was a girl named Kai,
Who stuck out her fingers for a guy. 
When she started to talk, 
She was able to walk, 
So she had to sit down on the fly. \\ \vspace{0.1pt}


==> deep_speare_poem.tex <==
1:  Method: Deep-Speare\\
There once was a judge named Larue, 
Was just found that her thought she was too, 
Herself on the jelly, 
To sex in her belly, 
So and what but the same things were true.\\ \vspace{0.1pt}

2:  Method: Deep-Speare\\
There once was a woman named Kay, 
Went for as he was two and they play, 
But he said she just hit, 
I see that you do it, 
Got so but when they thought that one day.\\ \vspace{0.1pt}

3:  Method: Deep-Speare\\
There was a honest judge named Dewitt, 
Screamed and as but she made men were fit, 
Did what that when he said, 
When he would put her head, 
But and I thought that she went on it.\\ \vspace{0.1pt}

4:  Method: Deep-Speare\\
There was a nasty surgeon named Rose, 
And but when he let out with the clothes, 
Did what but they have been, 
Knew what that she was one, 
Said and she was a man on her nose.\\ \vspace{0.1pt}

5:  Method: Deep-Speare\\
There was a hairy doctor named Yer, 
But was no one did what how he were, 
But she knew when he said, 
As the game and was bed, 
Out with a man and she fell in her.\\ \vspace{0.1pt}

6:  Method: Deep-Speare\\
There was a nervous man named Dewitt, 
A knew but was being always hit, 
But he had they have done, 
And she never no one, 
And he thought she said so they have it.\\ \vspace{0.1pt}

7:  Method: Deep-Speare\\
There was a honest butcher named Yer, 
High and but knew as who tried to ter, 
What and but it thought he, 
She went out on a sea, 
He said one that she was lean on her.\\ \vspace{0.1pt}

8:  Method: Deep-Speare\\
There was a stupid girl named Susann, 
Tried to drunk when her hair from the sun, 
He flew into his head, 
When then she let her bed, 
He said that she thought it went on one.\\ \vspace{0.1pt}

9:  Method: Deep-Speare\\
There was a bright surgeon named Ambrose, 
Was so who but when she made her clothes, 
When her body grew more, 
He went back in the door, 
He came out with a man in my nose.\\ \vspace{0.1pt}

10:  Method: Deep-Speare\\
There was a surgeon named Liane, 
But who was then came back to the sun, 
But a game and she said, 
When she cut off his head, 
When he got out and he went on one.\\ \vspace{0.1pt}

11:  Method: Deep-Speare\\
There was a bright doctor named Chan, 
But and wished who wore no it did been, 
The night that was away, 
He had a very day, 
And she knew what he thought she had one.\\ \vspace{0.1pt}

12:  Method: Deep-Speare\\
There was a lucky farmer named Ted, 
Was wished who never married a wed, 
As that she had a life, 
She had love to his wife, 
And so what he would see that he said.\\ \vspace{0.1pt}

13:  Method: Deep-Speare\\
There was a sexy farmer named Ted, 
Who was a man who played round his head, 
But he had a no wit, 
And but when he let it, 
You think that she did one that she said.\\ \vspace{0.1pt}

14:  Method: Deep-Speare\\
There was a shy farmer named Dewitt, 
Who knew so she never have been hit, 
Then married a teacher, 
He was by a creature, 
But he had no one that she had it.\\ \vspace{0.1pt}

15:  Method: Deep-Speare\\
There was a lady named Renee, 
Her pair that she fell back from a way, 
When he cried out a bit, 
But and when they put it, 
Went out and he flew up in one day.\\ \vspace{0.1pt}

16:  Method: Deep-Speare\\
There once was a farmer named Dewitt, 
But who knew that they got quite a hit, 
She had nothing could play, 
Very every day, 
That he had no one he went in it.\\ \vspace{0.1pt}

17:  Method: Deep-Speare\\
There was a sexy man named Stan, 
But found white who once played in a sun, 
And but he looked so for, 
Thought he was very more, 
Out and the ape was a man on one.\\ \vspace{0.1pt}

18:  Method: Deep-Speare\\
There was a sexy girl named Ann, 
Took his mother went out on the sun, 
Salts that she had a wit, 
And when that he knew it, 
Was so and she thought he had a one.\\ \vspace{0.1pt}

19:  Method: Deep-Speare\\
There was a shy boy named Dewitt, 
As but who knew he had on his wit, 
And then from a twenty, 
She went out a penny, 
Was more and who thought she sat on it.\\ \vspace{0.1pt}

20:  Method: Deep-Speare\\
There was a shy doctor named Ed, 
Who thought was no who knew that he said, 
But when he had a fun, 
Swallowed a trousers one, 
But and they put her toes in his head.\\ \vspace{0.1pt}

21:  Method: Deep-Speare\\
There was a lucky lady named Anne, 
Was so who had still came in the sun, 
So I knew as she tried, 
In all night and he died, 
And now when he said can have one.\\ \vspace{0.1pt}

22:  Method: Deep-Speare\\
There was a shy doctor named Yer, 
Out that who tried but she had a stir, 
As he played in his head, 
He was so that she said, 
And they have no something to put her.\\ \vspace{0.1pt}

23:  Method: Deep-Speare\\
There was a honest man named Ed, 
And who knew that he found on his head, 
She was much fatter than, 
But he might have no one, 
But who asked what to think that she said.\\ \vspace{0.1pt}

24:  Method: Deep-Speare\\
There was a serious girl named Freda, 
Had no girlfriend who thought that he said, 
But the ape on a chair, 
She cried off in a air, 
And so she found her toes on his head.\\ \vspace{0.1pt}

25:  Method: Deep-Speare\\
There was a skinny grandma named Yer, 
As who thought that she found it was stir, 
And he rode on a flies, 
But and he was a size, 
But the old man that she sat on her.\\ \vspace{0.1pt}

26:  Method: Deep-Speare\\
There was a silly man named Dewitt, 
Who was once took his man in a wit, 
That he lay on his head, 
With a husband she said, 
She just so he wanted to have it.\\ \vspace{0.1pt}

27:  Method: Deep-Speare\\
There was a wise tailor named Yer, 
Said and who thought he never prefer, 
Fell out from the stable, 
That what she was able, 
Not with a things that she went on her.\\ \vspace{0.1pt}

28:  Method: Deep-Speare\\
There was a smart doctor named Dyan, 
And had a far till his tooth was been, 
Who did so as he said, 
That she fell on his head, 
But he thought that she went out to one.\\ \vspace{0.1pt}

29:  Method: Deep-Speare\\
There was a wise farmer named Kay, 
Knew he who said that he once no me, 
His fish in a jelly, 
She cried up a belly, 
Went out and she shot out in the sea.\\ \vspace{0.1pt}

30:  Method: Deep-Speare\\
There was a designer named Yer, 
Who lay on his belly as a stir, 
When she started to bed, 
He fell back in his head, 
She was discovered a flat on her.\\ \vspace{0.1pt}

31:  Method: Deep-Speare\\
There was a lady named Marianne, 
Found a game who had never did been, 
As who wished he were wed, 
And he knew that she said, 
And she discovered a man that one.\\ \vspace{0.1pt}

32:  Method: Deep-Speare\\
There was a chunky man named Dewitt, 
But who was so they played in the hit, 
He discovered a game, 
That he received his name, 
She had a one that she went on it.\\ \vspace{0.1pt}

33:  Method: Deep-Speare\\
There once was a lady named Saran, 
It knew that she went out from the sun, 
From the night and away, 
When he wanted a day, 
But he thought that she started to one.\\ \vspace{0.1pt}

34:  Method: Deep-Speare\\
There was a harsh girl named Renee, 
High and who wished she had how to stay, 
But when she came his flies, 
He flew out in a size, 
But and when he went out in one day.\\ \vspace{0.1pt}

35:  Method: Deep-Speare\\
There was a quiet girl named Yer, 
But I knew till she thought they were stir, 
That she came into sight, 
So but he struck a light, 
Out and her size that he sat at her.\\ \vspace{0.1pt}

36:  Method: Deep-Speare\\
There was a wise woman named Larue, 
Fell on the bath when he started to, 
I found that she was dead, 
Was the ape in a bed, 
And he said what she thought it is true.\\ \vspace{0.1pt}

37:  Method: Deep-Speare\\
There was a brave man named Dewitt, 
Who tried but she had no that was hit, 
So as she pulled his bed, 
That he fell round his head, 
When he was a happened to put it.\\ \vspace{0.1pt}

38:  Method: Deep-Speare\\
There once was a liar named Jed, 
For and then but they came from his bed, 
She fell up in a sun, 
And so he had a one, 
When he wanted to sit in my head.\\ \vspace{0.1pt}

39:  Method: Deep-Speare\\
There was a humble woman named Yer, 
Was sang what but who knew what they were, 
Till who wanted to be, 
But and she thought that he, 
He said no one that she went to her.\\ \vspace{0.1pt}

40:  Method: Deep-Speare\\
There was a brave general named Jed, 
Once wished who was had it tried to bed, 
But she said what no fear, 
He went on a career, 
He was so that she fell in his head.\\ \vspace{0.1pt}

41:  Method: Deep-Speare\\
There was a neat lady named Yer, 
Wished was no just did what as they were, 
He married his teacher, 
As she had a creature, 
He thought that she had a tight on her.\\ \vspace{0.1pt}

42:  Method: Deep-Speare\\
There was a neat boy named Dewitt, 
A very thing who had quite a wit, 
He always never been, 
But as she said no one, 
She couldn't do anything in it.\\ \vspace{0.1pt}

43:  Method: Deep-Speare\\
There was a chunky man named Dewitt, 
The sea and then but when the big bit, 
He went out in a car, 
Black and he had a far, 
One when they do anything in it.\\ \vspace{0.1pt}

44:  Method: Deep-Speare\\
There was a hairy girl named Ruthann, 
But who found that she rode at the sun, 
As each night in his bed, 
He did no so he said, 
So they thought that she had it in one.\\ \vspace{0.1pt}

45:  Method: Deep-Speare\\
There was a hairy lady named Yer, 
As but who once fell up as a stir, 
So he played on his head, 
When he asked to his bed, 
She said no one that she went on her.\\ \vspace{0.1pt}

46:  Method: Deep-Speare\\
There was a skinny girl named Yer, 
Declared who was no men and they were, 
Wished he could never fit, 
But what that she did it, 
She knew nothing one that he shocked her.\\ \vspace{0.1pt}

47:  Method: Deep-Speare\\
There was a hairy boy named Stan, 
In the bath so they flew through a sun, 
At the day for his bought, 
At a night and his thought, 
So he never no time he was one.\\ \vspace{0.1pt}

48:  Method: Deep-Speare\\
There was a honest butcher named Yer, 
Up for his couple who had he were, 
He had in his offspring, 
But that she was a thing, 
Cos she just lean on a man in her.\\ \vspace{0.1pt}

49:  Method: Deep-Speare\\
There was a chunky man named Dewitt, 
Smiled as she took the ape was a bit, 
But she played on a jack, 
For and when he came back, 
But to girls and he went up in it.\\ \vspace{0.1pt}

50:  Method: Deep-Speare\\
There was a wise butcher named Dewitt, 
Said but who thought she was quite a wit, 
When she played in a shout, 
And but then he fell out, 
And one when he started to put it.\\ \vspace{0.1pt}

51:  Method: Deep-Speare\\
There once was a woman named Ruthann, 
But who was a plaster faster than, 
She had having a wit, 
Was so that he knew it, 
And so but he came out and had one.\\ \vspace{0.1pt}

52:  Method: Deep-Speare\\
There was a serious boy named Mose, 
In a pair and once fell in a rose, 
She knew what he was wed, 
And she asked with his head, 
Then he said to have one of my nose.\\ \vspace{0.1pt}

53:  Method: Deep-Speare\\
There once was a dentist named Renee, 
As but who always was jumping they, 
She thought he had a bit, 
So but when he found it, 
And when she would get out in one day.\\ \vspace{0.1pt}

54:  Method: Deep-Speare\\
There was a bright surgeon named Renee, 
A shout and then came off for halfway, 
That he cried off his flies, 
She went out for a size, 
Said and when they turned out from one day.\\ \vspace{0.1pt}

55:  Method: Deep-Speare\\
There was a wise boy named Dewitt, 
Screamed so but was wished he had to fit, 
Career who never were, 
As that she sat on her, 
And who thought she made her lean on it.\\ \vspace{0.1pt}

56:  Method: Deep-Speare\\
There was a skinny man named Dewitt, 
But and who declared he had a fit, 
But who wished he was wed, 
Had no love that she said, 
Was just so things that she sat on it.\\ \vspace{0.1pt}

57:  Method: Deep-Speare\\
There was a butcher named Dianne, 
But who did what and smiled as she run, 
Cried out from the ceiling, 
But that he was feeling, 
So what and he knew that she had one.\\ \vspace{0.1pt}

58:  Method: Deep-Speare\\
There was a wise warrior named Freda, 
Jumping who tried and played from his head, 
Who went out on a lot, 
And she had that he thought, 
So he was quite a man that she said.\\ \vspace{0.1pt}

59:  Method: Deep-Speare\\
There was a bright doctor named Dewitt, 
Twice in the ball who played with a wit, 
So she had in his nose, 
He had all his clients, 
But he said a one that she knew it.\\ \vspace{0.1pt}

60:  Method: Deep-Speare\\
There once was a girl named Georgann, 
The sea and she fell back from a sun, 
In that he rode away, 
But he very next day, 
When it discovered a thing was one.\\ \vspace{0.1pt}

61:  Method: Deep-Speare\\
There was a boring man named Dewitt, 
But who wanted to get like a bit, 
And when what so she said, 
That he fell round his head, 
But so that he had him to put it.\\ \vspace{0.1pt}

62:  Method: Deep-Speare\\
There was a lucky girl named Leann, 
Who was as but who wished it was done, 
But when he asked no sir, 
He said that she gave her, 
How to see that she went out on one.\\ \vspace{0.1pt}

63:  Method: Deep-Speare\\
There was a lucky girl named Diane, 
And once fell in a day who was been, 
She had never been wed, 
But when asked that she said, 
And but he was not that he had one.\\ \vspace{0.1pt}

64:  Method: Deep-Speare\\
There was a funny girl named Renee, 
Fell in but and wished he was halfway, 
When he took a funny, 
Got out of the money, 
For and but when she cried out one day.\\ \vspace{0.1pt}

65:  Method: Deep-Speare\\
There was a stupid girl named Renee, 
Tool and who knew that he went to stay, 
She pulled out from his flies, 
He had her very size, 
Was so she got turned out that one day.\\ \vspace{0.1pt}

66:  Method: Deep-Speare\\
There was a stupid lady named Yer, 
Knew who was what to things but they were, 
But I never tell me, 
She said to the thing he, 
He let the girls in confirming her.\\ \vspace{0.1pt}

67:  Method: Deep-Speare\\
There was a funny grandpa named Stan, 
Been wished and frequently might have been, 
But then they found away, 
He had never all day, 
But he knew when they went out that one.\\ \vspace{0.1pt}

68:  Method: Deep-Speare\\
There was a dazzling girl named Kay, 
Was tho but he said and they knew he, 
Swim in every night, 
That she fell in a light, 
That one she went out under the sea.\\ \vspace{0.1pt}

69:  Method: Deep-Speare\\
There was a nasty surgeon named Rose, 
Who had a thought that she pulled her toes, 
When he wanted to bed, 
But he fell in his head, 
A man when she went out in her nose.\\ \vspace{0.1pt}

70:  Method: Deep-Speare\\
There was a bright boy named Dewitt, 
Was as who thought she was quite a fit, 
Had a parrot were wed, 
But he fell in his head, 
But he said no one I can put it.\\ \vspace{0.1pt}

71:  Method: Deep-Speare\\
There was a hairy man named Ambrose, 
Slipped from the ball who fell in his toes, 
That she had he was true, 
But when he had a crew, 
That she was a shot up with his nose.\\ \vspace{0.1pt}

72:  Method: Deep-Speare\\
There was a honest liar named Hugh, 
Was his bridge who fell back in the crew, 
That she made her jelly, 
They put out his belly, 
She got so but they shot him in true.\\ \vspace{0.1pt}

73:  Method: Deep-Speare\\
There was a wise woman named Yer, 
Out on the sea and had he would stir, 
So but what that she said, 
When the ape with his head, 
And she thought that he went up at her.\\ \vspace{0.1pt}

74:  Method: Deep-Speare\\
There was a grandma named Marquerite, 
Was as for who wished he was so neat, 
But he started to can, 
Out but she like a man, 
That she wanted to sit on her feet.\\ \vspace{0.1pt}

75:  Method: Deep-Speare\\
There was a funky man named Dewitt, 
The couple who had was quite a wit, 
Knew that he in his life, 
Till but she gave his wife, 
And she said just so he can do it.\\ \vspace{0.1pt}

76:  Method: Deep-Speare\\
There was a sexy witch named Freda, 
As who looked so he played in a red, 
He flew into his head, 
But when she pulled his bed, 
Then and fell in a think that she said.\\ \vspace{0.1pt}

77:  Method: Deep-Speare\\
There was a chunky lady named Freda, 
Who tried that he had into his head, 
So he would get a bit, 
But and then once on it, 
And but she was no one that she said.\\ \vspace{0.1pt}

78:  Method: Deep-Speare\\
There was a quiet girl named Joanne, 
She was wished who always never been, 
And when he had a ball, 
But who was very small, 
Said so but she thought that he had one.\\ \vspace{0.1pt}

79:  Method: Deep-Speare\\
There was a quiet girl named Yer, 
But she started to a control ter, 
He went off in his bed, 
As he took off his head, 
But and she said so I used to her.\\ \vspace{0.1pt}

80:  Method: Deep-Speare\\
There once was a doctor named Mose, 
Who had a maid and she kicked his toes, 
So that she was jelly, 
Cried up on her belly, 
And but when they would sit on her nose.\\ \vspace{0.1pt}

81:  Method: Deep-Speare\\
There was a quiet boy named Dewitt, 
A tooth declared who married a wit, 
Had often always play, 
When but he was one day, 
And she thought he was cold and had it.\\ \vspace{0.1pt}

82:  Method: Deep-Speare\\
There was a bright doctor named Renee, 
Game who could swim that she was away, 
He decided to fit, 
Who thought that he knew it, 
But and now she reached out of one day.\\ \vspace{0.1pt}

83:  Method: Deep-Speare\\
There once was a girl named Renee, 
Who said and then out of the old way, 
She had never no wit, 
But no that he knew it, 
So but when he could have that one day.\\ \vspace{0.1pt}

84:  Method: Deep-Speare\\
There was a neat boy named Dewitt, 
Who screamed so she thought that he was hit, 
From the back with a shout, 
Then he said to get out, 
And but one might have been just in it.\\ \vspace{0.1pt}

85:  Method: Deep-Speare\\
There was a neat girl named Margarete, 
Once was but who wished he had a neat, 
Thought that she was so quite, 
So that she pulled her tight, 
Went out from the old man in her feet.\\ \vspace{0.1pt}

86:  Method: Deep-Speare\\
There was a rude girl named Dianne, 
For a drunk and she rode from the sun, 
On the back from his flies, 
Now he fell in his size, 
And he went into a head on one.\\ \vspace{0.1pt}

87:  Method: Deep-Speare\\
There was a hairy doctor named Rose, 
Who declared it thought that when he goes, 
She turned out on a flies, 
Who went up from the size, 
But and he made his up with her nose.\\ \vspace{0.1pt}

88:  Method: Deep-Speare\\
There was a doctor named Lianne, 
Couple who wished and never had been, 
Now till how as she said, 
That he played round his head, 
But when they thought that he had to one.\\ \vspace{0.1pt}

89:  Method: Deep-Speare\\
There was a nervous man named Dewitt, 
Thought that who was the ape had a hit, 
But she wanted to bout, 
When he tried to get out, 
Then and he said but she sat on it.\\ \vspace{0.1pt}

90:  Method: Deep-Speare\\
There was a bright surgeon named Dewitt, 
Tried but she took his dick was a hit, 
He ran up from a flies, 
That he fell in his size, 
So and but no one that she knew it.\\ \vspace{0.1pt}

91:  Method: Deep-Speare\\
There once was a surgeon named Dewitt, 
Could never found that she was no wit, 
And but he had a life, 
What as she said his wife, 
But then and a things that he knew it.\\ \vspace{0.1pt}

92:  Method: Deep-Speare\\
There once was a surgeon named Dewitt, 
Wished who was grew as he had his bit, 
One and but when a wed, 
She pulled out in his head, 
She said to things that he would do it.\\ \vspace{0.1pt}

93:  Method: Deep-Speare\\
There was a bright cleaner named Yer, 
A maid who were filled with his mouth were, 
When he wanted to sight, 
But and she let one light, 
Flew out in the size that he shocked her.\\ \vspace{0.1pt}

94:  Method: Deep-Speare\\
There was a quiet girl named Yer, 
Who was lived in as and wished they were, 
He never had a wit, 
When asked how she knew it, 
She said the ape was a man on her.\\ \vspace{0.1pt}

95:  Method: Deep-Speare\\
There was a quiet girl named Kay, 
Brother and once fell out on the way, 
As he went in a head, 
So that she had a bed, 
And he said that she cried out one day.\\ \vspace{0.1pt}

96:  Method: Deep-Speare\\
There was a woman named Leann, 
But was no who thought that she got been, 
And but he had a ears, 
Had a couple of years, 
She never still all day he was one.\\ \vspace{0.1pt}

97:  Method: Deep-Speare\\
There was a smart woman named Bridgette, 
Who was as but she flew near the heat, 
He discovered a grin, 
Who thought he was so thin, 
No one that she fell out with her feet.\\ \vspace{0.1pt}

98:  Method: Deep-Speare\\
There was a chunky boy named Ted, 
Was so as he knew that she would bed, 
As but he was no doubt, 
And but when they went out, 
That one white and fell lean on her head.\\ \vspace{0.1pt}

99:  Method: Deep-Speare\\
There was a bright lady named Joann, 
Who wished she had never cannot been, 
And but as I would bid, 
When the night and he did, 
But so he knew that she could have one.\\ \vspace{0.1pt}

100:  Method: Deep-Speare\\
There was a bright lady named Kay, 
Was as who wished she never would stay, 
Till when he had a bit, 
And but that he did it, 
But and now she had it was one day.\\ \vspace{0.1pt}

101:  Method: Deep-Speare\\
There once was a liar named Saran, 
As was wished who had a tooth was been, 
He cried out by a shoe, 
But she had to be true, 
So but she knew when he went in one.\\ \vspace{0.1pt}

102:  Method: Deep-Speare\\
There once was a doctor named Mose, 
But who was once tried into her clothes, 
When she came off and he, 
When he fell from the sea, 
And let one she went out in her nose.\\ \vspace{0.1pt}

103:  Method: Deep-Speare\\
There was a skinny man named Dewitt, 
Who wished he never got quite a wit, 
But she fish was a pin, 
When they once made him thin, 
And but he knew that she went on it.\\ \vspace{0.1pt}

104:  Method: Deep-Speare\\
There was a chunky man named Stan, 
That who wanted to swim on the sun, 
He went out from his crack, 
Then he fell from the back, 
And then came to his shot out of one.\\ \vspace{0.1pt}

105:  Method: Deep-Speare\\
There was a smart woman named Louanne, 
For a couple who knew he had been, 
And but wished he was not, 
But her husband she thought, 
That she was up on a man in one.\\ \vspace{0.1pt}

106:  Method: Deep-Speare\\
There was a smart man named Dewitt, 
Once knew who found she was by a wit, 
So that she took her head, 
But he wanted to bed, 
But with a thought that he sat on it.\\ \vspace{0.1pt}

107:  Method: Deep-Speare\\
There once was a boy named Dewitt, 
He thought that his tooth was being hit, 
But she had a divorce, 
But she cried out of course, 
And was a thing he had to put it.\\ \vspace{0.1pt}

108:  Method: Deep-Speare\\
There was a shy farmer named Dewitt, 
Took her head was when he got his bit, 
One night in his yellow, 
He married a fellow, 
She went out in a man and had it.\\ \vspace{0.1pt}

109:  Method: Deep-Speare\\
There was a grandma named Margarete, 
Who and smiled as she knew he was neat, 
That she rode out a flies, 
But he flew from the size, 
Discovered a shot out of his feet.\\ \vspace{0.1pt}

110:  Method: Deep-Speare\\
There once was a cleaner named Rosanne, 
As who smiled when she fell through a sun, 
But then he pulled his head, 
He in his mother said, 
And but to think that she went in one.\\ \vspace{0.1pt}

111:  Method: Deep-Speare\\
There was a nervous boy named Ambrose, 
Tried who married a woman and rose, 
And till his mother said, 
But when he pulled her head, 
But she thought that he was by her nose.\\ \vspace{0.1pt}

112:  Method: Deep-Speare\\
There was a brave man named Dewitt, 
And tho who wished she was very bit, 
But who played with a blue, 
And but he had a true, 
So he knew that she just to put it.\\ \vspace{0.1pt}

113:  Method: Deep-Speare\\
There was a general named Dewitt, 
So who had a thought that she was hit, 
From the ape in a flies, 
But he had at his size, 
And but he said no that she knew it.\\ \vspace{0.1pt}

114:  Method: Deep-Speare\\
There was a brave woman named Roxanne, 
Wished was a swore who never had been, 
The game and often said, 
That and he had his head, 
But I think that she thought he was one.\\ \vspace{0.1pt}

115:  Method: Deep-Speare\\
There was a wise lady named Georgann, 
Tho who knew that he wanted to run, 
And she said for a wit, 
When she never find it, 
For and but when he thought it was one.\\ \vspace{0.1pt}

116:  Method: Deep-Speare\\
There was a honest man named Dewitt, 
And who lived that she was very wit, 
Said but she had a red, 
And he cut off his head, 
But he was getting a lean on it.\\ \vspace{0.1pt}

117:  Method: Deep-Speare\\
There was a wise woman named Liane, 
As who knew he came out by the sun, 
The affair with her eyes, 
And had out of his size, 
Then and he went for a man of one.\\ \vspace{0.1pt}

118:  Method: Deep-Speare\\
There was a butcher named Maryanne, 
And who found that he had never been, 
He offered to his bed, 
Got but and so she said, 
But cos she might have been went on one.\\ \vspace{0.1pt}

119:  Method: Deep-Speare\\
There was a wise butcher named Stan, 
But who when they came off from the run, 
And then back from the flies, 
He turned out of a size, 
But and I knew that he fell in one.\\ \vspace{0.1pt}

120:  Method: Deep-Speare\\
There was a silly boy named Pete, 
Was wished but who had never was neat, 
What who could no what were, 
He knew that she found her, 
He thought that she fell up on her feet.\\ \vspace{0.1pt}

121:  Method: Deep-Speare\\
There was a funky grandma named Dann, 
She knew who wished he had never been, 
Said what but he was soon, 
To the swim in a moon, 
But and who fell in the edge of one.\\ \vspace{0.1pt}

122:  Method: Deep-Speare\\
There was a nasty bully named Jed, 
Was who thought that she fell like a red, 
So but he blew his shoe, 
Was a terrible crew, 
But then he found her toes in his head.\\ \vspace{0.1pt}

123:  Method: Deep-Speare\\
There once was a bully named Jed, 
So as that they fell down from his head, 
Then they played from the strife, 
When he tried to his wife, 
And she got a one and when he said.\\ \vspace{0.1pt}

124:  Method: Deep-Speare\\
There was a quiet author named Kay, 
Was no men but his dick came away, 
She went back in a sport, 
When he fell in a short, 
But he said it got very one day.\\ \vspace{0.1pt}

125:  Method: Deep-Speare\\
There was a brave woman named Renee, 
Was who met a young ape in a tree, 
It and when she was dead, 
But when they let her head, 
She said if they get up from the sea.\\ \vspace{0.1pt}

126:  Method: Deep-Speare\\
There was a serious girl named Kay, 
Who was very first hymns as they play, 
That he rode on a ball, 
And she had very small, 
And he knew that she had all one day.\\ \vspace{0.1pt}

127:  Method: Deep-Speare\\
There was a lucky chef named Susann, 
Smiled as but once fell out in his run, 
She had fish like a bit, 
But he had a mind it, 
And he thought that she walked it on one.\\ \vspace{0.1pt}

128:  Method: Deep-Speare\\
There was a butcher named Renee, 
Shook out from the crew and came away, 
He fell back with a eyes, 
When she asked in her size, 
Said and but she went out from one day.\\ \vspace{0.1pt}

129:  Method: Deep-Speare\\
There was a wise chef named Maryanne, 
As who rode on her back from the sun, 
That she went out and hit, 
When but he could do it, 
But more far than he set out of one.\\ \vspace{0.1pt}

130:  Method: Deep-Speare\\
There was a serious man named Hugh, 
But who married a parrot had two, 
Knew that she had a red, 
And once fell in his head, 
But he said and she thought he was true.\\ \vspace{0.1pt}

131:  Method: Deep-Speare\\
There was a skinny boy named Dewitt, 
Was stung and as she had on his fit, 
So he tried like a grin, 
So that he had a thin, 
But that she found one who sat on it.\\ \vspace{0.1pt}

132:  Method: Deep-Speare\\
There was a bright cleaner named Dewitt, 
The party and never had a wit, 
When they knew she got quite, 
So that he was a light, 
When but the one that he went in it.\\ \vspace{0.1pt}

133:  Method: Deep-Speare\\
There was a general named Stan, 
For but who thought that she did they been, 
Till then he fell away, 
But at night in the day, 
That she was getting a man on one.\\ \vspace{0.1pt}

134:  Method: Deep-Speare\\
There was a wise lady named Susanne, 
Had a couple who wished she had been, 
Was much faster than not, 
In a cause that he thought, 
But he knew that she found it was one.\\ \vspace{0.1pt}

135:  Method: Deep-Speare\\
There was a silly lady named Yer, 
Knew he grew and but so how they were, 
They all in his knowledge, 
So he wrote a college, 
The bishop girls in confirming her.\\ \vspace{0.1pt}

136:  Method: Deep-Speare\\
There was a nervous dentist named Rose, 
So who said that she went off her toes, 
He came back to jelly, 
Them up in a belly, 
But and when they shot off in his nose.\\ \vspace{0.1pt}

137:  Method: Deep-Speare\\
There was a bright dentist named Renee, 
Who took out on the ape as a tree, 
When she gave him to bed, 
Then he fell in his head, 
He knew so she went up in the sea.\\ \vspace{0.1pt}

138:  Method: Deep-Speare\\
There was a nasty boy named Dewitt, 
But who thought that she came by a hit, 
She cried out of divorce, 
Then discovered a course, 
He knew one that he went to have it.\\ \vspace{0.1pt}

139:  Method: Deep-Speare\\
There was a bright dentist named Dewitt, 
Who went out was the ape on a wit, 
But he thought that she said, 
When the hair in his head, 
Up and discovered a man on it.\\ \vspace{0.1pt}

140:  Method: Deep-Speare\\
There was a humble liar named Hugh, 
Who was what he knew how I can you, 
Said but when they have done, 
That she never did one, 
That he thought she discovered a true.\\ \vspace{0.1pt}

141:  Method: Deep-Speare\\
There was a neat phony named Jed, 
So but when they shot out from a red, 
She got into a nose, 
If he put his clients, 
Could strung up with his head that he said.\\ \vspace{0.1pt}

142:  Method: Deep-Speare\\
There once was a cleaner named Stan, 
But who tried out to swim by a sun, 
He who went out from sight, 
With a sea and the light, 
He once discovered the size of one.\\ \vspace{0.1pt}

143:  Method: Deep-Speare\\
There was a funky woman named Freda, 
But who found his tooth was had a red, 
But wished he had no fun, 
So she thought that no one, 
He knew that she discovered her head.\\ \vspace{0.1pt}

144:  Method: Deep-Speare\\
There was a bright woman named Freda, 
But as they found there was being wed, 
Wished she had never been, 
And till what he did one, 
But who asked so she knew that he said.\\ \vspace{0.1pt}

145:  Method: Deep-Speare\\
There once was a witch named Maryanne, 
As for and when he died from the sun, 
And he fell on a lot, 
But she knew that it thought, 
That she discovered a man on one.\\ \vspace{0.1pt}

146:  Method: Deep-Speare\\
There was a skinny boy named Ed, 
Man but who had no one as she said, 
Can hit with a jelly, 
When he pulled his belly, 
He shot through my arse up in his head.\\ \vspace{0.1pt}

147:  Method: Deep-Speare\\
There once was a witch named Suzanne, 
As but who wished he had never been, 
But what the ape was wed, 
So who thought that she said, 
So he knew that she went out in one.\\ \vspace{0.1pt}

148:  Method: Deep-Speare\\
There was a grandma named Margarete, 
For but who wished he was very neat, 
When she wanted to bed, 
So that she saw her head, 
Think that he was discovered her feet.\\ \vspace{0.1pt}

149:  Method: Deep-Speare\\
There was a quiet teacher named Hugh, 
The wished who was mistake by a stew, 
Was a flat on his head, 
That she fell on her bed, 
High and she said the love that is true.\\ \vspace{0.1pt}

150:  Method: Deep-Speare\\
There was a serious man named Mose, 
Was once as he fell out in his clothes, 
But he knew so she said, 
But when they put her head, 
When the thing she went out in my nose.\\ \vspace{0.1pt}

151:  Method: Deep-Speare\\
There was a lady named Roseanne, 
Tho who once but the fish had a fun, 
Was so but she got been, 
Who and he was a thin, 
He thought that she would get out to one.\\ \vspace{0.1pt}

152:  Method: Deep-Speare\\
There was a hairy boy named Mose, 
A maid who had an ape in the clothes, 
He was up from his shoe, 
She had out from the crew, 
No one that she went out in his nose.\\ \vspace{0.1pt}

153:  Method: Deep-Speare\\
There once was a dentist named Ed, 
Was when he struck the back on his head, 
As she fell in a shout, 
Then she never got out, 
The captain and asked her mother said.\\ \vspace{0.1pt}

154:  Method: Deep-Speare\\
There was a bright man named Dewitt, 
And but who thought men were being fit, 
That she made to jelly, 
Went back from his belly, 
She came down and started to put it.\\ \vspace{0.1pt}

155:  Method: Deep-Speare\\
There was a honest woman named Yer, 
Sea and but when he wanted a stir, 
As she fell by without, 
The bath that she cried out, 
But and the same one was once at her.\\ \vspace{0.1pt}

156:  Method: Deep-Speare\\
There was a stupid woman named Kay, 
Was but just as she wanted a play, 
Who but he had a hit, 
She thought that I do it, 
And so that he shot out from one day.\\ \vspace{0.1pt}

157:  Method: Deep-Speare\\
There was a hairy man named Ambrose, 
Tried but one once was fell from her rose, 
She did that he was wed, 
She cried out from his head, 
He discovered a man on her nose.\\ \vspace{0.1pt}

158:  Method: Deep-Speare\\
There was a honest man named Ned, 
Who smiled as she fell down in a bed, 
Then he had him to wed, 
Out and but that he said, 
When no sure to her hair on his head.\\ \vspace{0.1pt}

159:  Method: Deep-Speare\\
There was a doctor named Dewitt, 
Was at one that whose mouth had a wit, 
Or then when the jelly, 
Fell into her belly, 
But and when it made him to do it.\\ \vspace{0.1pt}

160:  Method: Deep-Speare\\
There once was a girl named Maryanne, 
As who found but his tooth had was fun, 
On the bath that he said, 
That she fell on his head, 
And when she knew he was died of one.\\ \vspace{0.1pt}

161:  Method: Deep-Speare\\
There was a silly lady named Yer, 
Was once who kicked a dance and he stir, 
That he had a penis, 
She grew and so nothing, 
So that she made cider inside her.\\ \vspace{0.1pt}

162:  Method: Deep-Speare\\
There was a stupid man named Dewitt, 
As that who wished she had just been hit, 
As what how till he took, 
Her husband he would look, 
Thought it but the same that she knew it.\\ \vspace{0.1pt}

163:  Method: Deep-Speare\\
There was a humble man named Stan, 
The sea and but then played from the sun, 
Affair with a fellow, 
He took all his clients, 
And now for a size that he was one.\\ \vspace{0.1pt}

164:  Method: Deep-Speare\\
There was a brave man named Dewitt, 
Tho who once declared he had a bit, 
For but one when they know, 
By a parrot and no, 
But that she said no that I knew it.\\ \vspace{0.1pt}

165:  Method: Deep-Speare\\
There once was a writer named Dewitt, 
Was no game who thought she had a bit, 
That she went in a sea, 
When he said one when he, 
I never get out who would fix it.\\ \vspace{0.1pt}

166:  Method: Deep-Speare\\
There was a journalist named Roseanne, 
Out and she did that he had a fun, 
When he wanted to shit, 
She said when I do it, 
And then you see that his thing to one.\\ \vspace{0.1pt}

167:  Method: Deep-Speare\\
There was a tailor named Dewitt, 
Who tried that but she had got a bit, 
And when he struck them wide, 
Then and night when he died, 
Was one now she said what they do it.\\ \vspace{0.1pt}

168:  Method: Deep-Speare\\
There was a sexy lady named Anne, 
With the bath till then came from a sun, 
Then cut off on a red, 
That he fell in his head, 
But and found that she knew he was one.\\ \vspace{0.1pt}

169:  Method: Deep-Speare\\
There was a chunky boy named Ed, 
But who seduced the girl with a red, 
That she fell in his head, 
When he played from his bed, 
But and wanted to be that he said.\\ \vspace{0.1pt}

170:  Method: Deep-Speare\\
There was a bright doctor named Ambrose, 
Was salts that she cried off through her toes, 
On the ape in a bed, 
But he jumped on a head, 
But she thought he went off with his nose.\\ \vspace{0.1pt}

171:  Method: Deep-Speare\\
There was a humble liar named Thuy, 
His head who was mistake in a stew, 
And she met for a lad, 
When I found that he had, 
So one as she thought that he was true.\\ \vspace{0.1pt}

172:  Method: Deep-Speare\\
There was a wise lady named Larue, 
Did one who once had a bit of blue, 
Then and she never hit, 
But no that he knew it, 
Was so but and found that he was true.\\ \vspace{0.1pt}

173:  Method: Deep-Speare\\
There was a wise woman named Yer, 
Who thought she was once wanted a stir, 
But for a doctor said, 
But when he gave his head, 
Who got no one that he fell in her.\\ \vspace{0.1pt}

174:  Method: Deep-Speare\\
There was a honest man named Stan, 
As but who wished they never had been, 
Then at course he was wed, 
Found that she had his head, 
Was so that she said he would have one.\\ \vspace{0.1pt}

175:  Method: Deep-Speare\\
There was a wise liar named Dewitt, 
Said as who wished I might have a bit, 
And so that he had been, 
She had never no one, 
And so she thought that he went on it.\\ \vspace{0.1pt}

176:  Method: Deep-Speare\\
There was a wise liar named Leann, 
Couple and who wished he had have been, 
But that she had a bit, 
Then and when he found it, 
She said when they never have at one.\\ \vspace{0.1pt}

177:  Method: Deep-Speare\\
There was a brave man named Dewitt, 
Who found that she had an very wit, 
But a fish from his shoe, 
But he swallowed a true, 
He thought that she wanted to put it.\\ \vspace{0.1pt}

178:  Method: Deep-Speare\\
There was a humble liar named Yer, 
High and but they found his tooth had were, 
Who wished he had was true, 
But and thought what he knew, 
That she was so that she would put her.\\ \vspace{0.1pt}

179:  Method: Deep-Speare\\
There once was a liar named Yer, 
But and who knew he did what they were, 
He flew up from a flies, 
She took out in his size, 
But and no one that she went on her.\\ \vspace{0.1pt}

180:  Method: Deep-Speare\\
There was a grandma named Marguerite, 
And was thought that who knew men was neat, 
He came back in a bed, 
So she fell on her head, 
He looked so she went up on her feet.\\ \vspace{0.1pt}

181:  Method: Deep-Speare\\
There was a nervous boy named Ambrose, 
Who screamed as when they flew through his toes, 
Wished he was very wed, 
So she knew that he said, 
But a thought that she was quite a nose.\\ \vspace{0.1pt}

182:  Method: Deep-Speare\\
There was a nasty dentist named Kay, 
Was smiled who he shook out of his tree, 
And but he got a jack, 
Said and then she came back, 
But they go to get down from a sea.\\ \vspace{0.1pt}

183:  Method: Deep-Speare\\
There was a hairy boy named Ed, 
Who smiled as he went off on his bed, 
When he made a jelly, 
Took up from his belly, 
And so one that they fell with her head.\\ \vspace{0.1pt}

184:  Method: Deep-Speare\\
There was a bright dentist named Dianne, 
On the sea who would ran on the sun, 
As she rode from a flies, 
As then played from a size, 
But and he was so that he had one.\\ \vspace{0.1pt}

185:  Method: Deep-Speare\\
There was a bright dentist named Dewitt, 
For who had was he bit on a hit, 
So but as he was well, 
And but one that she fell, 
Went out with a man and she had it.\\ \vspace{0.1pt}

186:  Method: Deep-Speare\\
There was a skinny girl named Freda, 
But no thought who had a tooth were red, 
He had never been wed, 
But he knew that she said, 
So one that she came up in her head.\\ \vspace{0.1pt}

187:  Method: Deep-Speare\\
There was a bright boy named Ambrose, 
Who till but once shook off in his clothes, 
When he got into bed, 
And so she pulled her head, 
And he said she get out in her nose.\\ \vspace{0.1pt}



==> human_poem.tex <==
1:  Method: Human Poets\\
There was an old man of Calcutta,
Who coated his tonsils with butter,
And converted his snore,
From a thunderous roar,
To a soft oleaginous mutter.\\ \vspace{0.1pt}

2:  Method: Human Poets\\
There was an old man of Melrose,
Who walked on the tips of his toes,
But they said it pleasant,
To see you at present,
You stupid old man of melrose.\\ \vspace{0.1pt}

3:  Method: Human Poets\\
There was a sick man of Tobago,
Who lived long on rice gruel and sago,
But at last to his bliss,
The physician said this,
To a roast leg of mutton you may go.\\ \vspace{0.1pt}

4:  Method: Human Poets\\
There was an old man with a Poker,
Who painted his face with red oker,
When they said a guy,
He made no reply,
But knocked them all down with his poker.\\ \vspace{0.1pt}

5:  Method: Human Poets\\
There was an old man of Peru,
Who never knew what he should do,
So he tore off his hair,
And behaved like a bear,
That intrinsic old man of peru.\\ \vspace{0.1pt}

6:  Method: Human Poets\\
There was a young curate called Lloyd,
Who was seldom if ever annoyed,
Although you might poke him,
You could never provoke him,
His sang was so terribly froid.\\ \vspace{0.1pt}

7:  Method: Human Poets\\
There was a young lady of Chichester,
Who made all the saints in their niches stir,
One morning at matins,
Her breasts in white satins,
Made the bishop of chichester’s britches stir.\\ \vspace{0.1pt}

8:  Method: Human Poets\\
There was a young plumber of Leigh,
Who was plumbing a girl by the sea,
Said the girl cease your plumbing,
I think someone’s coming,
Said the plumber still plumbing it’s me.\\ \vspace{0.1pt}

9:  Method: Human Poets\\
There was a young man from Kildare,
Who was doing his wife on the stair,
When the banister broke,
He just quickened his stroke,
And he finished her off in mid air.\\ \vspace{0.1pt}

10:  Method: Human Poets\\
There was a young girl of Uttoxeter,
Who noticed that men waved their cocks at her,
This would cause some surprises,
In nearby devizes,
But it’s what they all do in uttoxeter.\\ \vspace{0.1pt}

11:  Method: Human Poets\\
There was a young sailor named Bates,
Who danced the fandango on skates,
But a fall on his cutlass,
Rendered him nutless,
And practically useless on dates.\\ \vspace{0.1pt}

12:  Method: Human Poets\\
There was a young lady of Kent,
Who always said just what she meant,
People said she’s a dear,
So unique so sincere,
But they shunned her by common consent.\\ \vspace{0.1pt}

13:  Method: Human Poets\\
There once was a gal from glen Innes,
Who loved drinking brandy and guinness,
And she later got plenty,
Joined the navy at twenty,
And looked after the admiral’s pinnace.\\ \vspace{0.1pt}

14:  Method: Human Poets\\
There was an old man of the West,
Who wore a pale plum coloured vest,
When they said does it fit,
He replied not a bit,
That uneasy old man of the west.\\ \vspace{0.1pt}

15:  Method: Human Poets\\
There was a young lady called Clarice,
Who lived in the city of paris,
She wandered with sartre,
The streets of montmartre,
But married a chap called bert harris.\\ \vspace{0.1pt}

16:  Method: Human Poets\\
There once was a lady from Reno,
Who lost all her bucks playing keno,
So she lay on her back,
And opened her crack,
And now she owns half the casino.\\ \vspace{0.1pt}

17:  Method: Human Poets\\
There was a young man of Montrose,
Who had pockets in none of his clothes,
When asked by his lass,
Where he carried his brass,
He said darling I pay through the nose.\\ \vspace{0.1pt}

18:  Method: Human Poets\\
There once was a judge of Assize,
Whose bollocks were not the same size,
He’d look at the right,
With a gasp of delight,
But the left one brought tears to his eyes.\\ \vspace{0.1pt}

19:  Method: Human Poets\\
There was a young man from Laconia,
Whose mother in law had pneumonia,
He hoped for the worst,
And after march first,
They buried her neath a begonia.\\ \vspace{0.1pt}

20:  Method: Human Poets\\
There was a sad man from Montrose,
Whose love life was so full of woes,
For he loved nothing finer,
Than a good sixty niner,
But he always got shit up his nose.\\ \vspace{0.1pt}

21:  Method: Human Poets\\
There was an old person of Buda,
Whose conduct grew ruder and ruder,
Till at last with a hammer,
They silenced his clamour,
By smashing that person of buda.\\ \vspace{0.1pt}

22:  Method: Human Poets\\
There was a man from Capri,
Who tried to piss over a tree,
The tree was too high,
And it fell in his eye,
And now the poor bugger can’t see.\\ \vspace{0.1pt}

23:  Method: Human Poets\\
There was an old person of Leeds,
Whose head was infested with beads,
She sat on a stool,
And ate gooseberry fool,
Which agreed with that person of leeds.\\ \vspace{0.1pt}

24:  Method: Human Poets\\
There was an old man of the East,
Who gave all his children a feast,
But they all ate so much,
And their conduct was such,
That it killed that old man of the east.\\ \vspace{0.1pt}

25:  Method: Human Poets\\
There was an old farmer from Young,
Who was quite remarkably hung,
When cleaning the stable,
His member was able,
To serve as a fork for the dung.\\ \vspace{0.1pt}

26:  Method: Human Poets\\
There was a young fellow called Clyde,
Who once at a funeral was spied,
When asked who was dead,
He smilingly said,
No idea I just came for the ride.\\ \vspace{0.1pt}

27:  Method: Human Poets\\
There once was a blasphemous Colonel,
Whose oaths were obscene and infolonel,
The chaplain did protest,
But nobody noticed,
So he jotted them down in his jolonel.\\ \vspace{0.1pt}

28:  Method: Human Poets\\
There once was a fellow from Goshem,
Who took out his balls just to wash em,
His mother said jack,
If you don’t put em back,
I’ll tread on the buggers and squash em.\\ \vspace{0.1pt}

29:  Method: Human Poets\\
There was a good canon of Durham,
Who fished with a hook and a worrum,
Said the dean to the bishop,
I’ve brought a big fish up,
But I fear we may have to inter’m.\\ \vspace{0.1pt}

30:  Method: Human Poets\\
There was a young girl of Darjeeling,
Who danced with such exquisite feeling,
31:  Method: Human Poets\\
There was never a Sound,
For miles around,
Save of fly buttons hitting the ceiling,
,
32:  Method: Human Poets\\
There once was a naughty old Salmon,
Who maintained that he served god and mammon,
But please understand,
The poor fish was canned,
When he talked this nonsensical gammon.\\ \vspace{0.1pt}

33:  Method: Human Poets\\
There was a young woman from Thrace,
Whose corset was too tight to lace,
Her mother said nelly,
34:  Method: Human Poets\\
There’s more in your Belly,
Than ever went in through your face,
,
35:  Method: Human Poets\\
There once was a monarch of Spain,
Who was terribly naughty and vain,
When women were nigh,
He would open his fly,
And have them with sneers of disdain.\\ \vspace{0.1pt}

36:  Method: Human Poets\\
There was a small boy of Quebec,
Who was buried in snow to his neck,
When they said are you friz,
He replied yes I is,
But we don’t call this cold in quebec.\\ \vspace{0.1pt}

37:  Method: Human Poets\\
There was an old mickey called Cassidy,
Who was noted for impromptu mendacity,
When asked did he lie,
He replied to reply,
Would be to impugn his veracity.\\ \vspace{0.1pt}

38:  Method: Human Poets\\
There was a young person called Tate,
Who went out to dine at,
But I will not relate,
What that person named tate,
And his ate at.\\ \vspace{0.1pt}

39:  Method: Human Poets\\
There was a young lady from Purdbright,
Who never could quite get her turd right,
She only did shits,
In little round bits,
Just like a mouse or a bird might.\\ \vspace{0.1pt}

40:  Method: Human Poets\\
There was an old man of Bengal,
Who purchased a bat and a ball,
Some gloves and some pads,
It was one of his fads,
For he never played cricket at all.\\ \vspace{0.1pt}

41:  Method: Human Poets\\
There was a young monarch called Ed,
Who took mrs simpson to bed,
As they bounced up and down,
He said bugger the crown,
Give the thing to my brother instead.\\ \vspace{0.1pt}

42:  Method: Human Poets\\
There was an old man on some Rocks,
Who shut his wife up in a box,
When she said let me out,
He exclaimed without doubt,
You will pass all your life in that box.\\ \vspace{0.1pt}

43:  Method: Human Poets\\
There was an old person of Ware,
Who rode on the back of a bear,
When they asked does it trot,
He said certainly not,
It’s a moppsikin floppsikin bear.\\ \vspace{0.1pt}

44:  Method: Human Poets\\
There were three little owls in a Wood,
Who sang hymns whenever they could,
What the words were about,
One could never make out,
But one felt it was doing them good.\\ \vspace{0.1pt}

45:  Method: Human Poets\\
There was a young wife from Vancouver,
Who could use her mouth just like a hoover,
But her husband she said,
Was no fun in bed,
Cos he just didn’t like that.\\ \vspace{0.1pt}

46:  Method: Human Poets\\
There once was a fellow from Bowen,
Whose penis kept growin and growin,
It grew so tremendous,
Heavy and pendulous,
Twas no good for rooting just showing.\\ \vspace{0.1pt}

47:  Method: Human Poets\\
There was an old man of Nantucket,
Who kept all his cash in a bucket,
His daughter called nan,
Ran away with a man,
And as for the bucket nantucket.\\ \vspace{0.1pt}

48:  Method: Human Poets\\
There was a young fellow named Fisher,
Who was fishing for fish in a fissure,
Then a cod with a grin,
Pulled the fisherman in,
Now they’re fishing the fissure for fisher.\\ \vspace{0.1pt}

49:  Method: Human Poets\\
There once was a girl from Kentucky,
Who considered herself very lucky,
She’d unzipped the flies,
Of hundreds of guys,
And never found one that was yucky.\\ \vspace{0.1pt}

50:  Method: Human Poets\\
There was a young lady of Chiswick,
Who consulted a doctor of physic,
He tested her hormones,
And sexual performones,
Then prescribed her a strong aphrodisic.\\ \vspace{0.1pt}

51:  Method: Human Poets\\
There was a young maid of Peru,
Who swore she never would screw,
Except under stress,
Of forceful duress,
Like i’m ready how about you.\\ \vspace{0.1pt}

52:  Method: Human Poets\\
There was a strange student from Yale,
Who puts himself outside the pale,
Said the judge please refrain,
When passing through maine,
From exposing yourself again in the train.\\ \vspace{0.1pt}

53:  Method: Human Poets\\
There was a young lady called Starky,
Who had an affair with a darky,
The result of her sins,
Was quads and not twins,
One white and one black and two khaki.\\ \vspace{0.1pt}

54:  Method: Human Poets\\
There was a young fellow called Taylor,
Who was found fellating a sailor,
When they put him in gaol,
He worked out his bail,
By sucking the cock of his gaoler.\\ \vspace{0.1pt}

55:  Method: Human Poets\\
There was a young plumber of Blois,
Who was plumbing a girl dans le bois,
Said the girl cease your plumbing,
I think someone’s coming,
Said the plumber still plumbing c’est moi.\\ \vspace{0.1pt}

56:  Method: Human Poets\\
There was a young fellow called Hall,
Who fell in the spring in the fall,
Twould have been a sad thing,
Had he died in the spring,
But he didn’t he died in the fall.\\ \vspace{0.1pt}

57:  Method: Human Poets\\
There was an old drunkard of Devon,
Who died and ascended to heaven,
But he cried this is hades,
58:  Method: Human Poets\\
There are no naughty Ladies,
And the pubs are all shut by eleven,
,
59:  Method: Human Poets\\
There was a young fellow of Lyme,
Who lived with three wives at one time,
When asked why the third,
He replied one’s absurd,
And bigamy sir is a crime.\\ \vspace{0.1pt}

60:  Method: Human Poets\\
There was an old fellow called Spiegal,
Who decided to bugger a beagle,
Just as he came,
He called the dog’s name,
And the dog said you know it’s illegal.\\ \vspace{0.1pt}

61:  Method: Human Poets\\
There was a young lady of Munich,
Whose appetite simply was unich,
Oh my she cooed,
I really like food,
And she let out a tuck in her tunich.\\ \vspace{0.1pt}

62:  Method: Human Poets\\
There was an old man from Eugowra,
Who went for a day trip to nowra,
He wanted to see,
The sea see cos he,
Had never been further than cowra.\\ \vspace{0.1pt}

63:  Method: Human Poets\\
There was an old fellow from Delhi,
Who had a big pain in his belly,
He farted a bit,
Then suddenly shit,
The result was disgustingly smelly.\\ \vspace{0.1pt}

64:  Method: Human Poets\\
There was a young lady of Ulva,
Who was famed far and wide for her vulva,
Most englishmen said,
It was herrings and bread,
But the turks said it tasted of halva.\\ \vspace{0.1pt}

65:  Method: Human Poets\\
There was an old man of Kamschatka,
Who possessed a remarkably fat cur,
His gait and his waddle,
Were held as a model,
To all the fat dogs in kamschatka.\\ \vspace{0.1pt}

66:  Method: Human Poets\\
There was an old man of cape Horn,
Who wished he had never been born,
And he wouldn’t have been,
If his father had seen,
That the end of the rubber was torn.\\ \vspace{0.1pt}

67:  Method: Human Poets\\
There was a young girl from the Gong,
Who considered that petting was wrong,
She told boyfriend bill,
I’m not on the pill,
We’d better keep walking along.\\ \vspace{0.1pt}

68:  Method: Human Poets\\
There was a young plumber of Leigh,
Who was plumbing his girl by the sea,
She said stop your plumbing,
69:  Method: Human Poets\\
There’s somebody Coming,
Said the plumber still plumbing it’s me,
,
70:  Method: Human Poets\\
There was an old man of the Wrekin,
Whose shoes made a horrible creaking,
But they said tell us whether,
Your shoes are of leather,
Or of what you old man of the wrekin.\\ \vspace{0.1pt}

71:  Method: Human Poets\\
There was an old man of Corfu,
Who never knew what he should do,
So he rushed up and down,
Till the sun made him brown,
That bewildered old man of corfu.\\ \vspace{0.1pt}

72:  Method: Human Poets\\
There was an old man with a Beard,
Who sat on a horse when he reared,
But they said never mind,
You will fall off behind,
You propitious old man with a beard.\\ \vspace{0.1pt}

73:  Method: Human Poets\\
There was an old fellow called Hugger,
Who was captain and mate of a fishing smack,
When a yacht crossed his bows,
He said my word,
It’s an awfully good thing it wasn’t a liner.\\ \vspace{0.1pt}

74:  Method: Human Poets\\
There was a young man of cape Horn,
Who wished he had never been born,
Nor would he have been,
If his father had seen,
That the end of the rubber was torn.\\ \vspace{0.1pt}

75:  Method: Human Poets\\
There was a young lady of Norway,
Who casually sat in a doorway,
When the door squeezed her flat,
She exclaimed what of that,
The courageous young lady of norway.\\ \vspace{0.1pt}

76:  Method: Human Poets\\
There was a young girl of Penzance,
Who decided to take just one chance,
She let herself go,
On the lap of her beau,
And now all her sisters are aunts.\\ \vspace{0.1pt}

77:  Method: Human Poets\\
There once was a wicked young Minister,
Whose conduct was thought to be sinister,
By ruses nightmarish,
He seduced the whole parish,
Except for one squeamish old spinister.\\ \vspace{0.1pt}

78:  Method: Human Poets\\
There once was a young man named Gus,
Who for animals had a great lust,
He buggered an owl,
Two dogs and a fowl,
And a little green lizard that bust.\\ \vspace{0.1pt}

79:  Method: Human Poets\\
There was a young student of John’s,
Who wanted to bugger some swans,
But the loyal hall porter,
Said please take my daughter,
For the swans are reserved for the dons.\\ \vspace{0.1pt}

80:  Method: Human Poets\\
There was an old man of Vienna,
Who lived upon tincture of senna,
When that did not agree,
He took camomile tea,
That nasty old man of vienna.\\ \vspace{0.1pt}

81:  Method: Human Poets\\
There was an old lady of Brooking,
Who had a great talent for cooking,
She baked sixty pies,
All the same size,
And knew which was which without looking.\\ \vspace{0.1pt}

82:  Method: Human Poets\\
There was an old man of Khartoum,
Who kept two black sheep in his room,
To remind me he said,
Of some people who’re dead,
But I never can recollect whom.\\ \vspace{0.1pt}

83:  Method: Human Poets\\
There was an old man from Harrow,
Who tried to have sex with a sparrow,
The sparrow said no,
You can’t have a go,
The hole in my arse is too narrow.\\ \vspace{0.1pt}

84:  Method: Human Poets\\
There once was a student at Johns,
Who wanted to bugger the swans,
But the loyal hall porter,
Said sir take my daughter,
Them birds are reserved for the dons.\\ \vspace{0.1pt}

85:  Method: Human Poets\\
There was an old lady from Kent,
Who farted wherever she went,
At the home builders fair,
When she dropped a few there,
They plugged up her arse with cement.\\ \vspace{0.1pt}

86:  Method: Human Poets\\
There was a young man of Belgrade,
Who planned to seduce a fair maid,
And as it befell,
He succeeded quite well,
And the maid like the plan was well laid.\\ \vspace{0.1pt}

87:  Method: Human Poets\\
There once was a woman of Waikerie,
Who in waikerie built a big bakery,
She didn’t bake bread,
Just sweet things instead,
Now her bakery’s waikerie’s cakery.\\ \vspace{0.1pt}

88:  Method: Human Poets\\
There once was a man from Bulleen,
Who invented a wanking machine,
It did a good job,
On a pussy or knob,
And wanked itself off in between.\\ \vspace{0.1pt}

89:  Method: Human Poets\\
There was an old person of Fratton,
Who would go to church with his hat on,
When I wake up he said,
With my hat on my head,
I shall know that it hasn’t been sat on.\\ \vspace{0.1pt}

90:  Method: Human Poets\\
There was a young fellow named Skinner,
Who took a young lady to dinner,
At half past nine,
They sat down to dine,
And by quarter to ten it was in her.\\ \vspace{0.1pt}

91:  Method: Human Poets\\
There once was a fellow from Reims,
Who always had heavy wet dreams,
He was a great wit,
He encased them in shit,
And he sold them as chocolate creams.\\ \vspace{0.1pt}

92:  Method: Human Poets\\
There once was a vicar of Ryhill,
Who went for a shit on a high hill,
When his curate asked was it,
A goodly deposit,
He said vox et praetera nihil.\\ \vspace{0.1pt}

93:  Method: Human Poets\\
There was an old maid of Wodonga,
Whose urges grew steadily stronger,
Till at eighty she had one,
And it wasn’t a bad one,
Tho she said that she wished it was longer.\\ \vspace{0.1pt}

94:  Method: Human Poets\\
There was a young bride named Mcwing,
Who thought sex a delirious fling,
When her bridegroom grew ill,
From too much as they will,
She found other men do the same thing.\\ \vspace{0.1pt}

95:  Method: Human Poets\\
There was a young girl of Majorca,
Whose aunt was a very fast walker,
She walked seventy miles,
And leaped fifteen stiles,
Which astounded that girl of majorca.\\ \vspace{0.1pt}

96:  Method: Human Poets\\
There was an old maid of Vancouver,
Who captured a man by manoeuvre,
She jumped on his knee,
With some rare eau de vie,
And nothing on earth could remove her.\\ \vspace{0.1pt}

97:  Method: Human Poets\\
There was a young lady from Spain,
Who did it now and again,
Not now and again,
But now and again,
And again and again and again.\\ \vspace{0.1pt}

98:  Method: Human Poets\\
There was an old person of Mold,
Who shrank from sensations of cold,
So he purchased some muffs,
Some furs and some fluffs,
And wrapped himself from the cold.\\ \vspace{0.1pt}

99:  Method: Human Poets\\
There once was a lady from Noosa,
Whose morals got looser and looser,
She let young blokes squeeze her,
And tease her and please her,
And often let older blokes goose her.\\ \vspace{0.1pt}

100:  Method: Human Poets\\
There was a young lady of Florence,
Who for kissing professed great abhorrence,
But when she’d been kissed,
And found what she’d missed,
She cried till her tears came in torrents.\\ \vspace{0.1pt}

101:  Method: Human Poets\\
There was a young drover named Gorse,
Who fell madly in love with his horse,
Said his wife you rapscallion,
That horse is a stallion,
This constitutes grounds for divorce.\\ \vspace{0.1pt}

102:  Method: Human Poets\\
There was a young man of st Paul,
Whose prick was exceedingly small,
He could bugger a bug,
At the edge of a rug,
And the bug hardly felt it at all.\\ \vspace{0.1pt}

103:  Method: Human Poets\\
There was an old man of Aosta,
Who possessed a large cow but he lost her,
But they said you see,
She has rushed up a tree,
You invidious old man of aosta.\\ \vspace{0.1pt}

104:  Method: Human Poets\\
There was a young fellow called Lancelot,
Who neighbours all looked on askance a lot,
Whenever he’d pass,
A nice piece of arse,
The front of his pants would advance a lot.\\ \vspace{0.1pt}

105:  Method: Human Poets\\
There is a young girl in Kilkenny,
Who is worried by lovers so many,
That the saucy young elf,
Means to raffle herself,
The tickets are two for a penny.\\ \vspace{0.1pt}

106:  Method: Human Poets\\
There once was a monarch called Harry,
Whose efforts seemed doomed to miscarry,
Since his wish for a son,
Plus unlimited fun,
Made him marry and marry and marry.\\ \vspace{0.1pt}

107:  Method: Human Poets\\
There was a young artist called Saint,
Who swallowed some samples of paint,
All shades of the spectrum,
Flowed out of his rectrum,
With a colourful lack of restraint.\\ \vspace{0.1pt}

108:  Method: Human Poets\\
There was a young lady named Wemyss,
Who it semyss was afficted with dremyss,
She’d wake in the night,
In a terrible fright,
And shake the roof bemyss with her scremyss.\\ \vspace{0.1pt}

109:  Method: Human Poets\\
There was a young girl of Mauritius,
Who said no i’m not really vicious,
I get no sexual kick,
Out of sucking this prick,
It’s just that it tastes so delicious.\\ \vspace{0.1pt}

110:  Method: Human Poets\\
There was an old man in a Tree,
Who was horribly bored by a bee,
When they said does it buzz,
He replied yes it does,
It’s a regular brute of a bee.\\ \vspace{0.1pt}

111:  Method: Human Poets\\
There once was a monarch named Ed,
Who took mrs simpson to bed,
As they bounced up and down,
He said bugger the crown,
Give the thing to my brother instead.\\ \vspace{0.1pt}

112:  Method: Human Poets\\
There was a young lady called Hilda,
Who went for a walk with a builder,
He knew that he could,
And he should and he would,
And he did and it bloody near killed her.\\ \vspace{0.1pt}

113:  Method: Human Poets\\
There was an old man of the North,
Who fell into a basin of broth,
But a laudable cook,
Fished him out with a hook,
Which saved that old man of the north.\\ \vspace{0.1pt}

114:  Method: Human Poets\\
There was a young man of Newcastle,
Who thought of himself as a parcel,
Which he’d tied with red tape,
And addressed for a jape,
To what hope kafka the castle.\\ \vspace{0.1pt}

115:  Method: Human Poets\\
There was once a commander named Harrison,
Who stationed his troops in a garrison,
And there they would languish,
And mutter with anguish,
Attila was kind by comparison.\\ \vspace{0.1pt}

116:  Method: Human Poets\\
There once was a horse called phar Lap,
Who kept winning despite handicap,
The mighty red terror,
No other horse ever,
Deserved such a cheer and a clap.\\ \vspace{0.1pt}

117:  Method: Human Poets\\
There was a young lady of Slough,
Who said that she didn’t know how,
Till a young fellow caught her,
And jolly well taught her,
And she lodges in pimlico now.\\ \vspace{0.1pt}

118:  Method: Human Poets\\
There was a young harlot from Kew,
Who filled her vagina with glue,
And said with a grin,
If they pay to get in,
They can pay to get out of it too.\\ \vspace{0.1pt}

119:  Method: Human Poets\\
There was a young fellow named Willy,
Who acted remarkably silly,
At an all nations ball,
Dressed in nothing at all,
He claimed that his costume was chile.\\ \vspace{0.1pt}

120:  Method: Human Poets\\
There was a young lady Of,
Who murdered herself in a dream,
Since when she repeats,
To all whom she meets,
I am much more defunct than I seem.\\ \vspace{0.1pt}

121:  Method: Human Poets\\
There was a young girl from Kilkenny,
Whose usual charge was a penny,
But for half of that sum,
You could fondle her bum,
A source of great pleasure to many.\\ \vspace{0.1pt}

122:  Method: Human Poets\\
There was a young poet of Kew,
Who failed to emerge into view,
So he said i’ll dispense,
With rhyme metre and sense,
And he did and he’s now in who’s who.\\ \vspace{0.1pt}

123:  Method: Human Poets\\
There was a young girl from a Mission,
Who was seized by an awful suspicion,
That original sin,
Didn’t matter a pin,
In an era of nuclear fission.\\ \vspace{0.1pt}

124:  Method: Human Poets\\
There was a young fellow of Wadham,
Who asked for a ticket to sodom,
When they said we prefer,
Not to issue them sir,
He said don’t call me sir call me modom.\\ \vspace{0.1pt}

125:  Method: Human Poets\\
There was a young lady of Wilts,
Who walked to the highlands on stilts,
When the locals said shocking,
To show so much stocking,
She answered what about kilts.\\ \vspace{0.1pt}

126:  Method: Human Poets\\
There was an old person of Slough,
Who took all his meals with a cow,
Always said it’s uncanny,
She’s so like auntie fanny,
But he never would indicate how.\\ \vspace{0.1pt}

127:  Method: Human Poets\\
There was a young lady of Riga,
Who smiled as she rode on a tiger,
They returned from the ride,
With the lady inside,
And the smile on the face of the tiger.\\ \vspace{0.1pt}

128:  Method: Human Poets\\
There once was a lady named Starky,
Who had an affair with a darkie,
The results of her sins,
Were quadruplets not twins,
One black and one white and two khaki.\\ \vspace{0.1pt}

129:  Method: Human Poets\\
There was a young man of Porthcawl,
Who thought he was samson or saul,
These thoughts so obscure,
Were due to the brewer,
And not to his ego at all.\\ \vspace{0.1pt}

130:  Method: Human Poets\\
There was an old lady of Harrow,
Whose views were exceedingly narrow,
At the end of her paths,
She built two bird baths,
For the different sexes of sparrow.\\ \vspace{0.1pt}

131:  Method: Human Poets\\
There once was a girl from Vancouver,
Whose mouth had the strength of a hoover,
When she turned it on high,
A week would pass by,
Before anyone could remove her.\\ \vspace{0.1pt}

132:  Method: Human Poets\\
There was a young lady of Bute,
Who played on a silver gilt flute,
She played several jigs,
To her white pigs,
That amusing young lady of bute.\\ \vspace{0.1pt}

133:  Method: Human Poets\\
There once was a gal named Lewinsky,
Who played on a flute like stravinsky,
Twas hail to the chief,
On a flute made of beef,
Then wipe all the stuff off your chinsky.\\ \vspace{0.1pt}

134:  Method: Human Poets\\
There was an old man of st Bees,
Who was stung in the arm by a wasp,
When asked does it hurt,
He replied no it doesn’t,
I’m so glad it wasn’t a hornet.\\ \vspace{0.1pt}

135:  Method: Human Poets\\
There was a young fellow named Dice,
Who remarked they say bigamy’s nice,
Even two are a bore,
I’d prefer three or four,
For the plural of spouse it is spice.\\ \vspace{0.1pt}

136:  Method: Human Poets\\
There was a young pervert called Jack,
Who was licking his wife’s anal crack,
He’d developed the art,
Of avoiding the fart,
But was hit in the face by the flak.\\ \vspace{0.1pt}

137:  Method: Human Poets\\
There was a young fellow called Clyde,
Who once at a funeral was spied,
When asked who was dead,
He smilingly said,
I don’t just came for the ride.\\ \vspace{0.1pt}

138:  Method: Human Poets\\
There was a young lady of Brabant,
Who slept with an impotent savant,
She admitted we shouldn’t,
But it turned out he couldn’t,
So you can’t say we have when we haven’t.\\ \vspace{0.1pt}

139:  Method: Human Poets\\
There was a young person of Smyrna,
Whose grandmother threatened to burn her,
But she seized on the cat,
And said granny burn that,
You incongruous old woman of smyrna.\\ \vspace{0.1pt}

140:  Method: Human Poets\\
There is a young man of york Plains,
Who will never come in when it rains,
He seems to forget,
That rain makes him wet,
But he never was noted for brains.\\ \vspace{0.1pt}

141:  Method: Human Poets\\
There was a young girl of old Natchez,
Whose garments were always in patchez,
When comment arose,
On the state of her clothes,
She drawled when ah itchez ah scratchez.\\ \vspace{0.1pt}

142:  Method: Human Poets\\
There once was a sculptor named Phidias,
Whose manners in art were invidious,
He carved aphrodite,
Without any nightie,
Which startled the ultra fastidious.\\ \vspace{0.1pt}

143:  Method: Human Poets\\
There once was a man from Nantucket,
Who kept all of his cash in a bucket,
But his daughter named nan,
Ran away with a man,
And as for the bucket nantucket.\\ \vspace{0.1pt}

144:  Method: Human Poets\\
There was a faith healer of Deal,
Who said although pain isn’t real,
If I sit on a pin,
And it punctures my skin,
I dislike what I fancy I feel.\\ \vspace{0.1pt}

145:  Method: Human Poets\\
There was a young man of cape Race,
Whose mind was an utter disgrace,
He thought marie corelli,
Lived long before shelley,
And that wells was the name of a place.\\ \vspace{0.1pt}

146:  Method: Human Poets\\
There once were two babes in the Wood,
Who happened to meet robin hood,
Who said with a leer,
Would you think it queer,
If I stuffed you with turkey and pud.\\ \vspace{0.1pt}

147:  Method: Human Poets\\
There was an old man of the Nile,
Who sharpened his nails with a file,
Till he cut off his thumbs,
And said calmly this comes,
Of sharpening nails with a file.\\ \vspace{0.1pt}

148:  Method: Human Poets\\
There once was a judge of Belsize,
Whose bollocks were not the same size,
He’d look at the right,
With a gasp of delight,
But the left one brought tears to his eyes.\\ \vspace{0.1pt}

149:  Method: Human Poets\\
There was a young lady from Boort,
Whose legs were excessively short,
When combing her hair,
She would stand on a chair,
And lean on the back for support.\\ \vspace{0.1pt}

150:  Method: Human Poets\\
There once was an old man of Lyme,
Who married three wives at a time,
When asked why a third,
He replied one’s absurd,
And bigamy sir is a crime.\\ \vspace{0.1pt}

151:  Method: Human Poets\\
There was an old maid from mount Isa,
Who let the young milkman surprise her,
Now she goes all shivery,
When he makes a delivery,
And the rest of the town’s none the wiser.\\ \vspace{0.1pt}

152:  Method: Human Poets\\
There was a young lady called Etta,
Who fancied herself in a sweater,
Three reasons she had,
Keeping warm was not bad,
But the other two reasons were better.\\ \vspace{0.1pt}

153:  Method: Human Poets\\
There was a young fellow named Baker,
Who seduced a vivacious young quaker,
And while he was on it,
She straightened her bonnet,
And knelt to give thanks to her maker.\\ \vspace{0.1pt}

154:  Method: Human Poets\\
There was a young lady from Twickenham,
Whose shoes were too tight to walk quickenham,
She came back from a walk,
With her face white as chalk,
And took her shoes off and was sickenham.\\ \vspace{0.1pt}

155:  Method: Human Poets\\
There was an old man of the Isles,
Whose face was pervaded with smiles,
He sung high dum diddle,
And played on the fiddle,
That amiable man of the isles.\\ \vspace{0.1pt}

156:  Method: Human Poets\\
There was a young man from Rabaul,
Who had a hexagonal ball,
The square of his date,
Plus his penis times eight,
Was two fifths of five eights of fuck all.\\ \vspace{0.1pt}

157:  Method: Human Poets\\
There was an old person of Wick,
Who said tick a tick tick a tick,
Chickabee chickabaw,
Then he said nothing more,
This laconic old person of wick.\\ \vspace{0.1pt}

158:  Method: Human Poets\\
There was a young girl of Tralee,
Whose knowledge of french was oui oui,
When they said parlez vous,
She replied same to you,
She was famed for her bright repartee.\\ \vspace{0.1pt}

159:  Method: Human Poets\\
There once was a duchess I Knew,
Who always bit oysters in two,
For she had a misgiving,
Should any be living,
They’d raise such a hullabaloo.\\ \vspace{0.1pt}

160:  Method: Human Poets\\
There was an old man of the Cape,
Who made himself garments of crepe,
When asked do they tear,
He replied here and there,
But they’re perfectly splendid for shape.\\ \vspace{0.1pt}

161:  Method: Human Poets\\
There once were some learned Mds,
Who captured some germs of disease,
And infected a train,
Which without causing pain,
Allowed hundreds to catch it with ease.\\ \vspace{0.1pt}

162:  Method: Human Poets\\
There was a young poet of Thusis,
Who went twilight walks with the muses,
But the nymphs of the air,
Are not what they were,
And the practice has led to abuses.\\ \vspace{0.1pt}

163:  Method: Human Poets\\
There once was a man from Blackheath,
Who sat on a pair of false teeth,
He rose with a start,
And said bless my heart,
I’ve bitten myself underneath.\\ \vspace{0.1pt}

164:  Method: Human Poets\\
There once was an eccentric of Metz,
Who filled all his villa with pets,
Who filled all the floors,
Both windows and doors,
Which just left an outhouse for vets.\\ \vspace{0.1pt}

165:  Method: Human Poets\\
There was an old man from Calcutta,
Who was found lying dead in a gutter,
The heat from the sun,
Burned a hole in his bum,
And melted his bollocks to butter.\\ \vspace{0.1pt}

166:  Method: Human Poets\\
There was an old person of Cromer,
Who stood on one leg to read homer,
When he found he grew stiff,
He jumped over the cliff,
Which concluded that person of cromer.\\ \vspace{0.1pt}

167:  Method: Human Poets\\
There was a young lady of Louth,
Who returned from a trip in the south,
Her father said nelly,
168:  Method: Human Poets\\
There’s more in your Belly,
Than ever went in at your mouth,
,
169:  Method: Human Poets\\
There was a young lady called Gloria,
Who was had by sir gerald du maurier,
And then by six men,
And sir gerald again,
And the band of the waldorf astoria.\\ \vspace{0.1pt}

170:  Method: Human Poets\\
There was a young lady from Ulva,
Whose music hall turn with a culver,
Evoked great applause,
As she tore off her drawers,
And induced it to swoop up her vulva.\\ \vspace{0.1pt}

171:  Method: Human Poets\\
There was an old dame of Toulouse,
Who had no reputation to lose,
When she revelled at night,
Her friends thought her too tight,
And her enemies thought her too loose.\\ \vspace{0.1pt}

172:  Method: Human Poets\\
There was a young girl of Majorca,
Whose aunt was a very fast walker,
She walked seventy miles,
And leaped fifteen stiles,
Which astonished that girl of majorca.\\ \vspace{0.1pt}

173:  Method: Human Poets\\
There was a young lady named Rose,
Who had a large wart on her nose,
When she had it removed,
Her appearance improved,
But her glasses slipped down to her toes.\\ \vspace{0.1pt}

174:  Method: Human Poets\\
There was a young lady from Dover,
Whose passion was such that it drove her,
To call as she came,
Oh dear what a shame,
Now we will have to start over.\\ \vspace{0.1pt}

175:  Method: Human Poets\\
There was an old man on a Hill,
Who seldom if ever stood still,
He ran up and down,
In his gown,
Which adorned that old man on a hill.\\ \vspace{0.1pt}

176:  Method: Human Poets\\
There was an old clerk at the war Office,
Whose brain was no good as a store office,
Whatever he’d hear,
Would go in one ear,
And straight out the opposite orifice.\\ \vspace{0.1pt}

177:  Method: Human Poets\\
There was a young lady at Court,
Who said to the king with a snort,
Was it humour or shyness,
That prompted your highness,
To put spanish fly in my port.\\ \vspace{0.1pt}

178:  Method: Human Poets\\
There once was a mermaid called Myrtle,
Who had an affair with a tyrtle,
And what was phenomenal,
A swelling abdominal,
Proved the tyrtle and myrtle were fyrtle.\\ \vspace{0.1pt}

179:  Method: Human Poets\\
There was a young man from Darjeeling,
Who got on a bus bound for ealing,
It said at the door,
Don’t spit on the floor,
So he carefully spat on the ceiling.\\ \vspace{0.1pt}

180:  Method: Human Poets\\
There once was a man from Oporta,
Who daily got shorter and shorter,
The reason he said,
Was the hod on his head,
Which was filled with the heaviest mortar.\\ \vspace{0.1pt}

181:  Method: Human Poets\\
There was a young lady of Norway,
Who hung by her toes in a doorway,
She said to her beau,
Come over here joe,
I think i’ve discovered one more way.\\ \vspace{0.1pt}

182:  Method: Human Poets\\
There was once a guy from new Delhi,
Who could fit fifteen girls on his belly,
When asked how they fit,
He said tit to tit,
And gee don’t my nuts turn to jelly.\\ \vspace{0.1pt}

183:  Method: Human Poets\\
There once was a harlot of Glamis,
Who would undress without any quamis,
If you paid her enough,
She’d strip to the buff,
And let you enjoy all her chamis.\\ \vspace{0.1pt}

184:  Method: Human Poets\\
There was an old person of Ischia,
Whose conduct grew friskier and friskier,
He danced hornpipes and jigs,
And ate thousands of figs,
That lively old person of ischia.\\ \vspace{0.1pt}

185:  Method: Human Poets\\
There was a young lady of Sweden,
Who went by the slow train to weedon,
When they cried weedon station,
She made no observation,
But thought she should go back to sweden.\\ \vspace{0.1pt}

186:  Method: Human Poets\\
There was an old man of Calcutta,
Who perpetually ate bread and butter,
Till a great bit of muffin,
On which he was stuffing,
Choked that horrid old man of calcutta.\\ \vspace{0.1pt}

187:  Method: Human Poets\\
There was a young fellow called Wyatt,
Who had a big girl on the quiet,
But down on the wharf,
He kept a nice dwarf,
Just in case he should go on a diet.\\ \vspace{0.1pt}

188:  Method: Human Poets\\
There was a respectable Mister,
Who noticed an odd sort of blister,
Where no blister should be,
Which was dreadful cos he,
Had got it at home from his sister.\\ \vspace{0.1pt}

189:  Method: Human Poets\\
There was a young lady of Parma,
Whose conduct grew calmer and calmer,
When they said are you dumb,
She merely said hum,
That provoking young lady of parma.\\ \vspace{0.1pt}

190:  Method: Human Poets\\
There was an old person of Rheims,
Who was troubled with horrible dreams,
So to keep him awake,
They fed him with cake,
Which amused that old person of rheims.\\ \vspace{0.1pt}

191:  Method: Human Poets\\
There once was a young royal Marine,
Who tried to fart god save the queen,
When he reached the soprano,
Out came the guano,
And his britches took ages to clean.\\ \vspace{0.1pt}

192:  Method: Human Poets\\
There was a young lady from Scone,
Who went to the dentist alone,
In a fit of depravity,
He filled the wrong cavity,
She’s nursing the filling at home.\\ \vspace{0.1pt}

193:  Method: Human Poets\\
There was a young lady of Dorking,
Who bought a large bonnet for walking,
But its colour and size,
So bedazzled her eyes,
That she very soon went back to dorking.\\ \vspace{0.1pt}

194:  Method: Human Poets\\
There was an old person of Prague,
Who was suddenly seized with the plague,
But they gave him some butter,
Which caused him to mutter,
And cured that old person of prague.\\ \vspace{0.1pt}

195:  Method: Human Poets\\
There was a young genius of Queen’s,
Who was fond of exploding machines,
He once blew up a door,
But he’ll do it no more,
For it chanced that the door was the dean’s.\\ \vspace{0.1pt}

196:  Method: Human Poets\\
There was an old man at a Easement,
Who held up his hands in amazement,
When they said sir fall,
He replied not at all,
That incipient old man at a casement.\\ \vspace{0.1pt}

197:  Method: Human Poets\\
There was a young man of Ostend,
Who went for a drink with a friend,
They had a few jars,
With two boys in some bars,
And so each had a friend in the end.\\ \vspace{0.1pt}

198:  Method: Human Poets\\
There was a young fellow of Ceuta,
Who rode into church on his scooter,
He knocked down the dean,
And said sorry old bean,
I ought to have sounded my hooter.\\ \vspace{0.1pt}

199:  Method: Human Poets\\
There was a young girl from Uttoxeter,
Who sported a tight fitting baroque sweater,
Her mother cried smart,
You look like a tart,
And flung accusations of pox at her.\\ \vspace{0.1pt}

200:  Method: Human Poets\\
There was an old person of Dover,
Who rushed through a field of blue clover,
But some very large bees,
Stung his nose and his knees,
So he very soon went back to dover.\\ \vspace{0.1pt}

201:  Method: Human Poets\\
There was an old man of Dundee,
Who came home as drunk as can be,
He wound up the clock,
With the end of his cock,
And buggered his wife with the key.\\ \vspace{0.1pt}

202:  Method: Human Poets\\
There was a young lady of Ealing,
Who walked up and down on the ceiling,
She shouted oh heck,
I’ve broken my neck,
And it is a peculiar feeling.\\ \vspace{0.1pt}

203:  Method: Human Poets\\
There was a young girl of cape Cod,
Who thought babies were fashioned by god,
But twas not the almighty,
Who lifted her nightie,
But roger the lodger the sod.\\ \vspace{0.1pt}

204:  Method: Human Poets\\
There was a young lady of Lynn,
Who thought all lovemaking a sin,
But when she got tight,
It seemed quite all right,
So everyone plied her with gin.\\ \vspace{0.1pt}

205:  Method: Human Poets\\
There once was a lady named Dot,
Who liked to put flies up her twat,
The buggers would buzz,
Way down in her fuzz,
Till you glued their wings tight with a shot.\\ \vspace{0.1pt}


==> no_story_poem.tex <==
1: \textit{Born:-2.993}, Method: No-Story\\
There was a brave woman named Flor,
Whose father was a soldier in war. 
But her mother died young, 
She was raised by her tongue, 
So she never learned on the floor. \\ \vspace{0.1pt}

2: \textit{Shaken:-2.672}, Method: No-Story\\
There was a bartender named Kay,
Who did a great job on my birthday. 
When I went to see her, 
I was shocked by her fur, 
And that is the reason of this day. \\ \vspace{0.1pt}

3: \textit{Restore:-2.780}, Method: No-Story\\
There was a cleaner named Renee,
Who did a great job on my birthday. 
When I went to see her, 
 I was shocked by her fur, 
But I knew she was doing it day. \\ \vspace{0.1pt}

4: \textit{Laugh:-2.892}, Method: No-Story\\
There once was a girl named Kay,
Who had a big crush on my birthday. 
When I got to meet her, 
She was on a transfer, 
She was happy to talk and to play. \\ \vspace{0.1pt}

5: \textit{Tears:-2.818}, Method: No-Story\\
There was a vain lady named Renee,
Who was a young woman on her way. 
When she came to see her, 
She was afraid to stir, 
She thought that her mother was okay. \\ \vspace{0.1pt}

6: \textit{Surprise:-2.900}, Method: No-Story\\
There was a lady named Kay,
Who was a young woman on her way. 
But her mother was dead, 
And she had to the bed, 
So she slept on her stomach and lay. \\ \vspace{0.1pt}

7: \textit{Kindness:-2.825}, Method: No-Story\\
There was a teacher named Renee,
Who did a great job on my birthday. 
When I got to see her, 
I was shocked by her fur, 
She has a perfect coat of a grey. \\ \vspace{0.1pt}

8: \textit{Humiliation:-2.738}, Method: No-Story\\
There once was a girl named Lenore,
Whose father was a soldier in war. 
But her mother was dead, 
Her brother killed instead, 
So she had to go down on the floor. \\ \vspace{0.1pt}

9: \textit{Victory:-2.657}, Method: No-Story\\
There was a brave captain named Kay,
Who did a great job on my birthday. 
When I got to know her, 
She was on a transfer, 
So I had to come down on the day. \\ \vspace{0.1pt}

10: \textit{Wedding:-2.655}, Method: No-Story\\
There once was a tailor named Kay,
Who did a great job on my birthday. 
When I went to see her, 
I was shocked by her fur, 
But I knew she was doing it day. \\ \vspace{0.1pt}

11: \textit{Alien:-2.881}, Method: No-Story\\
There was a warrior named Renee,
Who was a young woman on her way. 
It was like a nightmare, 
She was trapped by her hair, 
And that is the story of this day. \\ \vspace{0.1pt}

12: \textit{Holiday:-2.772}, Method: No-Story\\
There was a lively chef named Thuy,
Who was a great cook on our crew. 
When we went to see her, 
We were on a transfer, 
And she came down and took our cue. \\ \vspace{0.1pt}

13: \textit{Christmas:-2.815}, Method: No-Story\\
There once was a grandma named Kay,
Who had a big house on her birthday. 
When she went to see her, 
She was shocked by her fur, 
And that is the story of this day. \\ \vspace{0.1pt}

14: \textit{Thanksgiving:-2.794}, Method: No-Story\\
There was a lucky chef named Bok,
Who had a great restaurant on her block. 
When I went to see her, 
I was on a transfer, 
But she said she was taking me walk. \\ \vspace{0.1pt}

15: \textit{Birthday:-2.785}, Method: No-Story\\
There was a lady named Kay,
Who was a young woman on her way. 
When she came to see her, 
She was afraid to stir, 
So she slept on her stomach and lay. \\ \vspace{0.1pt}

16: \textit{Injury:-2.720}, Method: No-Story\\
There was a lawyer named Grace,
Who did a great job on our case. 
When we went to trial, 
I was shocked by her style, 
But I knew she was doing me grace. \\ \vspace{0.1pt}

17: \textit{Pillow:-2.953}, Method: No-Story\\
There once was a girl named Lore,
Whose father was a soldier in war. 
When she came to see her, 
She was shocked by her bur, 
Then she found it hidden in the floor. \\ \vspace{0.1pt}

18: \textit{Fiance:-2.903}, Method: No-Story\\
There was a shy grandma named Kay,
Who had a big smile on her birthday. 
When she got to see her, 
She was shocked by her fur, 
She was happy to meet and to play. \\ \vspace{0.1pt}

19: \textit{Dawn:-2.821}, Method: No-Story\\
There once was a girl named Lenore,
Whose father was a soldier in war. 
But her mother was dead, 
Her brother was a head, 
So she went up and slept on the floor. \\ \vspace{0.1pt}

20: \textit{Traffic:-2.850}, Method: No-Story\\
There was a nasty judge named Grace,
Who had a bad temper on her case. 
When she went to trial, 
She was able to smile, 
So she had to go down on the face. \\ \vspace{0.1pt}

21: \textit{Heartbreak:-3.084}, Method: No-Story\\
There was a fierce girl named Lenore,
Whose father was a soldier in war. 
But her mother was dead, 
Her brother was a head, 
Then she lost him right outside the door. \\ \vspace{0.1pt}

22: \textit{Wine:-3.019}, Method: No-Story\\
There was a lively chef named Thuy,
Who was a great cook on our crew. 
When we got to know her, 
She was married to sir, 
And died with a beautiful statue. \\ \vspace{0.1pt}

23: \textit{Beer:-2.770}, Method: No-Story\\
There once was a waitress named Lorelei,
Who had a huge crush on our guy. 
When we got to meet her, 
She was on a transfer, 
And we went down and saw her nearby. \\ \vspace{0.1pt}

24: \textit{Musuem:-2.724}, Method: No-Story\\
There was a blacksmith named Marguerite,
Who had a small shop on our street. 
When I got to know her, 
I was struck by her bur, 
And that is the reason of this treat. \\ \vspace{0.1pt}

25: \textit{Mountain:-2.878}, Method: No-Story\\
There was a harsh woman named Lore,
Whose father was a soldier in war. 
She was like a shadow, 
She was afraid to go, 
She was frightened to walk and to soar. \\ \vspace{0.1pt}

26: \textit{River:-2.742}, Method: No-Story\\
There once was a girl named Flor,
Whose father was a soldier in war. 
But her mother was dead, 
Her uncle was a head, 
So she grew up and slept on the floor. \\ \vspace{0.1pt}

27: \textit{Memory:-2.667}, Method: No-Story\\
There was a grandma named Bok,
Who had a big house on our block. 
It was like a playground, 
And it was to the ground, 
It was easy to climb and to walk. \\ \vspace{0.1pt}

28: \textit{Mud:-2.794}, Method: No-Story\\
There was a cleaner named Kay,
Who did a great job on my birthday. 
When I got to see her, 
I was shocked by her fur, 
But I knew she was doing it day. \\ \vspace{0.1pt}

29: \textit{Spider:-2.864}, Method: No-Story\\
There was a neat lady named Thuy,
Who was a great cook on our crew. 
She was like a mentor, 
And she was to the core, 
And that is the spirit of this stew. \\ \vspace{0.1pt}

30: \textit{Rain:-2.841}, Method: No-Story\\
There was a harsh woman named Renee,
Who was a young girl on her birthday. 
But her mother was dead, 
She had been by her bed, 
She was afraid to move and to play. \\ \vspace{0.1pt}

31: \textit{Season:-2.888}, Method: No-Story\\
There was a bright captain named Larue,
Who was a great leader on our crew. 
She was like a mentor, 
And she was to the core, 
She wanted us down in the blue. \\ \vspace{0.1pt}

32: \textit{Winter:-3.061}, Method: No-Story\\
There was a boring girl named Kai,
Who had a big crush on our guy. 
When we went to meet her, 
We were told by her bur, 
To leave our little boy nearby. \\ \vspace{0.1pt}

33: \textit{Throne:-2.885}, Method: No-Story\\
There was a wise lady named Lenore,
Whose husband was a soldier in war. 
When he returned to base, 
He was met by his face, 
Then he saw him walk towards the door. \\ \vspace{0.1pt}

34: \textit{Politics:-2.849}, Method: No-Story\\
There was a professor named Kay,
Who was a young woman on her way. 
When she came to see her, 
She was told by her sir, 
That the man she saw was a friday. \\ \vspace{0.1pt}

35: \textit{Promise:-2.735}, Method: No-Story\\
There was a vain lady named Kay,
Who was a great beauty on her day. 
When I got to know her, 
She was married to sir, 
And that is the reason of this play. \\ \vspace{0.1pt}

36: \textit{Beach:-2.936}, Method: No-Story\\
There was a sexy girl named Grace,
Who had a great body on her face. 
She was back from the gym, 
She was ready to swim, 
Then she saw me walk towards the staircase. \\ \vspace{0.1pt}

37: \textit{Bank:-2.860}, Method: No-Story\\
There was a lawyer named Grace,
Who did a great job on our case. 
When we went to trial, 
We were shocked by her style, 
She was not the person we replace. \\ \vspace{0.1pt}

38: \textit{Money:-2.832}, Method: No-Story\\
There was a lady named Renee,
Who was a young woman on her way. 
When she came to meet her, 
She was on a transfer, 
So she had to sit down on the tray. \\ \vspace{0.1pt}

39: \textit{Limerick:-2.795}, Method: No-Story\\
There was a butcher named Renee,
Who did a great job on my birthday. 
When I got to see her, 
I was shocked by her fur, 
But she has always come in my way. \\ \vspace{0.1pt}

40: \textit{Love:-2.939}, Method: No-Story\\
There was a woman named Lore,
Whose father was a soldier in war. 
But her mother was dead, 
She was raised by her head, 
She was trained to kill and to ignore. \\ \vspace{0.1pt}

41: \textit{Cunning:-2.767}, Method: No-Story\\
There was a sly witch named Clare,
Who lived all her life in a nightmare. 
When she came to see her, 
She was afraid to stir, 
She was frightened to speak and to stare. \\ \vspace{0.1pt}

42: \textit{Dog:-2.943}, Method: No-Story\\
There was a funny girl named Lorelei,
Who had a big crush on our guy. 
When we went to see her, 
She was shocked by his fur, 
So she beat on his head and nearby. \\ \vspace{0.1pt}

43: \textit{Blood:-2.932}, Method: No-Story\\
There was a cruel nurse named Freda,
Who had a sick baby on her bed. 
But her husband was dead, 
She was afraid to read, 
So she slept on her stomach and fled. \\ \vspace{0.1pt}

44: \textit{Death:-3.355}, Method: No-Story\\
There was a woman named Lore,
Whose father was a soldier in war. 
But her mother died young, 
Left the family tongue, 
And now she is a student mentor. \\ \vspace{0.1pt}

45: \textit{War:-3.047}, Method: No-Story\\
There was a lieutenant named Larue,
Who was a young woman on my crew. 
She was like a mentor, 
And she was to the core, 
She wanted us down in the blue. \\ \vspace{0.1pt}

46: \textit{Disease:-2.939}, Method: No-Story\\
There was a surgeon named Renee,
Who did a great job on my birthday. 
When I got to know her, 
Which I did in the blur, 
I was thrilled to have a new resume. \\ \vspace{0.1pt}

47: \textit{World:-2.858}, Method: No-Story\\
There was a brave girl named Flor,
Whose father was a soldier in war. 
But her mother was dead, 
She was raised by her head, 
She was trained to kill and to ignore. \\ \vspace{0.1pt}

48: \textit{Planet:-2.795}, Method: No-Story\\
There was a wise woman named Kay,
Who was a young girl on her birthday. 
When she came to see her, 
She was shocked by her fur, 
So she tried to get down on the hay. \\ \vspace{0.1pt}

49: \textit{Fire:-3.039}, Method: No-Story\\
There was a woman named Laure,
Whose husband was a soldier in war. 
But her mother was dead, 
Her father was a head, 
And her brothers were older and four. \\ \vspace{0.1pt}

50: \textit{Water:-2.911}, Method: No-Story\\
There was a harsh woman named Grace,
Who had a bad temper on her face. 
It was like a nightmare, 
She was scared by her hair, 
So she went up and slept on the place. \\ \vspace{0.1pt}

51: \textit{Sports:-2.845}, Method: No-Story\\
There was a writer named Renee,
Who did a great job on my birthday. 
When I got to see her, 
I was shocked by her fur, 
But I knew she was doing it day. \\ \vspace{0.1pt}

52: \textit{Love:-2.805}, Method: No-Story\\
There once was a lady named Lenore,
Whose husband was a soldier in war. 
When she came to see her, 
She was told by her bur, 
That the man she saw was a mentor. \\ \vspace{0.1pt}

53: \textit{Car:-2.761}, Method: No-Story\\
There was a cleaner named Kay,
Who did a great job on my birthday. 
When I went to see her, 
I was shocked by her fur, 
And that is the reason of this day. \\ \vspace{0.1pt}

54: \textit{Animal:-2.785}, Method: No-Story\\
There was a silly girl named Lorelei,
Who had a big crush on our guy. 
When we went to see her, 
She was shocked by his fur, 
But she said he was wearing it high. \\ \vspace{0.1pt}

55: \textit{Violent:-2.771}, Method: No-Story\\
There was a woman named Kay,
Who was a young girl on her birthday. 
When she came to see her, 
She was scared by her fur, 
So she had to go down on the hay. \\ \vspace{0.1pt}

56: \textit{Opera:-2.847}, Method: No-Story\\
There was a dancer named Bess,
Who did all her dancing in a dress. 
When she returned to work, 
She was told by a clerk, 
This did not apply to her process. \\ \vspace{0.1pt}

57: \textit{Monster:-2.668}, Method: No-Story\\
There once was a girl named Cher,
Who lived all her life in a nightmare. 
When she came to see her, 
She was afraid to stir, 
She was frightened to speak and to stare. \\ \vspace{0.1pt}

58: \textit{Library:-2.748}, Method: No-Story\\
There was a smart teacher named Celeste,
Who was a good student on her test. 
When she started to talk, 
She was able to walk, 
So she got up and put on the vest. \\ \vspace{0.1pt}

59: \textit{Market:-2.795}, Method: No-Story\\
There was a farmer named Bridgette,
Who owned a small farm on our street. 
She was like a mentor, 
And she was to the core, 
She was loving to work and to eat. \\ \vspace{0.1pt}

60: \textit{Noble:-2.805}, Method: No-Story\\
There was a warrior named Kay,
Who was a young woman on her way. 
She was like a fairy, 
She was on a ferry, 
She was able to swim and to play. \\ \vspace{0.1pt}

61: \textit{Doctor:-2.873}, Method: No-Story\\
There was a surgeon named Freda,
Who did a great job on our head. 
She was like a mentor, 
And she was to the core, 
But she knew she was doing it dead. \\ \vspace{0.1pt}

62: \textit{Ball:-2.841}, Method: No-Story\\
There once was a captain named Thuy,
Who was a great leader on our crew. 
She was like a mentor, 
And she was to the core, 
But she knew we were doing it new. \\ \vspace{0.1pt}

63: \textit{Funeral:-3.056}, Method: No-Story\\
There was a grandma named Bok,
Who had a big house on our block. 
It was like a playground, 
It was one large compound, 
It has a nice view out in the walk. \\ \vspace{0.1pt}

64: \textit{Body:-2.842}, Method: No-Story\\
There once was a girl named Kai,
Who had a big crush on our guy. 
When we went to see her, 
She was shocked by her fur, 
So she got up and put on the tie. \\ \vspace{0.1pt}

65: \textit{Smart:-2.745}, Method: No-Story\\
There was a designer named Tess,
Who did a great job on our dress. 
When we went to meet her, 
She was on a transfer, 
So we had to go down on the press. \\ \vspace{0.1pt}

66: \textit{Exercise:-2.834}, Method: No-Story\\
There was a teacher named Pam,
Who did a great job on our program. 
She was like a mentor, 
And she was to the core, 
She was willing to learn and to jam. \\ \vspace{0.1pt}

67: \textit{Gun:-2.692}, Method: No-Story\\
There was a stupid girl named Lorelei,
Who had a huge crush on our guy. 
When we went to meet her, 
We were on a transfer, 
So we had to go down on the fly. \\ \vspace{0.1pt}

68: \textit{Art:-2.794}, Method: No-Story\\
There was a designer named Tess,
Who did a great job on our dress. 
When we went to see her, 
We were shocked by her fur, 
Which was done with the finest process. \\ \vspace{0.1pt}

69: \textit{Music:-2.790}, Method: No-Story\\
There was a dancer named Tess,
Who did all her dancing in a dress. 
It was for her birthday, 
Which she did in the day, 
So she got up and put on the mess. \\ \vspace{0.1pt}

70: \textit{Boxing:-2.944}, Method: No-Story\\
There was a dancer named Tess,
Who did all her dancing in a dress. 
When she returned to work, 
She was told by her clerk, 
She was ordered to strip and to press. \\ \vspace{0.1pt}

71: \textit{Forest:-2.637}, Method: No-Story\\
There was a wise farmer named Brande,
Who had a great garden on her land. 
But her husband was dead, 
And she had to the bed, 
So she had to sleep down on the sand. \\ \vspace{0.1pt}

72: \textit{Philosophy:-2.834}, Method: No-Story\\
There was a teacher named Pam,
Who did a great job on our program. 
She was like a mentor, 
And she was to the core, 
She was willing to learn and to jam. \\ \vspace{0.1pt}

73: \textit{Night:-2.708}, Method: No-Story\\
There was a bright lady named Laure,
Whose husband was a soldier in war. 
When he returned to base, 
He was met by his face, 
So he had to go down on the floor. \\ \vspace{0.1pt}

74: \textit{Scary:-2.948}, Method: No-Story\\
There once was a girl named Flor,
Whose father was a soldier in war. 
When she came to see her, 
She was struck by her fur, 
And she took down and buried her store. \\ \vspace{0.1pt}

75: \textit{Creativity:-2.794}, Method: No-Story\\
There was a designer named Tess,
Who did a great job on our dress. 
When we went to see her, 
We were shocked by her fur, 
Which was done with the finest process. \\ \vspace{0.1pt}

76: \textit{Evil:-2.851}, Method: No-Story\\
There was a warrior named Renee,
Who was a young woman on her way. 
But her mother was dead, 
She had been by her bed, 
So she slept on her stomach and lay. \\ \vspace{0.1pt}

77: \textit{Angry:-2.720}, Method: No-Story\\
There once was a lady named Flor,
Whose husband was a soldier in war. 
When she came to see her, 
She was struck by his fur, 
So she had to go down on the floor. \\ \vspace{0.1pt}

78: \textit{Pride:-2.710}, Method: No-Story\\
There was a warrior named Renee,
Who was a young woman on her way. 
When she came to meet her, 
She was told by her sir, 
She was welcome to come and to stay. \\ \vspace{0.1pt}

79: \textit{Law:-2.918}, Method: No-Story\\
There was a professor named Pam,
Who did a great job on our program. 
She was like a mentor, 
And she was to the core, 
So she really helped on the programme. \\ \vspace{0.1pt}

80: \textit{School:-3.015}, Method: No-Story\\
There was a shy teacher named Renee,
Who had a big crush on my birthday. 
It was like a nightmare, 
I was trapped by my hair, 
So I slept on my stomach and lay. \\ \vspace{0.1pt}

81: \textit{Light:-2.787}, Method: No-Story\\
There was a quiet girl named Lore,
Whose father was a soldier in war. 
But her mother was dead, 
Her uncle was a head, 
So she had to go down on the floor. \\ \vspace{0.1pt}

82: \textit{Rich:-2.798}, Method: No-Story\\
There was a smart farmer named Brande,
Who had a big garden on her land. 
But her husband was sick, 
So she took down the brick, 
And now she has a giant wasteland. \\ \vspace{0.1pt}

83: \textit{Color:-2.734}, Method: No-Story\\
There was a neat cleaner named Kay,
Who did a great job on my birthday. 
When I went to see her, 
I was shocked by her fur, 
But she has always come in my way. \\ \vspace{0.1pt}

84: \textit{Leader:-2.680}, Method: No-Story\\
There was a lieutenant named Larue,
Who did a great job on our crew. 
She was like a mentor, 
And she was to the core, 
She was willing to learn and to do. \\ \vspace{0.1pt}

85: \textit{Airplane:-2.791}, Method: No-Story\\
There was a neat captain named Thuy,
Who was a great leader on my crew. 
When I got to know her, 
She was able to stir, 
She was willing to learn and to do. \\ \vspace{0.1pt}

86: \textit{Park:-3.024}, Method: No-Story\\
There was a funny girl named Lorelei,
Who had a big crush on our guy. 
But the moment we met, 
We instantly fell wet, 
And that is the beauty of this tie. \\ \vspace{0.1pt}

87: \textit{Loss:-2.816}, Method: No-Story\\
There was a surgeon named Kay,
Who did a great job on my birthday. 
When I got to see her, 
She was shocked by my fur, 
So I had to go down on the tray. \\ \vspace{0.1pt}

88: \textit{Weight:-3.098}, Method: No-Story\\
There was a wise doctor named Renee,
Who was a great healer on her day. 
She was like a mentor, 
And she was to the core, 
So she was up and go on the way. \\ \vspace{0.1pt}

89: \textit{Useful:-2.867}, Method: No-Story\\
There was a author named Amal,
Who wrote a short story on my wall. 
When I got to know her, 
She was married to sir, 
So I had to get down on the ball. \\ \vspace{0.1pt}

90: \textit{Applaud:-2.600}, Method: No-Story\\
There was a wise judge named Kay,
Who was a young girl on her birthday. 
When she came to see her, 
She was afraid to stir, 
So she had to lie down on the hay. \\ \vspace{0.1pt}

91: \textit{Home:-2.787}, Method: No-Story\\
There was a smart grandma named Bok,
Who had a big house on our block. 
When I got to know her, 
I was struck by her were, 
And that is the beauty of this walk. \\ \vspace{0.1pt}

92: \textit{Union:-2.952}, Method: No-Story\\
There was a fierce teacher named Kay,
Who was a young woman on her way. 
When she came to see her, 
She was scared by her fur, 
But she is still brave in our day. \\ \vspace{0.1pt}

93: \textit{Child:-2.890}, Method: No-Story\\
There was a cruel girl named Maire,
Who lived all her life in a nightmare. 
She came back from the grave, 
And she said to the slave, 
And that is the reason of this prayer. \\ \vspace{0.1pt}

94: \textit{Working:-3.127}, Method: No-Story\\
There was a teacher named Bok,
Who was a black woman on my block. 
She was like a mentor, 
And she was to the core, 
And she was still like mother of rock. \\ \vspace{0.1pt}

95: \textit{Cheat:-3.034}, Method: No-Story\\
There was a liar named Flor,
Whose husband was a soldier in war. 
When she tried to stop her, 
She was ordered to stir, 
But she refused her orders and tore. \\ \vspace{0.1pt}

96: \textit{Fall:-2.967}, Method: No-Story\\
There was a wise woman named Renee,
Who was a young girl on her birthday. 
When she came to see her, 
She was shocked by her fur, 
It had grown to be a full sunday. \\ \vspace{0.1pt}

97: \textit{Time:-2.799}, Method: No-Story\\
There was a doctor named Kay,
Who did a great job on my birthday. 
When I got to see her, 
I was shocked by her fur, 
And that is the reason of this day. \\ \vspace{0.1pt}

98: \textit{Hope:-2.806}, Method: No-Story\\
There was a lady named Kay,
Who was a young lady on her way. 
But her mother was dead, 
She had been by her bed, 
So she had to go down on the hay. \\ \vspace{0.1pt}

99: \textit{Flower:-2.705}, Method: No-Story\\
There was a lady named Renee,
Who was a young woman on her way. 
When she came to see her, 
She was afraid to stir, 
She was frightened to speak and to pray. \\ \vspace{0.1pt}

100: \textit{Random:-2.698}, Method: No-Story\\
There was a boring girl named Kai,
Who had a huge crush on our guy. 
When we went to meet her, 
We were on a transfer, 
So we had to go down on the fly. \\ \vspace{0.1pt}

101: \textit{Impressive:-2.829}, Method: No-Story\\
There was a neat artist named Renee,
Who did a great job on my birthday. 
When I got to see her, 
I was shocked by her fur, 
But I think that she really okay. \\ \vspace{0.1pt}

102: \textit{Born:-3.077}, Method: No-Story\\
There was a brave boy named Saul,
Who lived all his life within a wall. 
He was like a shadow, 
But he also was though, 
So he had to go down on the ball. \\ \vspace{0.1pt}

103: \textit{Born:-2.807}, Method: No-Story\\
There was a brave boy named Theodore,
Whose father was a soldier in war. 
When he returned to school, 
He was struck by a tool, 
And that is the basis of this score. \\ \vspace{0.1pt}

104: \textit{Shaken:-2.738}, Method: No-Story\\
There was a fierce man named Nathanael,
Who was a great hunter on his trail. 
When he came to meet her, 
He was struck by her fur, 
And knew her because she was female. \\ \vspace{0.1pt}

105: \textit{Restore:-3.061}, Method: No-Story\\
There was a vain man named Scot,
Who had all his money in a pot. 
When he came to trial, 
He had the same profile, 
But nobody wanted what he got. \\ \vspace{0.1pt}

106: \textit{Laugh:-2.628}, Method: No-Story\\
There was a funny boy named Dario,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
And he got down and took my photo. \\ \vspace{0.1pt}

107: \textit{Tears:-2.851}, Method: No-Story\\
There was a vain man named Lyle,
Who had all his money in a pile. 
When he came to see her, 
He was afraid to stir, 
Because she was holding his trial. \\ \vspace{0.1pt}

108: \textit{Surprise:-3.062}, Method: No-Story\\
There was a lucky man named Lyle,
Who had all his money in a pile. 
He was back from the war, 
And he had to the store, 
And get food to his wife in exile. \\ \vspace{0.1pt}

109: \textit{Kindness:-2.862}, Method: No-Story\\
There was a polite man named Hugh,
Who was a good friend on our crew. 
He was like a mentor, 
And he was to the core, 
He knew that our mission was true. \\ \vspace{0.1pt}

110: \textit{Humiliation:-2.843}, Method: No-Story\\
There was a bully named Pete,
Who was a bad boy on our street. 
He was a musician, 
He was on a mission, 
So he was up and come on the beat. \\ \vspace{0.1pt}

111: \textit{Victory:-2.815}, Method: No-Story\\
There was a fierce captain named Kip,
Who was a great fighter on his ship. 
But his father was dead, 
He was left by his bed, 
So he had to go down on the trip. \\ \vspace{0.1pt}

112: \textit{Wedding:-2.682}, Method: No-Story\\
There was a tailor named Les,
Who did a great job on our dress. 
When we went to see her, 
We were shocked by her fur, 
Which was done with the finest process. \\ \vspace{0.1pt}

113: \textit{Alien:-2.997}, Method: No-Story\\
There was a silly man named Cole,
Who had all his money in a hole. 
He was back from the war, 
And he was to the door, 
He was ready to go and to roll. \\ \vspace{0.1pt}

114: \textit{Holiday:-2.907}, Method: No-Story\\
There was a bright chef named Hugh,
Who was a great cook on our crew. 
He was like a mentor, 
And he was to the fore, 
So we had to be down on the blue. \\ \vspace{0.1pt}

115: \textit{Christmas:-2.829}, Method: No-Story\\
There once was a boy named Pierre,
Who lived all his life in a nightmare. 
When he came to see her, 
He was struck by her fur, 
But she said he was wearing it bare. \\ \vspace{0.1pt}

116: \textit{Thanksgiving:-2.888}, Method: No-Story\\
There was a humble chef named Hugh,
Who was a great cook on our crew. 
He was like a mentor, 
And he was to the core, 
He was hard to get a good review. \\ \vspace{0.1pt}

117: \textit{Birthday:-2.628}, Method: No-Story\\
There was a funny boy named Beau,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
And he got down and took my photo. \\ \vspace{0.1pt}

118: \textit{Injury:-2.720}, Method: No-Story\\
There was a surgeon named Ted,
Who did a great job on our head. 
He was like a mentor, 
And he was to the core, 
He was really the reason we led. \\ \vspace{0.1pt}

119: \textit{Pillow:-2.977}, Method: No-Story\\
There was a bright grandpa named Brock,
Who was a good friend on our block. 
He was like a mentor, 
And he was to the core, 
But he knew he was doing it talk. \\ \vspace{0.1pt}

120: \textit{Fiance:-3.046}, Method: No-Story\\
There was a shy grandpa named Brock,
Who was a good friend on our block. 
He was like a mentor, 
And he was to the door, 
And say hi to my mother in shock. \\ \vspace{0.1pt}

121: \textit{Dawn:-2.563}, Method: No-Story\\
There was a brave boy named Salvador,
Whose father was a soldier in war. 
When he returned to school, 
He was struck by a pool, 
So he had to get down on the floor. \\ \vspace{0.1pt}

122: \textit{Traffic:-2.723}, Method: No-Story\\
There once was a man named Javier,
Who lived all his life in a nightmare. 
He was like a shadow, 
He was afraid to go, 
He was frightened to walk and to stare. \\ \vspace{0.1pt}

123: \textit{Heartbreak:-2.782}, Method: No-Story\\
There once was a boy named Theodore,
Whose father was a soldier in war. 
When he got to combat, 
He was killed by a cat, 
So he went up and slept on the floor. \\ \vspace{0.1pt}

124: \textit{Wine:-2.816}, Method: No-Story\\
There was a neat chef named Pete,
Who did a great job on our meat. 
He was like a mentor, 
And he was to the core, 
He is a good guy out in the street. \\ \vspace{0.1pt}

125: \textit{Musuem:-2.774}, Method: No-Story\\
There once was a blacksmith named Pete,
Who owned a small shop on our street. 
He was a musician, 
And with his permission, 
I went through the store and bought concrete. \\ \vspace{0.1pt}

126: \textit{Beer:-2.561}, Method: No-Story\\
There was a bubbly man named Sergio,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
But he said he was taking it slow. \\ \vspace{0.1pt}

127: \textit{Mountain:-2.813}, Method: No-Story\\
There was a brave boy named Claudio,
Who did a great job on our show. 
He was like a mentor, 
And he was to the core, 
He was really the reason we grow. \\ \vspace{0.1pt}

128: \textit{Memory:-2.810}, Method: No-Story\\
There was a general named Graham,
Who did a great job on our program. 
He was like a mentor, 
And he was to the core, 
He was willing to learn and to jam. \\ \vspace{0.1pt}

129: \textit{Mud:-2.961}, Method: No-Story\\
There was a harsh boy named Salvador,
Whose father was a soldier in war. 
When he returned to school, 
He was shocked by his cool, 
But somehow accepted what he wore. \\ \vspace{0.1pt}

130: \textit{Spider:-2.816}, Method: No-Story\\
There was a warrior named Hugh,
Who was a good friend on our crew. 
He was like a mentor, 
And he was to the core, 
But he knew we were doing it true. \\ \vspace{0.1pt}

131: \textit{River:-3.128}, Method: No-Story\\
There was a brave farmer named Brock,
Who had a small farm on our block. 
He was like a mentor, 
And he was to the core, 
He is a good guy out in the walk. \\ \vspace{0.1pt}

132: \textit{Season:-2.868}, Method: No-Story\\
There was a bright captain named Kip,
Who was a great leader on our ship. 
He was like a mentor, 
And he was to the core, 
So I really enjoyed on the trip. \\ \vspace{0.1pt}

133: \textit{Rain:-2.553}, Method: No-Story\\
There was a bright boy named Salvador,
Whose father was a soldier in war. 
But his mother was dead, 
He was left by his bed, 
So he had to sleep down on the floor. \\ \vspace{0.1pt}

134: \textit{Winter:-2.788}, Method: No-Story\\
There was a lucky boy named Scot,
Who had all his money in a pot. 
He was back from the war, 
And he had to the store, 
So he had to go down on the spot. \\ \vspace{0.1pt}

135: \textit{Throne:-2.783}, Method: No-Story\\
There was a warrior named Kip,
Who was a great leader on his ship. 
He was like a mentor, 
It was hard to ignore, 
And that is the spirit of this trip. \\ \vspace{0.1pt}

136: \textit{Politics:-2.937}, Method: No-Story\\
There was a general named Abraham,
Who did a great job on our program. 
He was like a mentor, 
And he was to the core, 
He was really the reason we am. \\ \vspace{0.1pt}

137: \textit{Beach:-2.889}, Method: No-Story\\
There was a bright boy named Brock,
Who was a great athlete on his block. 
When he got to football, 
He was able to fall, 
So he had to go down on the walk. \\ \vspace{0.1pt}

138: \textit{Promise:-3.015}, Method: No-Story\\
There was a lucky man named Lyle,
Who had all his money in a pile. 
He was back from the war, 
And he had to the store, 
So he never went on the trial. \\ \vspace{0.1pt}

139: \textit{Bank:-2.992}, Method: No-Story\\
There was a greedy man named Lyle,
Who had all his money in a pile. 
He was back from the war, 
And he had to the store, 
So he never went on the trial. \\ \vspace{0.1pt}

140: \textit{Money:-2.959}, Method: No-Story\\
There was a lucky man named Lyle,
Who had all his money in a pile. 
He was back from the war, 
And he had to the store, 
Then he saw me stand in the aisle. \\ \vspace{0.1pt}

141: \textit{Limerick:-2.478}, Method: No-Story\\
There once was a grandpa named Pete,
Who owned a small farm on our street. 
He was a musician, 
He was on a mission, 
He was proud to be a black athlete. \\ \vspace{0.1pt}

142: \textit{Love:-3.119}, Method: No-Story\\
There was a lucky boy named Lyle,
Who had all his money in a pile. 
But his father was dead, 
He had been by his bed, 
And he was not like man of trial. \\ \vspace{0.1pt}

143: \textit{Cunning:-2.978}, Method: No-Story\\
There was a warrior named Kip,
Who was a great leader on his ship. 
He was like a mentor, 
It was hard to ignore, 
So I got up and put on the whip. \\ \vspace{0.1pt}

144: \textit{Dog:-3.091}, Method: No-Story\\
There was a nasty boy named Brock,
Who was a bad kid on our block. 
He was like a nightmare, 
He really was unfair, 
And that is the story of this talk. \\ \vspace{0.1pt}

145: \textit{Blood:-2.832}, Method: No-Story\\
There was a doctor named Chase,
Who did a great job on our case. 
When we went to trial, 
I was shocked by his style, 
But I knew he was doing us grace. \\ \vspace{0.1pt}

146: \textit{Death:-2.906}, Method: No-Story\\
There was a brave boy named Theodore,
Whose father was a soldier in war. 
When he returned to school, 
He was shocked by his cool, 
He was not the student he before. \\ \vspace{0.1pt}

147: \textit{War:-2.732}, Method: No-Story\\
There was a cruel man named Pierre,
Who lived all his life in a nightmare. 
He was like a shadow, 
He was afraid to go, 
He was frightened to walk and to stare. \\ \vspace{0.1pt}

148: \textit{Disease:-2.858}, Method: No-Story\\
There was a doctor named Chase,
Who did a great job on our case. 
When we went to trial, 
I was shocked by his style, 
And that is the reason of this place. \\ \vspace{0.1pt}

149: \textit{World:-2.826}, Method: No-Story\\
There was a lucky man named Lyle,
Who had all his money in a pile. 
He was back from the war, 
And he had to the store, 
So he got up and put on the smile. \\ \vspace{0.1pt}

150: \textit{Planet:-3.015}, Method: No-Story\\
There was a lucky man named Lyle,
Who had all his money in a pile. 
He was back from the war, 
And he had to the store, 
So he never went on the trial. \\ \vspace{0.1pt}

151: \textit{Fire:-2.675}, Method: No-Story\\
There was a fierce boy named Salvador,
Whose father was a soldier in war. 
When he returned to school, 
He was shocked by his cool, 
So he tried to get down on the floor. \\ \vspace{0.1pt}

152: \textit{Sports:-2.573}, Method: No-Story\\
There was a boxer named Beau,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
But he said he was taking it slow. \\ \vspace{0.1pt}

153: \textit{Water:-2.464}, Method: No-Story\\
There was a neat cleaner named Benito,
Who did a great job on our show. 
He was like a mentor, 
And he was to the core, 
He was willing to learn and to grow. \\ \vspace{0.1pt}

154: \textit{Love:-2.963}, Method: No-Story\\
There was a jealous boy named Salvador,
Whose father was a soldier in war. 
When he came to see her, 
He was shocked by her fur, 
Which was covered with the worst before. \\ \vspace{0.1pt}

155: \textit{Car:-2.565}, Method: No-Story\\
There was a funny boy named Benito,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
But he said he was taking it slow. \\ \vspace{0.1pt}

156: \textit{Animal:-2.894}, Method: No-Story\\
There was a nasty boy named Brock,
Who was a bad kid on our block. 
He was a musician, 
He was on a mission, 
He is a good guy out in the walk. \\ \vspace{0.1pt}

157: \textit{Violent:-2.773}, Method: No-Story\\
There was a nasty boy named Brock,
Who was a bad kid on our block. 
He was like a nightmare, 
He was scared by his hair, 
He was afraid to walk and to talk. \\ \vspace{0.1pt}

158: \textit{Opera:-2.543}, Method: No-Story\\
There was a lame actor named Benito,
Who did a great job on our show. 
He was like a mentor, 
And he was to the core, 
He was willing to learn and to grow. \\ \vspace{0.1pt}

159: \textit{Library:-2.868}, Method: No-Story\\
There was a smart teacher named Gaylord,
Who was a good student on my board. 
When I started to play, 
I was able to stay, 
And that is the goal of this record. \\ \vspace{0.1pt}

160: \textit{Monster:-2.798}, Method: No-Story\\
There was a warrior named Kip,
Who fought a great battle on his ship. 
When he returned to land, 
He was met by a band, 
And that is the story of this trip. \\ \vspace{0.1pt}

161: \textit{Noble:-2.819}, Method: No-Story\\
There was a soldier named Hugh,
Who was a good friend on our crew. 
He was like a mentor, 
And he was to the core, 
But he knew we were doing it true. \\ \vspace{0.1pt}

162: \textit{Market:-3.088}, Method: No-Story\\
There was a wise farmer named Scot,
Who had a small farm on our lot. 
He was like a mentor, 
And he was to the core, 
He knew that my family was hot. \\ \vspace{0.1pt}

163: \textit{Doctor:-2.885}, Method: No-Story\\
There was a surgeon named Ned,
Who did a great job on our head. 
He was like a mentor, 
And he was to the core, 
He wanted us down in the bed. \\ \vspace{0.1pt}

164: \textit{Funeral:-2.851}, Method: No-Story\\
There was a soldier named Hugh,
Who was a good friend on our crew. 
He was like a mentor, 
And he was to the core, 
He knew that our mission was true. \\ \vspace{0.1pt}

165: \textit{Ball:-2.831}, Method: No-Story\\
There once was a boy named Javier,
Who lived all his life in a nightmare. 
When he came to see her, 
He was struck by her fur, 
And that is the reason of this hair. \\ \vspace{0.1pt}

166: \textit{Body:-2.644}, Method: No-Story\\
There was a skinny man named Claudio,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
And he got down and took my photo. \\ \vspace{0.1pt}

167: \textit{Smart:-2.855}, Method: No-Story\\
There once was a man named Scot,
Who had all his money in a pot. 
When he went to trial, 
He was cleared by his file, 
So he got up and quit on the spot. \\ \vspace{0.1pt}

168: \textit{Exercise:-2.719}, Method: No-Story\\
There was a lazy judge named Chase,
Who did a great job on our case. 
When we went to trial, 
We had the same profile, 
So we had to go down on the base. \\ \vspace{0.1pt}

169: \textit{Gun:-2.620}, Method: No-Story\\
There was a silly boy named Dario,
Who was a big star on our show. 
He came back from the war, 
And he got to the door, 
And he looked down and saw my photo. \\ \vspace{0.1pt}

170: \textit{Art:-2.972}, Method: No-Story\\
There was a designer named Ward,
Who did a great job on our board. 
He was like a mentor, 
And he was to the core, 
He was willing to learn and to ward. \\ \vspace{0.1pt}

171: \textit{Music:-2.659}, Method: No-Story\\
There was a lively boy named Salvador,
Whose father was a soldier in war. 
But his mother was dead, 
He was left by his bed, 
So he went up and slept on the floor. \\ \vspace{0.1pt}

172: \textit{Boxing:-2.646}, Method: No-Story\\
There was a boxer named Romeo,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
And he got down and took my photo. \\ \vspace{0.1pt}

173: \textit{Philosophy:-2.711}, Method: No-Story\\
There was a general named Sergio,
Who was a big star on our show. 
He was a musician, 
He was on a mission, 
And he came down and got his photo. \\ \vspace{0.1pt}

174: \textit{Forest:-2.962}, Method: No-Story\\
There was a bright farmer named Brock,
Who had a big farm on our block. 
He was like a mentor, 
And he was to the fore, 
So we had to be down on the clock. \\ \vspace{0.1pt}

175: \textit{Night:-2.595}, Method: No-Story\\
There was a lucky boy named Dario,
Who was a big star on our show. 
He came back from the war, 
And he got to the door, 
And he looked down and saw my photo. \\ \vspace{0.1pt}

176: \textit{Scary:-2.534}, Method: No-Story\\
There once was a boy named Theodore,
Whose father was a soldier in war. 
But his mother was dead, 
He was left by his bed, 
So he had to sleep down on the floor. \\ \vspace{0.1pt}

177: \textit{Evil:-2.990}, Method: No-Story\\
There was a warrior named Kip,
Who fought a great battle on his ship. 
When he returned to shore, 
He was met by a door, 
And it opened down and left its grip. \\ \vspace{0.1pt}

178: \textit{Law:-2.700}, Method: No-Story\\
There was a harsh judge named Chase,
Who was a tough guy on our case. 
When we got to trial, 
We were able to smile, 
And that is the beauty of this place. \\ \vspace{0.1pt}

179: \textit{Creativity:-2.777}, Method: No-Story\\
There was a designer named Lyle,
Who did a great job on my profile. 
He was like a mentor, 
And he was to the core, 
He totally understood my style. \\ \vspace{0.1pt}

180: \textit{Angry:-3.024}, Method: No-Story\\
There was a rude boy named Salvador,
Whose father was a soldier in war. 
When he returned to school, 
He was struck by his cool, 
And took on the uniform therefore. \\ \vspace{0.1pt}

181: \textit{Pride:-2.651}, Method: No-Story\\
There was a humble boy named Theodore,
Whose father was a soldier in war. 
But his mother was dead, 
He was left by his bed, 
So he went up and slept on the floor. \\ \vspace{0.1pt}

182: \textit{Light:-2.474}, Method: No-Story\\
There was a bright cleaner named Beau,
Who did a great job on our show. 
He was like a mentor, 
And he was to the core, 
He was willing to learn and to grow. \\ \vspace{0.1pt}

183: \textit{School:-2.930}, Method: No-Story\\
There was a shy boy named Nathanael,
Whose father was a lawyer in jail. 
When he came to see her, 
He was struck by her fur, 
So he went up and slept on the rail. \\ \vspace{0.1pt}

184: \textit{Color:-2.965}, Method: No-Story\\
There was a designer named Lyle,
Who did a great job on my profile. 
When I went to see her, 
I was on a transfer, 
I was sure to get a good trial. \\ \vspace{0.1pt}

185: \textit{Leader:-2.786}, Method: No-Story\\
There was a soldier named Hugh,
Who was a good friend on our crew. 
He was like a mentor, 
And he was to the core, 
He was willing to work and to do. \\ \vspace{0.1pt}

186: \textit{Rich:-2.556}, Method: No-Story\\
There was a lively boy named Salvador,
Whose father was a soldier in war. 
But his mother was dead, 
He was left by his bed, 
So he had to sleep down on the floor. \\ \vspace{0.1pt}

187: \textit{Park:-2.851}, Method: No-Story\\
There was a lively boy named Kip,
Who was a good sport on our trip. 
When we returned to town, 
We had the same breakdown, 
So we had to go down on the ship. \\ \vspace{0.1pt}

188: \textit{Airplane:-2.466}, Method: No-Story\\
There was a firefighter named Beau,
Who did a great job on our show. 
He was like a mentor, 
And he was to the core, 
He was willing to learn and to grow. \\ \vspace{0.1pt}

189: \textit{Loss:-2.663}, Method: No-Story\\
There was a wise surgeon named Kip,
Who was a good doctor on our ship. 
He was a physician, 
He was on a mission, 
So he had to go down on the trip. \\ \vspace{0.1pt}

190: \textit{Weight:-2.832}, Method: No-Story\\
There was a doctor named Chase,
Who did a great job on our case. 
When we went to trial, 
I was shocked by his style, 
But I knew he was doing us grace. \\ \vspace{0.1pt}

191: \textit{Useful:-2.715}, Method: No-Story\\
There was a tailor named Bert,
Who did a great job on our shirt. 
He was like a mentor, 
And he was to the core, 
He was willing to learn and to hurt. \\ \vspace{0.1pt}

192: \textit{Applaud:-2.854}, Method: No-Story\\
There was a humble judge named Chase,
Who did a great job on our case. 
When we went to trial, 
It was the same profile, 
And it was not like something of race. \\ \vspace{0.1pt}

193: \textit{Home:-3.032}, Method: No-Story\\
There was a neat boy named Brock,
Who was a good friend on our block. 
When I got to know her, 
She was married to sir, 
But she does not live in our walk. \\ \vspace{0.1pt}

194: \textit{Child:-2.790}, Method: No-Story\\
There was a cruel boy named Javier,
Who lived all his life in a nightmare. 
He was like a shadow, 
He was afraid to go, 
So he went up and slept on the chair. \\ \vspace{0.1pt}

195: \textit{Union:-2.988}, Method: No-Story\\
There was a fierce lawyer named Ward,
Who had a great deal on his record. 
When he came to trial, 
He had the same profile, 
So he got up and put on the sword. \\ \vspace{0.1pt}

196: \textit{Working:-2.950}, Method: No-Story\\
There was a smart teacher named Ward,
Who was a good student on my board. 
He was like a mentor, 
And he was to the core, 
He was really the reason I scored. \\ \vspace{0.1pt}

197: \textit{Cheat:-2.798}, Method: No-Story\\
There was a warrior named Kip,
Who fought a great battle on his ship. 
When he returned to land, 
He was met by a band, 
And that is the story of this trip. \\ \vspace{0.1pt}

198: \textit{Time:-2.928}, Method: No-Story\\
There was a general named Abraham,
Who did a great job on our program. 
He was like a mentor, 
And he was to the core, 
He really enjoyed our programme. \\ \vspace{0.1pt}

199: \textit{Fall:-2.932}, Method: No-Story\\
There was a wise boy named Salvador,
Whose father was a soldier in war. 
When he returned to school, 
He was struck by a tool, 
So he quickly learned on the floor. \\ \vspace{0.1pt}

200: \textit{Hope:-2.906}, Method: No-Story\\
There was a brave boy named Salvador,
Whose father was a soldier in war. 
When he returned to school, 
He was shocked by his cool, 
He was not the student he before. \\ \vspace{0.1pt}

201: \textit{Random:-2.565}, Method: No-Story\\
There was a funny boy named Romeo,
Who was a big star on our show. 
He came back from the war, 
And he went to the store, 
But he said he was taking it slow. \\ \vspace{0.1pt}

202: \textit{Flower:-2.747}, Method: No-Story\\
There was a lucky boy named Scot,
Who had all his money in a pot. 
But his mother was dead, 
His father was a head, 
So he had to go down on the spot. \\ \vspace{0.1pt}

203: \textit{Impressive:-2.956}, Method: No-Story\\
There was a neat artist named Lyle,
Who did a great job on my profile. 
When I got to meet her, 
She was shocked by my fur, 
And that is the reason of this smile. \\ \vspace{0.1pt}





==> single_template_poem.tex <==
1: \textit{Musuem:-3.573}, Method: Single-Template\\
There was a blacksmith named Bridgette,
Who housed a small cottage on her street. 
She was like a statue, 
She was the perfect view, 
She was up in heaven and concrete. \\ \vspace{0.1pt}

2: \textit{Dawn:-2.862}, Method: Single-Template\\
There was a warrior named Rose,
Who slept on a mountain of shadows. 
When she awoke to light, 
She was shocked by a sight, 
And she fell down and covered her nose. \\ \vspace{0.1pt}

3: \textit{Memory:-3.209}, Method: Single-Template\\
There was a wise grandma named Lorraine,
Who used a hot iron on her brain. 
It was like a process, 
It was so much progress, 
She thought that her mother was insane. \\ \vspace{0.1pt}

4: \textit{Alien:-2.758}, Method: Single-Template\\
There was a warrior named Brande,
Who captured an area of land. 
When she began to fight, 
She was struck by a light, 
And she fell down and wounded her hand. \\ \vspace{0.1pt}

5: \textit{Heartbreak:-3.019}, Method: Single-Template\\
There once was a girl named Cher,
Who cried all her life in a nightmare. 
When she started to cry, 
Her mother told a lie, 
She said that her daughter was elsewhere. \\ \vspace{0.1pt}

6: \textit{Traffic:-3.256}, Method: Single-Template\\
There was a smart judge named Marguerite,
Who stopped a drunk driver on my street. 
She asked for my address, 
I gave the right access, 
And she got down and started her beat. \\ \vspace{0.1pt}

7: \textit{Pillow:-3.319}, Method: Single-Template\\
There was a chunky girl named Grace,
Who felt a strange presence on her face. 
She looked like a fairy, 
She was on a ferry, 
She was up in paradise and space. \\ \vspace{0.1pt}

8: \textit{Injury:-3.033}, Method: Single-Template\\
There was a surgeon named Geri,
Who healed a gunshot wound on her knee. 
When she returned to fight, 
She was shocked by her sight, 
And she fell down and broke her sunday. \\ \vspace{0.1pt}

9: \textit{Wine:-3.225}, Method: Single-Template\\
There was a waitress named Kay,
Who served a great meal on our day. 
It was a tradition, 
We were on a mission, 
And it was not easy work sunday. \\ \vspace{0.1pt}

10: \textit{Christmas:-3.134}, Method: Single-Template\\
There was a silly girl named Renee,
Who got a black eye on her birthday. 
It was like a rainbow, 
And she went to the show, 
She walked through the crowd and cried okay. \\ \vspace{0.1pt}

11: \textit{Thanksgiving:-3.147}, Method: Single-Template\\
There once was a lady named Kay,
Who ate a hot dog on her birthday. 
When she started to cry, 
It was the perfect guy, 
And she fell asleep quickly sunday. \\ \vspace{0.1pt}

12: \textit{Fiance:-2.969}, Method: Single-Template\\
There was a shy waitress named Kai,
Who talked as she waited on a guy. 
When she started to flirt, 
It was enough to hurt, 
But she thought she was getting him high. \\ \vspace{0.1pt}

13: \textit{Shaken:-3.225}, Method: Single-Template\\
There was a loud waitress named Tess,
Who poured a cold beer on our mess. 
When we arrived to stand, 
We were met by her hand, 
And she sat down and opened her dress. \\ \vspace{0.1pt}

14: \textit{Holiday:-3.311}, Method: Single-Template\\
There was a lucky girl named Renee,
Who stayed as she was on a birthday. 
It was like a spring, 
It was the perfect thing, 
It was nice to have a big buffet. \\ \vspace{0.1pt}

15: \textit{Kindness:-3.031}, Method: Single-Template\\
There once was a teacher named Kay,
Who learned a new language on her way. 
When she returned to mind, 
She was surprised to find, 
She was able to talk and to play. \\ \vspace{0.1pt}

16: \textit{River:-3.370}, Method: Single-Template\\
There once was a woman named Louise,
Who wandered on a mountain of seas. 
She came back from the sea, 
Took shelter of that tree, 
And she sat down and opened her trees. \\ \vspace{0.1pt}

17: \textit{Birthday:-2.971}, Method: Single-Template\\
There once was a lady named Renee,
Who gave all her money in a day. 
It was like a contest, 
And it was to the west, 
So we had to go down on the way. \\ \vspace{0.1pt}

18: \textit{Tears:-2.827}, Method: Single-Template\\
There was a vain lady named Grace,
Who felt a strange feeling on her face. 
When she started to cry, 
She was afraid to die, 
But she does not suffer in her place. \\ \vspace{0.1pt}

19: \textit{Surprise:-3.031}, Method: Single-Template\\
There was a shy lady named Kay,
Who did a great job on my birthday. 
She came back from the break, 
And we went to the lake, 
Was totally a different day. \\ \vspace{0.1pt}

20: \textit{Humiliation:-3.146}, Method: Single-Template\\
There was a lady named Grace,
Who faced a big problem on her face. 
She decided to cry, 
And she cried to the sky, 
It was easy to see and to trace. \\ \vspace{0.1pt}

21: \textit{Beer:-3.197}, Method: Single-Template\\
There was a silly chef named Kay,
Who ate all her dinner in a day. 
She was a potato, 
But had a nice torso, 
So she got up and slept on the tray. \\ \vspace{0.1pt}

22: \textit{Mud:-3.405}, Method: Single-Template\\
There was a chunky witch named Bok,
Who stuck out her fingers for a rock. 
It was like a playground, 
And it was to the ground, 
And that is the beauty of this walk. \\ \vspace{0.1pt}

23: \textit{Restore:-3.043}, Method: Single-Template\\
There was a wise cleaner named In,
Who tried a new method on her skin. 
When she returned to work, 
She was told by her clerk, 
She was ordered to strip and to spin. \\ \vspace{0.1pt}

24: \textit{Wedding:-2.883}, Method: Single-Template\\
There was a tailor named Rose,
Who decided on one of my clothes. 
I got back from the shop, 
And I went to the top, 
And I looked down and noticed my nose. \\ \vspace{0.1pt}

25: \textit{Victory:-2.781}, Method: Single-Template\\
There was a lieutenant named Grace,
Who fought a great battle on my place. 
She was back from the war, 
And she came to the door, 
And she sat down and opened her face. \\ \vspace{0.1pt}

26: \textit{Laugh:-3.118}, Method: Single-Template\\
There was a loud girl named Grace,
Who smiled a big smile on our face. 
I noticed on the way, 
She was stopped by a tray, 
And she looked down and saw our place. \\ \vspace{0.1pt}

27: \textit{Promise:-3.525}, Method: Single-Template\\
There was a vain liar named Dot,
Who wanted an audience of thought. 
She was a nobody, 
She was ashamed to be, 
She was proud to be a complete shot. \\ \vspace{0.1pt}

28: \textit{Season:-2.856}, Method: Single-Template\\
There was a shy captain named Kay,
Who put a big smile on our day. 
It was like a spring, 
It was the perfect thing, 
It was nice to have a warm birthday. \\ \vspace{0.1pt}

29: \textit{Rain:-3.169}, Method: Single-Template\\
There was a quiet girl named Marcell,
Who kept a close eye on our trail. 
When we got to twilight, 
We were met by a light, 
Which was filled with the finest detail. \\ \vspace{0.1pt}

30: \textit{Throne:-3.360}, Method: Single-Template\\
There once was a lady named Bethel,
Whose husband fled a battle in hell. 
When she returned to land, 
She was met by a hand, 
And asked her because she was rebel. \\ \vspace{0.1pt}

31: \textit{Politics:-3.150}, Method: Single-Template\\
There was a professor named Kay,
Who learned a new language on her way. 
She came back from the war, 
And she went to the store, 
And now she has a job resume. \\ \vspace{0.1pt}

32: \textit{Winter:-3.260}, Method: Single-Template\\
There was a bright lady named Rose,
Who decided on one of her clothes. 
It was on the daytime, 
It was the perfect time, 
It was also the moment she chose. \\ \vspace{0.1pt}

33: \textit{Beach:-3.382}, Method: Single-Template\\
There was a lazy girl named Rose,
Who went on a holiday of clothes. 
She came back from the trip, 
Found the dress on her slip, 
And decided on the perfect pose. \\ \vspace{0.1pt}

34: \textit{Spider:-3.407}, Method: Single-Template\\
There was a funny witch named Nicole,
Who trapped all my money in a hole. 
I got back from the cave, 
And I went to the grave, 
And killed her because she was charcoal. \\ \vspace{0.1pt}

35: \textit{Cunning:-3.258}, Method: Single-Template\\
There once was a liar named Kai,
Who fooled a grand jury on her lie. 
I had a suspicion, 
I was on a mission, 
I was ready to fight and to die. \\ \vspace{0.1pt}

36: \textit{Limerick:-4.092}, Method: Single-Template\\
There was a writer named Rose,
Who wright a short story on his prose. 
It was a satire, 
But it also had fire, 
And it came down and hit our nose. \\ \vspace{0.1pt}

37: \textit{Money:-2.841}, Method: Single-Template\\
There was a woman named Kay,
Who got a flat tire on her way. 
When she returned to work, 
She was told by a clerk, 
She did not have money left this day. \\ \vspace{0.1pt}

38: \textit{Love:-2.959}, Method: Single-Template\\
There was a jealous girl named Kay,
Who got a flat tire on her way. 
It was for her birthday, 
It was the perfect day, 
She walked through the door and saw sunday. \\ \vspace{0.1pt}

39: \textit{Bank:-2.867}, Method: Single-Template\\
There once was a farmer named Margarete,
Who owned a small farm on our street. 
She worked on the railroad, 
And she took to the road, 
And now she has a family seat. \\ \vspace{0.1pt}

40: \textit{Born:-2.707}, Method: Single-Template\\
There was a brave farmer named Kay,
Who died a young girl on her birthday. 
She came back from the grave, 
And she went to the cave, 
And she sat down and began her day. \\ \vspace{0.1pt}

41: \textit{War:-2.792}, Method: Single-Template\\
There was a warrior named Brande,
Who fought a great battle on her land. 
When she arrived to fight, 
She was struck by a light, 
And fell on the treacherous wasteland. \\ \vspace{0.1pt}

42: \textit{World:-2.919}, Method: Single-Template\\
There was a brave girl named Kay,
Who made a huge impact on my day. 
She was a nobody, 
She was raised by a tree, 
And she came down and saved my birthday. \\ \vspace{0.1pt}

43: \textit{Death:-3.051}, Method: Single-Template\\
There was a cruel judge named Clare,
Who lived all her life in a nightmare. 
When she returned to hell, 
She was able to tell, 
She saw all her friends lying nowhere. \\ \vspace{0.1pt}

44: \textit{Water:-3.157}, Method: Single-Template\\
There once was a cleaner named Dot,
Who washed out her windows for a pot. 
When she returned to land, 
She was able to stand, 
So she went up and slept on the spot. \\ \vspace{0.1pt}

45: \textit{Blood:-2.931}, Method: Single-Template\\
There was a vain doctor named Collette,
Who drank all her water in a sweat. 
She was a physician, 
She was on a mission, 
She was trained to be a great asset. \\ \vspace{0.1pt}

46: \textit{Sports:-3.004}, Method: Single-Template\\
There was a smart writer named Grace,
Who put a great spin on our race. 
She started on the show, 
She was ready to go, 
She was prepared to fight and to ace. \\ \vspace{0.1pt}

47: \textit{Fire:-3.236}, Method: Single-Template\\
There was a fierce woman named Maryann,
Who brought out my feelings for a man. 
We met on the roadside, 
It was raining outside, 
She said that her husband was afghan. \\ \vspace{0.1pt}

48: \textit{Planet:-2.851}, Method: Single-Template\\
There was a warrior named Brande,
Who lived a long time on our land. 
She came back from the war, 
And she went to the door, 
And stood on the threshold beforehand. \\ \vspace{0.1pt}

49: \textit{Disease:-3.237}, Method: Single-Template\\
There was a stubborn nurse named Joycelyn,
Who suffered an injury of skin. 
When she returned to fight, 
She was shocked by her sight, 
And now she has a permanent grin. \\ \vspace{0.1pt}

50: \textit{Dog:-2.696}, Method: Single-Template\\
There was a lucky girl named Loraine,
Who got a free ride on our train. 
When she started to walk, 
She was afraid to talk, 
So she had to sit down on the plane. \\ \vspace{0.1pt}

51: \textit{Love:-3.310}, Method: Single-Template\\
There was a jealous girl named Renee,
Who got a new boyfriend on her way. 
It was for her birthday, 
And she went to the play, 
And saw her because she was halfway. \\ \vspace{0.1pt}

52: \textit{Opera:-3.121}, Method: Single-Template\\
There was a lame dancer named Amal,
Who danced as she sat on a football. 
It was like a nightmare, 
It was painful to stare, 
But I knew she was watching me crawl. \\ \vspace{0.1pt}

53: \textit{Animal:-3.150}, Method: Single-Template\\
There was a woman named Renee,
Who found a dead body on her way. 
When she returned to land, 
She was met by her band, 
And they took down and burned her cache. \\ \vspace{0.1pt}

54: \textit{Car:-3.054}, Method: Single-Template\\
There was a smart woman named Jone,
Who put all her money in a loan. 
It was like a fire, 
And it burned to the wire, 
And she went down and broke her backbone. \\ \vspace{0.1pt}

55: \textit{Monster:-3.032}, Method: Single-Template\\
There was a sexy girl named Freda,
Who got a flat tire on her head. 
When she started to scream, 
She was stopped by her team, 
But they said she was doing it dead. \\ \vspace{0.1pt}

56: \textit{Library:-3.228}, Method: Single-Template\\
There once was a teacher named Dot,
Who found a dead body on her lot. 
She came back from the store, 
Saw the clothes that she wore, 
And knew her because she heard gunshot. \\ \vspace{0.1pt}

57: \textit{Noble:-3.437}, Method: Single-Template\\
There once was a lady named Ariane,
Who wished a good morning on her man. 
It was a tradition, 
She was on a mission, 
She was ready to go and to van. \\ \vspace{0.1pt}

58: \textit{Exercise:-3.333}, Method: Single-Template\\
There was a wise woman named Renee,
Who learned a great fortune on her way. 
When she returned to work, 
She was married to turk, 
But she knew she was getting him gay. \\ \vspace{0.1pt}

59: \textit{Market:-3.097}, Method: Single-Template\\
There was a wise farmer named Grace,
Who bought a small farm on our place. 
She started on the lot, 
And we moved to the plot, 
And now she has a permanent space. \\ \vspace{0.1pt}

60: \textit{Funeral:-3.188}, Method: Single-Template\\
There once was a grandma named Kay,
Who died a sad death on her birthday. 
She was like a statue, 
She had the perfect view, 
She was tall to be a female day. \\ \vspace{0.1pt}

61: \textit{Body:-2.966}, Method: Single-Template\\
There was a skinny girl named Grace,
Who put a big smile on our face. 
We got back from the break, 
And we went to the lake, 
Was totally a different place. \\ \vspace{0.1pt}

62: \textit{Doctor:-2.738}, Method: Single-Template\\
There was a nervous nurse named Loraine,
Who had a new baby on her brain. 
When she learned to talk, 
She was able to walk, 
She finally understood her pain. \\ \vspace{0.1pt}

63: \textit{Smart:-3.245}, Method: Single-Template\\
There was a smart lady named Lorelei,
Who put a blind fold on our guy. 
She asked for our key, 
And we went to the tree, 
And we had keys everywhere nearby. \\ \vspace{0.1pt}

64: \textit{Art:-2.691}, Method: Single-Template\\
There was a neat teacher named Kay,
Who made a big impact on my way. 
She was a musician, 
She was on a mission, 
She was ready to go and to play. \\ \vspace{0.1pt}

65: \textit{Gun:-2.939}, Method: Single-Template\\
There was a loud woman named Grace,
Who put a big smile on our face. 
It was like a flashlight, 
It was the perfect light, 
It came through the window and hit space. \\ \vspace{0.1pt}

66: \textit{Ball:-2.847}, Method: Single-Template\\
There was a lucky girl named Freda,
Who made a huge impact on my head. 
She was like a spring, 
She was the perfect thing, 
She was easy to write and to read. \\ \vspace{0.1pt}

67: \textit{Creativity:-3.503}, Method: Single-Template\\
There was a artist named Ines,
Who learned a great deal on her process. 
She started on the art, 
But she also worked smart, 
And she wrote down and showed her progress. \\ \vspace{0.1pt}

68: \textit{Boxing:-3.072}, Method: Single-Template\\
There was a warrior named Brande,
Who fought a great battle on her hand. 
She came back from the fight, 
Healed the wound on her knight, 
And entered the battlefield with brand. \\ \vspace{0.1pt}

69: \textit{Forest:-3.240}, Method: Single-Template\\
There was a bright lady named Bok,
Who covered as she went on a walk. 
She looked like a rainbow, 
She had so much shadow, 
It was hard to focus and to talk. \\ \vspace{0.1pt}

70: \textit{Philosophy:-3.159}, Method: Single-Template\\
There was a wise teacher named Bess,
Who taught a short course on my progress. 
She was like a mentor, 
And I felt to the core, 
She really admired my process. \\ \vspace{0.1pt}

71: \textit{Scary:-3.280}, Method: Single-Template\\
There was a boring girl named Sharleen,
Who seemed a good fit on our scene. 
She was like a nightmare, 
She was perfect to wear, 
She was easy to read and to mean. \\ \vspace{0.1pt}

72: \textit{Violent:-3.075}, Method: Single-Template\\
There was a harsh woman named Lore,
Whose husband killed a baby in war. 
When she returned to hell, 
She was saved by a spell, 
And now she is a holy mentor. \\ \vspace{0.1pt}

73: \textit{Night:-2.936}, Method: Single-Template\\
There was a quiet girl named Laure,
Who had a big smile on her before. 
It was for her birthday, 
It was the perfect day, 
It was also the party she wore. \\ \vspace{0.1pt}

74: \textit{Evil:-3.703}, Method: Single-Template\\
There was a selfish witch named Adell,
Whose soul possessed a demon in hell. 
She decided to flee, 
But it soon became he, 
And now she is a demon rebel. \\ \vspace{0.1pt}

75: \textit{Angry:-3.156}, Method: Single-Template\\
There was a fierce woman named Michele,
Whose death provoked a riot in hell. 
When she arrived to fight, 
She was killed by a knight, 
But she does not die within her cell. \\ \vspace{0.1pt}

76: \textit{Music:-2.949}, Method: Single-Template\\
There was a teacher named Brande,
Who played a big role on our band. 
She was on the record, 
And she came to the board, 
And now she has a permanent hand. \\ \vspace{0.1pt}

77: \textit{Color:-3.289}, Method: Single-Template\\
There once was a artist named Grace,
Who used a red lipstick on her face. 
When she started to fade, 
She was the perfect shade, 
But I am not ashamed for race. \\ \vspace{0.1pt}

78: \textit{Pride:-2.812}, Method: Single-Template\\
There was a fierce woman named Nicolle,
Who felt a deep longing on her soul. 
When she started to cry, 
She was afraid to die, 
So she chose to go down on the hole. \\ \vspace{0.1pt}

79: \textit{Rich:-3.060}, Method: Single-Template\\
There once was a farmer named Arline,
Who made a huge profit on her wine. 
It was a tradition, 
She was on a mission, 
And she did not like something of mine. \\ \vspace{0.1pt}

80: \textit{Law:-3.081}, Method: Single-Template\\
There was a honest judge named Grace,
Who passed a fair judgment on my case. 
She said on the trial, 
She was shocked by my file, 
It was strange to see a female face. \\ \vspace{0.1pt}

81: \textit{Light:-3.229}, Method: Single-Template\\
There was a woman named Renee,
Who made all her money in a way. 
It was like a rainbow, 
It was the perfect show, 
I loved that her character was gay. \\ \vspace{0.1pt}

82: \textit{Weight:-3.099}, Method: Single-Template\\
There was a wise girl named Shin,
Who felt a strange presence on her skin. 
When she started to sweat, 
Her body was so wet, 
She thought that her husband had akin. \\ \vspace{0.1pt}

83: \textit{Loss:-2.975}, Method: Single-Template\\
There was a wise woman named Kay,
Who helped a poor widow on her way. 
When she returned to fight, 
She was struck by a light, 
And she fell down and became her prey. \\ \vspace{0.1pt}

84: \textit{Leader:-2.932}, Method: Single-Template\\
There was a lieutenant named Kay,
Who led a small army on their way. 
When they arrived to fight, 
She was killed by a knight, 
But she does not die in our play. \\ \vspace{0.1pt}

85: \textit{Useful:-2.741}, Method: Single-Template\\
There was a smart cleaner named Dot,
Who found a dead body on her lot. 
When she returned to work, 
She was told by a clerk, 
She was not the manager she thought. \\ \vspace{0.1pt}

86: \textit{School:-3.049}, Method: Single-Template\\
There was a shy teacher named Pam,
Who did a great job on our program. 
She was like a mentor, 
And she taught to the core, 
And she got down and wrote our programme. \\ \vspace{0.1pt}

87: \textit{Applaud:-3.729}, Method: Single-Template\\
There was a wise writer named Dede,
Who wished a great deal on her indeed. 
She wanted to impress, 
She was eager to press, 
And she looked down and noticed her speed. \\ \vspace{0.1pt}

88: \textit{Union:-3.710}, Method: Single-Template\\
There was a fierce teacher named Willette,
Whose family paid a fortune in debt. 
When she returned to school, 
She was shocked by her cool, 
Young teachers are older and upset. \\ \vspace{0.1pt}

89: \textit{Airplane:-3.188}, Method: Single-Template\\
There was a captain named Germaine,
Who flew a big flag on our plane. 
We were on the highway, 
And we got to the bay, 
And we went right past something insane. \\ \vspace{0.1pt}

90: \textit{Child:-2.640}, Method: Single-Template\\
There was a nervous girl named Grace,
Who put a big smile on our face. 
When she started to cry, 
I was ready to die, 
But I knew she was giving me grace. \\ \vspace{0.1pt}

91: \textit{Park:-2.871}, Method: Single-Template\\
There once was a lady named Bridgette,
Who drove a white van on our street. 
We were on the highway, 
And we saw to the way, 
And we went down and took our seat. \\ \vspace{0.1pt}

92: \textit{Home:-2.758}, Method: Single-Template\\
There was a neat grandma named Kay,
Who had a new baby on her way. 
When she returned to town, 
Her son had a breakdown, 
And that is the story of this day. \\ \vspace{0.1pt}

93: \textit{Hope:-2.883}, Method: Single-Template\\
There was a lucky girl named Renee,
Who got a flat tire on her way. 
She decided to stay, 
It was the perfect day, 
It was easy to walk and to play. \\ \vspace{0.1pt}

94: \textit{Flower:-3.158}, Method: Single-Template\\
There was a bright woman named Ines,
Who cut a perfect line on her dress. 
It was on the rainbow, 
It was on a photo, 
It was easy to find and to press. \\ \vspace{0.1pt}

95: \textit{Cheat:-3.001}, Method: Single-Template\\
There was a hustler named Renee,
Who put all her money in a play. 
She was like a girlfriend, 
She would have a boyfriend, 
She was ready to go and to stay. \\ \vspace{0.1pt}

96: \textit{Working:-2.870}, Method: Single-Template\\
There was a smart nurse named Ines,
Who kept a close eye on my progress. 
When I needed to talk, 
She was ready to walk, 
But she does not travel in her dress. \\ \vspace{0.1pt}

97: \textit{Time:-2.993}, Method: Single-Template\\
There was a lady named Kay,
Who spent all her money in a day. 
She was a nobody, 
She was raised by a tree, 
She did not know life happened this way. \\ \vspace{0.1pt}


